Diagnosing and Repairing Distributed Routing Configurations Using Selective Symbolic Simulation

Although substantial progress has been made in automatically verifying whether distributed routing configurations conform to certain requirements, diagnosing and repairing configuration errors remains manual and time-consuming. To fill this gap, we propose S^2Sim, a novel system for automatic routing configuration diagnosis and repair. Our key insight is that by selectively simulating variants of the given configuration in a symbolic way, we can find an intent-compliant variant, whose differences between the given configuration reveal the errors in the given configuration and suggest the patches. Building on this insight, we also design techniques to support complex scenarios (e.g., multiple protocol networks) and requirements (e.g., k-link failure tolerance). We implement a prototype of S^2Sim and evaluate its performance using networks of size O(10) ~ O(1000) with synthetic real-world configurations. Results show that S^2Sim diagnoses and repairs errors for 1) all WAN configurations within 10 s and 2) all DCN configurations within 20 minutes.

==> abstract.tex <==
\begin{abstract}

% \parablue{Qiao, 0.5 pages}

Although substantial progress has been made in automatically verifying whether distributed routing configurations conform to certain requirements, diagnosing and repairing configuration errors remains manual and time-consuming. To fill this gap, we propose \system{}, a novel system for automatic routing configuration diagnosis and repair.
\rulan{Our key insight is that by selectively performing concrete and symbolic simulation to explore only the paths deemed relevant (\ie, those that could meet the specified requirements),
we can identify configuration variants that drive simulation through such paths. The differences between the variants and the original configuration help uncover errors and suggest potential patches.} 
Building on this insight, we also design techniques to support complex scenarios (\eg, multiple protocol networks) and requirements (\eg, k-link failure tolerance).
We implement a prototype of \system{} and evaluate its performance using networks of size $O(10) \sim O(1000)$ with synthetic real-world configurations. Results show that \system{} diagnoses and repairs errors for 1) all WAN configurations within 10 s and 2) all DCN configurations within 20 minutes.




\end{abstract}


==> basic_design.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/repaired-cfgs.pdf}
%     \caption{The repair results of the example.}
%     \label{fig: repaired-cfgs}
% \end{figure}

\section{Basic Design}
\label{sec: sss}
We will delve into the detailed design of the \system{} in this section.
We support BGP protocol, prefix/community/as-path filters, access-control lists (ACLs), and attributes such as route aggregation and multi-path routing. We will also introduce how this design generalizes to the OSPF protocol and handles multi-protocol networks in \(\S\ref{sec:multi-protocol}\), and supports failure tolerance intents in \(\S\ref{sec:k-failure}\).


\para{The network intent.} 
\system{} allows operators to specify the intent as a 5-tuple \((src, dst, n, P, type)\), where \(P\) is the path set that the operator intends for the traffic destined for prefix \(n\) to follow, from the source node \(src\) to the destination node \(dst\). The \(type\) is the path requirement type of \(P\). The path set \(P\) can be expressed as a regular expression, and we support 3 path requirement types: (1) \(any\_path\), which means the traffic should be forwarded along any paths in \(P\); (2) \(fail \le k\), which means the traffic should be forwarded along any paths in \(P\) under at most \(k\) link failures; (3) \(equal\_path\), which means the traffic should be forwarded along all paths in \(P\) equally.



\subsection{Intent-compliant Data Plane Computation} 
\label{subsec:forwarding tree}

We represent the intended data plane for a set of intents from different sources to the same prefix in the same destination as a set of forwarding paths, where the outgoing edge of each node indicates its best next hop, and all these paths form a forwarding tree.
Inspired by the product graph~\cite{beckett2016don, soule2018merlin, xiang2023beyond}, which uses automata theory to multiply the path regular expression and the topology to get all paths in the topology that match the regular expression. 
We leverage this insight but only find one valid path for each intent's regular expression to construct the forwarding tree. 




The intent-compliant data plane computation algorithm~\ref{algorithm: DP} works as follows. First, given the network, the reused paths, and the unsatisfied intents, we convert the network topology into a directed graph. Then, we enforce path constraints by retaining only the reused path for each source node (lines 1–2). Specifically, for each node on a reused path, we delete all edges except for the one to its next hop. 
When searching the intent-complaint path for each intent, we convert its regular expression into a Deterministic Finite Automaton (DFA) and multiply it with the direct graph via a breadth-first search to find the shortest valid path that complies with the intent (line 5). 
Once a valid path is found, we remove it from the unsatisfied set and take this path as a constraint to guide subsequent topology multiplications (lines 15–17).

If there is no valid path for an intent, it indicates that the current path constraints are too strict. 
To address this, we apply a greedy strategy that always removes all equally longest paths first (line 7) to relax constraints.  
Specifically, for each of these longest paths, we remove it from the reused path set, making the intent as unsatisfied (\ie, the path can be recomputed), and relaxing the path constraint by re-adding all edges for the source node in the direct graph (line 9-11). We then restart the search for valid paths for all unsatisfied intents.

This process iterates until valid paths are found for all unsatisfied intents. To prevent infinite loops during path search, if an intent is processed more than once, we ensure that each new multiplication seeks a path different from those already discovered. Finally, all valid paths are added to the reused path set, forming an intent-compliant data plane.





 





% The traversal will terminate once all DFAs have reached the final state at some node. Thus, we find at least one path that matches each regular expression. Since we choose the breath-first search strategy, it will first find the shortest path for each intent. In this example, \(ACWD\) and \(BED\) are the founded paths for the two DFAs, respectively, which form an intended forwarding tree.





\begin{algorithm}[t]
\SetAlgoLined 
\caption{Computing an intent-compliant data plane.}
\KwIn{
The network topology $G$,
reused path set $C$,  
unsatisfied intent set $S$.
}
\KwOut{The intent-compliant data plane.}

$DG = convertToDirectedGraph(G)$ \\
$DG = addConstraints(DG, C)$ \\

\While{ $\neg$isEmpty(S) }{
    \ForEach{intent $I \in S$}{
    $path = multiply(DG, I)$ \\
    \If{$path= \emptyset $}{
        $P=getLongestPaths(C)$ \\
        \ForEach{ $lpath \in P$}{
            $C=C\backslash \{lpath\}$ \\
            $S=S\cup getIntent(lpath)$ \\
            $DG=relaxConstraints(DG, lpath)$ \\
        }
        $break$\\
    }
    $S=S\backslash \{I\}$ \\
    $C=C\cup path$ \\
    $DG=addConstraints(DG, path)$ \\
    }
}
return $C$

\label{algorithm: DP}
\end{algorithm}







% based on the routing-level topology (BGP neighbor relationship in the example network). we extract from the network configuration. Suppose there is no such path for a requirement in the routing-level topology. We will try to add routing neighbors by scanning the configuration to search for potential neighbors that are configured but have not established peer sessions successfully.



% Then we reverse the forwarding graph to get the routing graph\footnote{Generall, reversing edges hop-by-hop is feasible, but there could be a little difference in multiple-protocol networks, this will be discussed in \S\ref{multi-protocol section}.}, which indicates the necessary route propagation and selection of each routing process, as Figure~\ref{sss process}(c) shows. 





\subsection{Generating contracts}\label{router behaviors}

% \rulan{static routes, ACL, ECMP}

\system{} abstracts a set of branching conditions controlled by the configuration as Boolean router behavior variables. 
As Table~\ref{tab:router behavior} shows, including (1) basic BGP behaviors we illustrate in \S\ref{basic_workflow}: peering, importing/exporting a route, and selecting a route; (2) redistribution behavior for exchanging routes between different types of routing process; (3) equally prefer behavior for equivalent multi-path routing; and (4) forwarding behavior for the ACL control. 
We represent the guided constraint with these variables and only explore the branches where the constraint is satisfied. 
We then introduce how to generate a set of constraints that indicate the formation of an intended forwarding tree.


\para{The intended best route of each node.} The paths of the forwarding tree indicate the propagation of the best routes. We use two well-known mandatory BGP attributes \(AS\_PATH\) and \(NEXT\_HOP\) that can be computed from the forwarding tree to represent a set of best routes we intend to select at each node \footnote{We also perverse the actual \(AS\_PATH\) of each route in case of there are route policies that could modify this attribute.}, \eg, the forwarding path of A is \([A, C, W, D]\) (corresponding route's as-path list is \([3,5,6]\)), so we have BEST$_A$=\(\{10/8, [3,5,6], C\}\), which represents the routes whose \(AS\_PATH\) matches \([3,5,6]\), \(NEXT\_HOP\) is \(C\), with any other attributes should be the best route of \(A\). 

\para{Route propagation constraints.}
We then add constraints to the route propagation process to ensure that the intended route is propagated successfully along the reversed forwarding paths. We use three types of variables: $isPeered, isImported$, and $isExported$ to specify the intended router behaviors. If there is an edge from \(u\) to \(v\), suppose \(r\) is the route sent by \(v\) to \(u\) and \(r'\) is the route received by \(u\) from \(v\), we have constraints:
\[isPeered_{u,v}==True\]
\[\forall r \in BEST_v \Longrightarrow isExported_{v,u}^r==True\]
\[\forall r' \in BEST_u \Longrightarrow  isImported_{u,v}^{r'}==True\]

\(isPeered\) constraint specifies \(u\) and \(v\) should be routing neighbor, 
\(isExported\ (isImported)\) constraint specifies \(v\) (\(u\)) should export (import) its intended best route to (from) \(u\) (\(v\)) successfully. 
For the root node \(root\) (without outgoing edge) of the forwarding tree, we have \(RedisToBgp_{root}^{pfx}==True\), indicating that \(root\) should redistribute the original route.


\para{Route selection constraints.} 
Given each node's intended best route, we need to add constraints to its route selection process to ensure that the intended route is correctly selected.                    
Specifically, if node \(u\)'s best next hop is \(v\), for each of \(u\)'s other neighbors \(n\), given route \(r\) from \(v\) and route \(r'\) from \(n\), we have:  
\[ \forall r \in BEST_u,\forall {r'} \notin BEST_u \Longrightarrow BgpPrefer_u^{r,r'}==True\]
It means the route received from a node's best next hop, which matches its best route, should be the most preferred. 


\para{Packet forwarding constraints.} 
Although the above constraints could guide the simulation to form the intended routes. The actual data plane forwarding behavior could be unintended due to the presence of an ACL, which allows a router to block traffic directly in the data plane. To handle ACLs, we add a \(canForward_{u,v}^p==True\) constraint for each edge \(u\rightarrow v\), where the \(p\) is the packet destined for the destination prefix, representing that the packet should be forwarded along the forwarding tree as intended. 


% For example, $A\rightarrow B$ indicates: (1) A and B , \ie,  holds, (2) for each route $r$ sent to B, if it matches BEST\_A, it should be successfully exported, as condition (1) shows, (3) for each route $r$ received from A, if it matches BEST\_B, it should be successfully imported, as condition (2) shows. Also, C should prefer the route from neighbor E, which also matches BEST\_C, to routes from all other neighbors W and B, as conditions (3)-(4) show.





 

\begin{table}[t]
  \small
  \centering
  \begin{tabular}{|p{2.5cm}|p{5cm}|} 

    \hline
    \textbf{Boolean variable} & \textbf{Description} \\

    \hline
    $isPeered_{u,v}$ & Does node $u$ establish BGP peer session with $v$ successfully. \\

    \hline
    $BgpPrefer_u^{r_1, r_2}$ & Does node \(u\) prefer route $r_1$  to $r_2$. \\ 

    % \hline
    % $equal(r_1, r_2)$ & Do routes $r_1$ and $r_2$ are equally preferred. \\

    \hline
    \(RedisToBgp_u^{pfx}\) & Does node \(u\) redistribute its route with prefix \(prx\) to its BGP successfully.\\

    \hline
    $isExported_{u,v}^r$ &  Can node $u$ successfully export route $r$ to $v$ based on import rules. \\

    \hline
    $isImported_{u,v}^r$ & Can node $u$ successfully import route $r$ from $v$ based on import rules.\\

    \hline
    \(canForward_{u,v}^p\) & Can node \(n\) successfully forward packet \(p\) to node \(m\) based on ACL rules. \\
 
    \hline
    
  \end{tabular}
  \caption{Router behavior variables.}
  \vspace{-1em}
  \label{tab:router behavior}
\end{table}




% We first abstract the router configuration, which controls how each routing process exchanges advertisements with neighbors and computes paths, into four Boolean \textit{router behavior variables}. 


% To automatically generate the constraints that could lead the simulation to execute to a point where the network state meets all intents. 




\subsection{Repairing The Error} \label{subsec:patch generation}

% \para{Diagnosing the errors.} 
% We diagnose the violated conditions, \ie, the given configuration does not hold, as configuration errors. The corresponding router behaviors of each condition can be mapped to the given configuration files in a systematic way. In the example, $Cond_1=false$ and $Cond_2=false$ are configuration errors, indicating that Err1 is the missing of redistribution configuration and Err2 is $r_4$ should not be preferred over $r_3$.

\para{The repair template.} 
We consider the necessary low-level configuration component that controls the corresponding high-level broken router behavior as the repair template. 
Specifically, for \(isPeered\) and \(RedisToBgp\) behaviors, we directly complete the neighboring (\ie, IP address, AS number, enable routing) or redistribution commands with respect to the corresponding IP/prefix. 
Other behaviors are typically governed by specific policies, \ie, import policy controls \(BgpPrefer\) and \(isImported\) behaviors, export policy controls \(isExported\) behaviors while ACL controls \(canForward\) behaviors. Each policy is defined as a set of rules structured in a match-set format to process specific routes ( ACLs are relatively simple, as they only permit or deny packets without modifying them). We use the rule with all types of matches and set actions as the repair template, then search for the specific values to complete the rule.
% Specifically, the template for repairing \(BgpPrefer\) or \(isImported\) behavior is the import policy that is responsible for 


\para{Computing the patch as a constraint-solving problem.}
Given a policy to be repaired and a set of routes/packets to be processed with it, we first add a new rule on top of the policy, symbolize each rule value, and encode the intended process result of each route/packet as a constraint-solving problem, then compute a satisfiable assignment using the SMT solver as the patch.
Figure~\ref{fig:patch constraint} shows how we encode the fix of policy M, where M controls a broken and unbroken behavior. 
In this example, assume the new rule of M must permit \(r_2\), prefer \(r_2\) over \(r_3\), and avoid matching \(r_1\). The template rule has two matches and sets local-preference, as it is a non-transitive BGP attribute. Constraint (1) ensures this rule matches first; Constraint (2) permits matched routes. Constraints (2)-(3) ensure \(r_2\) matches while \(r_3\) does not, and Constraint (5) ensures that \(r_2\) is preferred to \(r_3\). Finally, we convert the satisfiable assignment of these values, following the configuration syntax, to generate the repair patch.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/patch-solving.png}
    \caption{Encoding the repair constraints for route policy M.}
    \label{fig:patch constraint}
\end{figure}


\subsection{Supporting Complex Configuration}

\para{Handling multi-path routing.} 
Multi-path routing is a routing strategy where packet forwarding to a single destination can occur over multiple best paths with equal routing priority.
Given an equal-cost multi-path routing intent \((src, dst,n,P,equal\_path)\), where \(P=\{p_1, ...,p_n\}\).
We address this intent by extending the forwarding tree (where each node has only one next-hop) to the forwarding graph (where each node can have multiple next-hops). 
Thus, a node \(n\) could have multiple intended routes propagated along the reversed forwarding paths, suppose they are \(BEST_{p_1},...,BEST_{p_n}\), we denoted the best routes of \(n\) as \(BEST_n=BEST_{p_1} \cup ...\cup BEST_{p_n}\).
We introduce a new Boolean router behavior variable \(BgpEqualPrefer_u^{r_1,r_2}\) to indicate whether two routes are equally preferred. 
Specifically, assume routes \(r_i,r_j\) are from node \(n\)'s best next hops, and \(r_k\) is form other neighbors, we have:
\[\forall r_i\in BEST_n, \forall r_j\in BEST_n \Longrightarrow BgpEqualPrefer_{n}^{r_i,r_j}==True\]
\[\forall r_i\in BEST_n, \forall r_k\notin BEST_n \Longrightarrow BgpPrefer_{n}^{r_i,r_k}==True\]
\[\forall r_j\in BEST_n, \forall r_k\notin BEST_n \Longrightarrow BgpPrefer_{n}^{r_j,r_k}==True\]

They indicate that the routes received from the best next hops, which match the best route, should be equally preferred, and each should be preferred to any other route.


\para{Handling route aggregation.}
Route aggregation is a method of combining multiple IP prefixes into a single, larger prefix to reduce the size of the routing table and improve network efficiency. 
If a node is configured to aggregate a prefix, it only announces the aggregated route to its neighbor. 
Thus, all traffic destined for the aggregated prefix will traverse the same path from the source nodes to the aggregated node. 
When constructing the forwarding tree, we need to carefully choose the paths to the prefixes that could be aggregated for each source. 
Specifically, given two candidate path sets \(P_u^{n_1}\) and \(P_u^{n_2}\) for node \(u\) to reach networks \(n_1\) (intent 1) and \(n_2\) (intent 2), respectively, if there exists a node \(a\) that will aggregate both \(n_1\) and \(n_2\), we group the paths from the two sets based on whether the sub-path from \(u\) to \(a\) is the same. 
We remove any groups containing paths from only one intent, as these paths would conflict with those from the other intent. Only paths within the same group can be selected for constructing the forwarding trees for the two intents, ensuring sub-path consistency from the source to the aggregation node.




==> basic_design_old.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/repaired-cfgs.pdf}
%     \caption{The repair results of the example.}
%     \label{fig: repaired-cfgs}
% \end{figure}

\section{Basic Design}
\label{sec: sss}
We will delve into the detailed design of the \system{} in this section.
We support BGP protocol, prefix/community/as-path filters, access-control lists (ACLs), and attributes such as route aggregation and multi-path routing. We will also introduce how this design generalizes to the OSPF protocol and handles multi-protocol networks in \(\S\ref{sec:multi-protocol}\), and supports failure tolerance intents in \(\S\ref{sec:k-failure}\).


\para{The network intent.} 
\system{} allows operators to specify the intent as a 5-tuple \((src, dst, n, P, type)\), where \(P\) is the path set that the operator intends for the traffic destined for prefix \(n\) to follow, from the source node \(src\) to the destination node \(dst\). The \(type\) is the path requirement type of \(P\). The path set \(P\) can be expressed as a regular expression, and we support 3 path requirement types: (1) \(any\_path\), which means the traffic should be forwarded along any paths in \(P\); (2) \(fail \le k\), which means the traffic should be forwarded along any paths in \(P\) under at most \(k\) link failures; (3) \(equal\_path\), which means the traffic should be forwarded along all paths in \(P\) equally.

% \system{} allows operators to specify the intent as a 5-tuple \((src, dst, n, P, type)\), where \(P\) is the path set that the operator intends for the traffic destined for prefix \(n\) to follow, from the source node \(src\) to the destination node \(dst\). The \(type\) is the path requirement type of \(P\). The path set \(P\) can be expressed as a regular expression, and we support 3 path requirement types: (1) \(any\_path\), which means the traffic should be forwarded along any paths in \(P\); (2) \(fail \le k\), which means the traffic should be forwarded along any paths in \(P\) under at most \(k\) link failures; (3) \(equal\_path\), which means the traffic should be forwarded along all paths in \(P\) equally.


\subsection{Computing The Intent-compliant Data Plane} 
\label{subsec:forwarding tree}

We represent the intended data plane for a set of intents from different sources to the same prefix in the same destination as a forwarding tree, where the outgoing edge of each node indicates its best next hop, and the path to the destination is its intended forwarding path.
Our approach to constructing the forwarding tree is inspired by the product graph~\cite{beckett2016don, soule2018merlin, xiang2023beyond}, which uses automata theory to multiply the path regular expression and the topology to get a directed acyclic graph (DAG), resulting in a directed acyclic graph (DAG) that captures all paths in the topology that match the regular expression. 
% Additionally, we introduce two key design adaptations tailored to our scenario
Additionally, we have considered three key points: (1) Avoiding path conflicts, meaning that a path complying with one intent may have sub-paths that conflict with other intents, (2) Avoiding next-hop conflicts, meaning that the next hop for the same node in different paths may conflict with each other, and (2) Minimizing data plane impact, meaning we try to preserve existing paths (that do not conflict with other intents) as much as possible when computing the new intended forwarding graph.


Given a set of path regular expressions and the topology, we first represent each regular expression as a Deterministic Finite Automaton (DFA), and then we traverse the topology along all DFAs to construct the DAG, finally building the conflict-free forwarding tree.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/product-graph.png}
%     \caption{The forwarding tree construction.}
%     \label{fig:forwarding-tree construction}
% \end{figure}

\para{Conflict-free forwarding tree construction.} We address the potential path conflicts by always searching the intersection of acceptable topology nodes of all DFAs. 
We use a similar topology as the example network in Figure~\ref{fig:forwarding-tree construction} to show the construction process. 
There are two intents whose path regular expressions are \(A.*W.*D\) and \(B.*!A.*D\),
The DFA of the first one accepts all paths from \(A\) to \(D\) that pass through \(W\) and the DFA of the second one accepts all paths from \(B\) to \(D\) that do not pass through \(A\).
We traverse the topology using the breath-first search while tracking the state of each DFA to construct the product DAG. 

Each DAG node is represented as $(l, s_1, s_2, ..., s_n)$, where $l$ is the node's topology location and $s_i$ is the current state of each DFA. 
For example, $(B_2, 1, 1)$ means that when traversing to \(B\), the first DFA reaches state 1, and the second DFA reaches state 1. 
We add an edge from a DAG node $(l,...)$ to the next DAG node $(l',...)$ only if $l'$ is the topological neighbor of $l$ and $l'$ can be accepted by all non-initial states in $(l,...)$. For example, $(C_2, 1, 1)$ did not continue traversing $D$ because DFA \(1\) cannot accept $D$ at state \(1\). A DAG node goes to the dead state if there is no more acceptable topology node at that point, \ie, as the gray node \((B_3,2,1)\) shows.
We use the double circle to represent the ended node, where at least one DFA reaches the final state, \eg, \((D_1,3,0)\) indicates that path \(AWD\) is accepted by DFA \(1\).
Each traversal branch terminates if it goes to the dead state or the ended state. Thus, we find all path-conflict-free paths that match each regular expression. 

Next, we choose one next-hop-conflict-free path from a set of candidate paths for each intent to build the intent-complaint forwarding tree.
In this example, the candidates for intent 1 and intent 2 are paths accepted by \(\{D_1,D_2,D_3\}\) and \(\{D_2,D_4,D_5\}\), respectively.
We begin by selecting the shortest path for each intent, \eg, \(AWD\) (accepted by \(D_1\)) and \(BCD\) (accepted by \(D_2\)), to form the intended forwarding tree. 
However, if a next-hop conflict arises between two paths (\eg, paths accepted by \(D_1\) and \(D_4\)), one of them is replaced with an alternative, conflict-free path. This process continues iteratively until a next-hop-conflict-free combination of paths is found.



% The traversal will terminate once all DFAs have reached the final state at some node. Thus, we find at least one path that matches each regular expression. Since we choose the breath-first search strategy, it will first find the shortest path for each intent. In this example, \(ACWD\) and \(BED\) are the founded paths for the two DFAs, respectively, which form an intended forwarding tree.



\para{Data plane impact minimization.} We preserve the actual paths that are taken by satisfied intents to minimize the impact on the existing data plane when computing the intended forwarding tree. Specifically, if a path \(p=[x_0, x_1,..., x_n]\), where \(x_0\) is the source and \(x_n\) is the destination, already complies with the intent \((src, dst, n, P,any\_path)\), we will replace this intent's regular expression with \(p\), which is also a regular expression that exactly matches a specific path, to build its DFA, as the intent (2) shown in Figure~\ref{sss process}(a).

\begin{algorithm}[t]
\caption{The greedy algorithm for finding an intent-compliant data plane.}
\KwIn{
The network topology $Graph$,
The satisfied path set $P_s=\{p_1,...,p_m\}$,  
The DFAs of all unsatisfied intents $\{DFA_1,...,DFA_n\}$.
}
$Tree = merge(P_s);$ \\ 
$DFA_{all} = DFA_1 \cup ...\cup DFA_n;$ \\
$DiGraph = convertToDirectedGraph(G);$ \\
$DiGraph = preserve(DG, P_s);$ \\
$DAGraph= DFA_{all} \times DiGraph$; \\
\While{ $(notAllIntentsHaveAPath(DAGraph))$ }{
    \State $node = removeDeepestLeafNode(Tree);$ \\
    \State $DiGraph = loose(DiGraph, node);$ \\
    \State $DAGraph=search(DAGraph,DiGraph,DFA_{all});$
}
\ENDWhile  
$// assign non-conflict paths for each intent.$

\label{algorithm: greedy}
\end{algorithm}



However, preserving all satisfied paths does not always guarantee that a feasible solution can be found, \ie, it may lead to pruning the branches that could search to find a forwarding tree. In this case, we use a greedy algorithm to remove these paths to find how many existing paths can be preserved. 
As shown in Algorithm 1, we first sort the set of satisfied paths \(P_s\) by length to prioritize removing the shortest paths. This greedy strategy maximizes the preservation of the existing data plane.
We then iterate the possible number of paths to remove, starting with removing one path, then two paths, and so on.
Each iteration tests all ordered combinations of removing \(k\) paths.
The algorithm will terminate once there is an intended forwarding tree can be found.


% based on the routing-level topology (BGP neighbor relationship in the example network). we extract from the network configuration. Suppose there is no such path for a requirement in the routing-level topology. We will try to add routing neighbors by scanning the configuration to search for potential neighbors that are configured but have not established peer sessions successfully.








\subsection{Generating Router Behavior Constraints}\label{router behaviors}

% \rulan{static routes, ACL, ECMP}

\system{} abstracts a set of branching conditions controlled by the configuration as Boolean router behavior variables. 
As Table~\ref{tab:router behavior} shows, including (1) basic BGP behaviors we illustrate in \S\ref{basic_workflow}: peering, importing/exporting a route, and selecting a route; (2) redistribution behavior for exchanging routes between different types of routing process; (3) equally prefer behavior for equivalent multi-path routing; and (4) forwarding behavior for the ACL control. 
We represent the guided constraint with these variables and only explore the branches where the constraint is satisfied. 
We then introduce how to generate a set of constraints that indicate the formation of an intended forwarding tree.


% Then we reverse the forwarding graph to get the routing graph\footnote{Generall, reversing edges hop-by-hop is feasible, but there could be a little difference in multiple-protocol networks, this will be discussed in \S\ref{multi-protocol section}.}, which indicates the necessary route propagation and selection of each routing process, as Figure~\ref{sss process}(c) shows. 




\para{The intended best route of each node.} The paths of the forwarding tree indicate the propagation of the best routes. We use two well-known mandatory BGP attributes \(AS\_PATH\) and \(NEXT\_HOP\) that can be computed from the forwarding tree to represent a set of best routes we intend to select at each node \footnote{We also perverse the actual \(AS\_PATH\) of each route in case of there are route policies that could modify this attribute.}, \eg, the forwarding path of A is \([A, C, W, D]\) (corresponding route's as-path list is \([3,5,6]\)), so we have BEST$_A$=\(\{10/8, [3,5,6], C\}\), which represents the routes whose \(AS\_PATH\) matches \([3,5,6]\), \(NEXT\_HOP\) is \(C\), with any other attributes should be the best route of \(A\). 

\para{Route propagation constraints.}
We then add constraints to the route propagation process to ensure that the intended route is propagated successfully along the reversed forwarding paths. We use three types of variables: $BgpPeer, canImport$, and $canExport$ to specify the intended router behaviors. If there is an edge from \(u\) to \(v\), suppose \(r\) is the route sent by \(v\) to \(u\) and \(r'\) is the route received by \(u\) from \(v\), we have constraints:
\[BgpPeer_{u,v}==True\]
\[\forall r \in BEST_v \Longrightarrow canExport_{v,u}^r==True\]
\[\forall r' \in BEST_u \Longrightarrow  canImport_{u,v}^{r'}==True\]

\(BgpPeer\) constraint specifies \(u\) and \(v\) should be routing neighbor, 
\(canExport\ (canImport)\) constraint specifies \(v\) (\(u\)) should export (import) its intended best route to (from) \(u\) (\(v\)) successfully. 
For the root node \(root\) (without outgoing edge) of the forwarding tree, we have \(RedisToBgp_{root}^{pfx}==True\), indicating that \(root\) should redistribute the original route.


\para{Route selection constraints.} 
Given each node's intended best route, we need to add constraints to its route selection process to ensure that the intended route is correctly selected.                    
Specifically, if node \(u\)'s best next hop is \(v\), for each of \(u\)'s other neighbors \(n\), given route \(r\) from \(v\) and route \(r'\) from \(n\), we have:  
\[ \forall r \in BEST_u,\forall {r'} \notin BEST_u \Longrightarrow BgpPrefer_u^{r,r'}==True\]
It means the route received from a node's best next hop, which matches its best route, should be the most preferred. 


\para{Packet forwarding constraints.} 
Although the above constraints could guide the simulation to form the intended routes. The actual data plane forwarding behavior could be unintended due to the presence of an ACL, which allows a router to block traffic directly in the data plane. To handle ACLs, we add a \(canForward_{u,v}^p==True\) constraint for each edge \(u\rightarrow v\), where the \(p\) is the packet destined for the destination prefix, representing that the packet should be forwarded along the forwarding tree as intended. 


% For example, $A\rightarrow B$ indicates: (1) A and B , \ie,  holds, (2) for each route $r$ sent to B, if it matches BEST\_A, it should be successfully exported, as condition (1) shows, (3) for each route $r$ received from A, if it matches BEST\_B, it should be successfully imported, as condition (2) shows. Also, C should prefer the route from neighbor E, which also matches BEST\_C, to routes from all other neighbors W and B, as conditions (3)-(4) show.





 

\begin{table}[t]
  \small
  \centering
  \begin{tabular}{|p{2.5cm}|p{5cm}|} 

    \hline
    \textbf{Boolean variable} & \textbf{Description} \\

    \hline
    $BgpPeer_{u,v}$ & Does node $u$ establish BGP peer session with $v$ successfully. \\

    \hline
    $BgpPrefer_u^{r_1, r_2}$ & Does node \(u\) prefer route $r_1$  to $r_2$. \\ 

    % \hline
    % $equal(r_1, r_2)$ & Do routes $r_1$ and $r_2$ are equally preferred. \\

    \hline
    \(RedisToBgp_u^{pfx}\) & Does node \(u\) redistribute its route with prefix \(prx\) to its BGP successfully.\\

    \hline
    $canExport_{u,v}^r$ &  Can node $u$ successfully export route $r$ to $v$ based on import rules. \\

    \hline
    $canImport_{u,v}^r$ & Can node $u$ successfully import route $r$ from $v$ based on import rules.\\

    \hline
    \(canForward_{u,v}^p\) & Can node \(n\) successfully forward packet \(p\) to node \(m\) based on ACL rules. \\
 
    \hline
    
  \end{tabular}
  \caption{Router behavior variables.}
  \vspace{-1em}
  \label{tab:router behavior}
\end{table}




% We first abstract the router configuration, which controls how each routing process exchanges advertisements with neighbors and computes paths, into four Boolean \textit{router behavior variables}. 


% To automatically generate the constraints that could lead the simulation to execute to a point where the network state meets all intents. 




\subsection{Repairing The Error} \label{subsec:patch generation}

% \para{Diagnosing the errors.} 
% We diagnose the violated conditions, \ie, the given configuration does not hold, as configuration errors. The corresponding router behaviors of each condition can be mapped to the given configuration files in a systematic way. In the example, $Cond_1=false$ and $Cond_2=false$ are configuration errors, indicating that Err1 is the missing of redistribution configuration and Err2 is $r_4$ should not be preferred over $r_3$.

\para{The repair template.} 
We consider the necessary low-level configuration component that controls the corresponding high-level broken router behavior as the repair template. 
Specifically, for \(BgpPeer\) and \(RedisToBgp\) behaviors, we directly complete the neighboring (\ie, IP address, AS number, enable routing) or redistribution commands with respect to the corresponding IP/prefix. 
Other behaviors are typically governed by specific policies, \ie, import policy controls \(BgpPrefer\) and \(canImport\) behaviors, export policy controls \(canExport\) behaviors while ACL controls \(canForward\) behaviors. Each policy is defined as a set of rules structured in a match-set format to process specific routes ( ACLs are relatively simple, as they only permit or deny packets without modifying them). We use the rule with all types of matches and set actions as the repair template, then search for the specific values to complete the rule.
% Specifically, the template for repairing \(BgpPrefer\) or \(canImport\) behavior is the import policy that is responsible for 


\para{Computing the patch as a constraint-solving problem.}
Given a policy to be repaired and a set of routes/packets to be processed with it, we first add a new rule on top of the policy, symbolize each rule value, and encode the intended process result of each route/packet as a constraint-solving problem, then compute a satisfiable assignment using the SMT solver as the patch.
Figure~\ref{fig:patch constraint} shows how we encode the fix of policy M, where M controls a broken and unbroken behavior. 
In this example, assume the new rule of M must permit \(r_2\), prefer \(r_2\) over \(r_3\), and avoid matching \(r_1\). The template rule has two matches and sets local-preference, as it is a non-transitive BGP attribute. Constraint (1) ensures this rule matches first; Constraint (2) permits matched routes. Constraints (2)-(3) ensure \(r_2\) matches while \(r_3\) does not, and Constraint (5) ensures that \(r_2\) is preferred to \(r_3\). Finally, we convert the satisfiable assignment of these values, following the configuration syntax, to generate the repair patch.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/patch-solving.png}
    \caption{Encoding the repair constraints for route policy M.}
    \label{fig:patch constraint}
\end{figure}


\subsection{Supporting Complex Configuration}

\para{Handling multi-path routing.} 
Multi-path routing is a routing strategy where packet forwarding to a single destination can occur over multiple best paths with equal routing priority.
Given an equal-cost multi-path routing intent \((src, dst,n,P,equal\_path)\), where \(P=\{p_1, ...,p_n\}\).
We address this intent by extending the forwarding tree (where each node has only one next-hop) to the forwarding graph (where each node can have multiple next-hops). 
Thus, a node \(n\) could have multiple intended routes propagated along the reversed forwarding paths, suppose they are \(BEST_{p_1},...,BEST_{p_n}\), we denoted the best routes of \(n\) as \(BEST_n=BEST_{p_1} \cup ...\cup BEST_{p_n}\).
We introduce a new Boolean router behavior variable \(BgpEqualPrefer_u^{r_1,r_2}\) to indicate whether two routes are equally preferred. 
Specifically, assume routes \(r_i,r_j\) are from node \(n\)'s best next hops, and \(r_k\) is form other neighbors, we have:
\[\forall r_i\in BEST_n, \forall r_j\in BEST_n \Longrightarrow BgpEqualPrefer_{n}^{r_i,r_j}==True\]
\[\forall r_i\in BEST_n, \forall r_k\notin BEST_n \Longrightarrow BgpPrefer_{n}^{r_i,r_k}==True\]
\[\forall r_j\in BEST_n, \forall r_k\notin BEST_n \Longrightarrow BgpPrefer_{n}^{r_j,r_k}==True\]

They indicate that the routes received from the best next hops, which match the best route, should be equally preferred, and each should be preferred to any other route.


\para{Handling route aggregation.}
Route aggregation is a method of combining multiple IP prefixes into a single, larger prefix to reduce the size of the routing table and improve network efficiency. 
If a node is configured to aggregate a prefix, it only announces the aggregated route to its neighbor. 
Thus, all traffic destined for the aggregated prefix will traverse the same path from the source nodes to the aggregated node. 
When constructing the forwarding tree, we need to carefully choose the paths to the prefixes that could be aggregated for each source. 
Specifically, given two candidate path sets \(P_u^{n_1}\) and \(P_u^{n_2}\) for node \(u\) to reach networks \(n_1\) (intent 1) and \(n_2\) (intent 2), respectively, if there exists a node \(a\) that will aggregate both \(n_1\) and \(n_2\), we group the paths from the two sets based on whether the sub-path from \(u\) to \(a\) is the same. 
We remove any groups containing paths from only one intent, as these paths would conflict with those from the other intent. Only paths within the same group can be selected for constructing the forwarding trees for the two intents, ensuring sub-path consistency from the source to the aggregation node.




==> data-flow.tex <==
% \vspace{-1em}
\section{Data-Flow Diagnoser}
\label{sec:data-flow}

%We leverage data-flow analysis to diagnose observable errors. Similar to the data-flow analysis in program analysis, such an approach is very efficient in finding errors, since the data-flow execution sequence prunes the solution space.

%In this section, we first present how to generate an error execution trace from CRG and encode the trace with SMT constraints to facilitate error diagnosis, and then present algorithms for configuration error localization. Finally, we show how to explain configuration errors.

In this section, we show how to diagnose traceable configuration errors using data-flow analysis. In particular, we adopt the minimal unsatisfiable core (MUC) and interpolation approach to diagnose the error trace.
MUC is a minimal set of unsatisfiable statements that prove the unsatisfiability of the trace and the interpolation of it is a set of formulas that represent the network states that lead to the error. 
We reduce the error trace to a minimal set of statements that contribute to the error and compute the interpolation for them to provide the minimal and sound error explanation. 

% \vspace{-1em}
\subsection{Error Trace Generation}
We first generate an error execution trace from CRG. The linear execution sequence can be encoded as an execution trace with SMT constraints.
Informally, a trace is a tuple $(\pi, \phi)$ where $\pi$ is the execution sequence of the network and $\phi$ is the state formula that describes the desired output state of the trace (\ie, the requirement of the network). The execution of a trace $(\pi, \phi)$ is a conjunction of the trace formula $TF(\pi) = T_1 \wedge ... \wedge T_{n}$ where $n$ is the length of the trace. 
Let $\pi[i]$ be the $i$-th statement in the execution sequence, and $T_i$ be the corresponding transition formula.
A trace is called an error trace if $TF(\pi) \wedge \phi$ is unsatisfiable. 

We use the example in Figure \ref{fig:crg}(a) to show how to generate an error trace. The requirement is that the traffic from $T0$ to $T1$ should leave AS1 from router B (\ie, S-B-D). However, the actual forwarding path is S-A-D, which violates the requirement. 
This is because router A sets a higher local preference (\ie, 130) than that  set by router B (\ie, 120) for routes from router D. %We can apply data flow analysis to the CRG in Figure \ref{fig:crg}(b) to diagnose the error.
Figure \ref{fig:trace} shows the corresponding error trace, including route computation steps in all nodes. %and corresponding program statements.

\begin{figure}[t]
    \centering
    \includegraphics[width=242pt]{figures/trace.pdf}
    \caption{The error trace of the CRG in Figure \ref{fig:crg}. (We refer to $lp$ as local preference and $np$ as next hop)}
    \label{fig:trace}
    % \vspace{-0.1in}
\end{figure}

% \vspace{-1em}
\subsection{Configuration Error Localization}

%Given an error trace $\Phi$, there are multiple ways to diagnose the error trace in the field of program analysis. 
%We now describe our approach to diagnosing the error trace using minimal unsatisfiable core (MUC) and interpolation. 


%\para{Computing MUCs for an error trace.} 
%Given an error trace $\Phi=TF(\pi) \wedge \phi$, each $T_i$ is one or several SMT clauses which is translated from statement $\pi[i]$ and the final state $\phi$ is forwarding requirements. 
%Since the trace formula $TF(\pi)$ is always satisfiable, each MUC of $\Phi$ must involve the forwarding requirement $\phi$. 

\iffalse{
\rulan{
Each MUC represents only one of the aspects of the error, hence we need to diagnose all MUCs that include configuration-related statements for completeness.
}
}\fi
We use the classical MACRO algorithm \cite{liffiton2016fast} to compute all MUCs, each of which corresponds to one possible error root cause. The algorithm shrinks the unsatisfiable core in order and iteratively blocks up the computed MUC to enumerate all MUCs efficiently. The red rectangular in Figure \ref{fig:trace} shows an example MUC, which slices the error trace.

Another issue is how to map the MUC to the execution sequence.
%\para{Maping the MUC to execution sequence.} 
The execution sequence $\pi[1,...,n]$ is translated into the trace formula $TF(\pi)=T_1 \wedge ... \wedge T_n$. Let $T_i$ consist of a set of clauses $c_1\wedge...\wedge c_m$. We add a new boolean constraint $p_i$ to track these clauses so that we can map them to the initial statement $\pi[i]$, \ie, replacing $c_j$ with $p_i\wedge(p_i \implies c_j)$ 
%Then, the SMT formula $T_i=c_1\wedge...\wedge c_m$ is encoded as $\bigwedge \limits_{j=1,..,m} p_i\wedge(p_i \implies c_j).$

%We name the boolean constant $p$ in this format, $rc*$ is the route computation that the statement is involved in:

% \vspace{-1em}
\subsection{Configuration Error Explanation}

Given a pair of formulas $A$ and $B$ where $\neg(A\wedge B)$ holds, an interpolant~\cite{craig1957three} of $A$ and $B$ is a formula $I$ over the common symbols of $A$ and $B$ such that $A\implies I$ and $B\implies \neg I$. It indicates the inconsistency between the pair of formulas. Given an indexed sequence $\Phi=[A_i]^n_{i=1}$ such that $A_1\wedge...\wedge A_n=false$ (\eg, the execution sequence), the interpolants for $\Phi$ is a sequence $I_0, I_1,..., I_n$ which labels each $A_i$ with inconsistent variables that explain the unsatisfiablility of $\Phi$. 

We generate the error explanation for the error trace by interpolating MUC. Specifically, we compute interpolants along the MUC slice based on the hybrid algorithm \cite{murali2014gives} and preserve the dependency of specific variables (\ie, configuration-related variables), so that we can observe which configuration variables contribute to the error.

%\para{Inductive Interpolation sequence.} An interpolant for a position in an error execution trace is a formula over execution variables that captures the states that will still produce the error if the execution of the trace is continued from that position. The interpolation sequence shows the intermediate state abstractions that lead to the error. 

%\para{Computing interpolant using MUC.} Since both the MUC-based and interpolation-based approaches can get a slice of the execution path. Furthermore, the interpolation sequence can provide intermediate state abstractions along with the slice. In order to compute the minimal and sound inductive interpolation sequences efficiently, we leverage the MUCs generated from the MUC enumeration algorithm to compute interpolants based on the hybrid algorithm \cite{murali2014gives} and preserve the dependency of configuration variables. 

%\para{Localizing configuration errors from error explanation.} 
Then we localize configuration errors from the error explanation. Each interpolant in the interpolation sequence of MUC is a formula that captures the intermediate state that produces the error. Since the execution trace is a serial of route computations, interpolants can explain why an erroneous route is generated and the contributing configuration variables. The right side of Figure \ref{fig:trace} shows the error explanation of the violation of the way-pointing requirement for S (traffic from $T0$ to $T1$). First, D generates a target route to $T1$ and propagates it to peer A and B (the first red dash line box); node A then receives the route from D and selects it as the best route since A has only one route, and propagates it to peer B and S; third, B receives routes from A and D respectively and selects the route from A as the best route because of higher local preference (\ie, $bestB2.lp=130$ and $ri2.lp=120$ as the explanation). Finally, the requirement (\ie, assertion) is violated, since the requirement specifies the next hop of B must be D.  

%We filter non-configuration variables in interpolation sequence and keep the configuration-related variables that indicate the configuration lines as errors to be repaired. 

==> evaluation.tex <==
\section{Performance Evaluation}\label{sec:eval}

We implement a prototype of \system{} as a plugin of Batfish\cite{fogel2015general} in 8K LoC in Java and will open source it after publishing. 
Our experiments are performed on a Linux server with two Intel Xeon Silver 4210R 2.40GHz CPUs and 128GB of DDR4 DRAM. 
We evaluate \system{} in three dimensions: 
(1) Can \system{} diagnose and repair real configuration errors? (2) How accurate is \system{}'s error diagnosis and repair (compared to the SOTA tools)? (3) How efficiently \system{} diagnose and repair the errors?
% \todo{\system{} also works well with other simulation-based verification tools. We have made another version of \system{} adapted to a data plane verification tool from a well-known network company and its customized configuration language. \system{} successfully repairs the erroneous configurations according to the requirements in networks scale from O(10) to O(1000) while supporting customized repair (asked to conduct repair for specific devices, not importing static routes, etc.).} 





\subsection{Methodology}\label{subsec: methodology}

\para{Datasets.}
To demonstrate the soundness and correctness of the diagnosis results provided by \system{}, we conduct experiments on both Topology Zoo~\cite{knight2011internet} topologies (\ie, WAN) and fat-tree topologies (\ie, DCN). 

We use synthetic configurations with node numbers ranging from O (10) to O (100) as datasets. For Topology Zoo topologies, configurations for each network are synthesized to fulfill initial connection requirements using NetComplete \cite{el2018netcomplete}, including single-protocol (\ie, BGP, OSPF) and multi-protocol (\ie, BGP as overlay, OSPF as underlay). Additionally, we conduct single-protocol experiments on fat-tree topologies with k values ranging from 4 to 32. All configurations are written in Cisco’s IOS language.

\para{Requirements.} %The types of requirements involved in the following experiments.
Each requirement is a packet forwarding requirement for a pair of the source node $S$ to reach the destination $D$ via a path represented by a regular expression. %According to experience, 
Common requirements include: 1) reachability, \ie, $(S, D, n, S*D, k)$, 2) way-point, \ie, $(S, D, n, S*W*D, k)$, where $W$ represents the way-point nodes, 3) bypass, \ie, $(S, D, n, S*\neg B*D, k)$, where $B$ represents the bypass nodes. To check the capability of \system{} to support the $k$-link failure scenario, we also give some requirements with $k>0$.
%can still provide reliable services in the event of link failures, we also give some reachability requirements under the $k$-link failure scenarios.
%it is critical to consider the $k$-link failure scenario. Therefore, we've
%% design and implement support for k-failure requirements. Also, in the single protocol scenario, we do experiments to address the reachability 
%given some reachability requirements under the $k$-link failure scenarios.

\para{Configuration errors.} 
To demonstrate that \system{} can accurately diagnose and localize configuration errors, we need erroneous network configurations along with predefined network requirements. Given that errors in actual network configurations are often undisclosed, obtaining real erroneous configurations is impractical. Therefore, we adopt a method of randomly injecting errors into the correct configurations to generate erroneous network configurations. 
Drawing on our collaborative experience with a well-known network company and considering the protocol properties, we design a series of errors.

\begin{figure*}[t]
\setlength{\abovecaptionskip}{-0em}
\setlength{\belowcaptionskip}{-0cm}
    \centering
    % \begin{minipage}{0.98\linewidth}
        %\input{green-evaluation}
        %\input{incremental-evaluation}
	\centering
            \begin{subfigure}{0.495\linewidth}
        	   \setlength{\abovecaptionskip}{0cm}
                \setlength{\belowcaptionskip}{-0.cm}
     		\centering\includegraphics[width=\linewidth]{figures/BGP-Topology_zoo-Bar.pdf}
            	\caption{\label{fig:BGP-Topology_zoo-Bar}\footnotesize Topology Zoo topologies in the single-protocol scenario.}
        	\end{subfigure}
         \begin{subfigure}{0.495\linewidth}
        	   \setlength{\abovecaptionskip}{0cm}
                \setlength{\belowcaptionskip}{-0.cm}
     		\centering\includegraphics[width=\linewidth]{figures/BGP-Topology_zoo-Bar_k-failure.pdf}
            \caption{\label{fig:K-failure-Topology_zoo-Bar}\footnotesize Topology Zoo topologies under fault-tolerance scenario.}
            \end{subfigure}
     
    	\begin{subfigure}{0.495\linewidth}
    	   \setlength{\abovecaptionskip}{0cm}
            \setlength{\belowcaptionskip}{-0.cm}
 		\centering\includegraphics[width=\linewidth]{figures/BGP-Fattree-Bar_1.pdf}
        	\caption{\label{fig:BGP-fattree-Bar}\footnotesize Fat-tree topologies in the single-protocol scenario.}
    	\end{subfigure}
     \begin{subfigure}{0.495\linewidth}
    	   \setlength{\abovecaptionskip}{0cm}
            \setlength{\belowcaptionskip}{-0.cm}
 		\centering\includegraphics[width=\linewidth]{figures/BGP-Fattree-Bar_k-failure.pdf}
        \caption{\label{fig:K-failure-fattree-Bar}\footnotesize Fat-tree topologies under the fault-tolerance scenario.}
    	\end{subfigure}
     
    \caption{End-to-end performance of \system{} in the single-protocol and fault-tolerance scenarios.}
    % \end{minipage}
\end{figure*}

For OSPF, we focus on neighbor's establishment and link costs. 
% For OSPF, we use neighbors' establishment and link cost commands. 
For BGP, we categorize errors into four types. 
1)\textit{ Redistribution error}. This type of error eventually causes the route not to originate. We mainly consider the redistribution from static and connected routes to BGP, such as no redistribution command, invalid static route command, etc.
%Some cases can lead to this type of error, 
2)\textit{ Missing peer error}. It means there are invalid or no peer relationship commands in the configurations. 
3)\textit{ Route sending or receiving error}. This type of error includes the filter command in the route import/export policy, no route reflector command (for iBGP), etc. 
4)\textit{ Route preference error}. This type of error specifically pertains to way-point or bypass requirements. In the following experiments, we mainly use the local preference command. 
%We introduce this kind of error by modifying the local preference. 
%And we inject errors for these two properties.

% During experiments, we randomly inject one or several types of errors and then run \system{} for diagnosis and repair.

\para{Metrics.} We evaluate the performance of \system{} in terms of correctness, efficiency, and scalability.

There is always more than one repair solution for a network requirement violation. For \emph{correctness}, if the network meets the requirements after modifying the configuration according to \system{}'s repair solution, we assume the diagnosis and repair results are correct. We also record the number of modified configuration lines and compute the modified ratio of configurations.
% to argue \system{} can pinpoint the root cause of the error
% In all simulations, \system{} successfully diagnoses and repairs all errors in the networks. 
%We posit that the result is correct if the repaired configuration satisfies the network requirements. 
For \emph{efficiency}, we record the simulation time with and without diagnosing and repairing. Since the first round of simulation (for verification) is unavoidable, we focus more on the second round of simulation, the actual overhead of diagnosis and repair. 
By recording \system{}'s runtime in various topological scales and error scenarios, we can gain insights into \system{}'s performance when dealing with large-scale networks and intricate configurations.
% The results show that for all networks in the datasets, \system{} can finish diagnosing \textbf{within one minute}. 
For \emph{scalability}, we extend topologies to larger scales to run stress tests on \system{}. By conducting experiments on large-scale topologies, we ensure that \system{} can continue to deliver reliable and efficient services, even in a network with a scale of O(1000).
% The experiment results illustrate that \system{} can provide reliable and efficient services, even in a network with a scale of O(1000).





\subsection{Functionality Demonstrations}\label{subsec: demonstration}

We build a network of 7 routers in Figure \ref{fig: multi-protocol example} and synthesize configurations written in Cisco's language for each router. As mentioned in \S\ref{subsection: BGP in multi-protocol}, there are four ASes in the network connected with BGP. Routers in each AS use OSPF to connect. Subnet \textit{n} in AS 4 is the destination in the network requirements. We input the network to \system{} with different requirements: 1) reachability from S to the subnet \textit{n}, 2) reachability with a way-point node $C_{4}$ from S to the subnet \textit{n}, and 3) reachability from S to the subnet \textit{n} under 1 link failure. For each requirement, \system{} always outputs the right diagnose result and returns the fixed configurations. We also provide a functional demo on \cite{demo-2024}.

\begin{figure*}[t]
    \centering
	\begin{subfigure}[t]{0.495\textwidth}
	    \centering\includegraphics[width=\linewidth]{figures/Fattree-Topology-CDF.pdf}
		\caption{\label{fig:Fattree-Topology-zoo-CDF} Overhead in non-fault-tolerant scenarios.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.495\textwidth}
	    \centering\includegraphics[width=\linewidth]{figures/Fattree-Topology-CDF_K.pdf}
		\caption{\label{fig:Fattree-Topology-zoo-CDF(K)} Overhead in fault-tolerant scenarios. }

	\end{subfigure}
    \caption{Diagnosis and repair overhead of \system{}.}
    % \vspace{-1em}
\end{figure*}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Multi-protocol-Bar.pdf}
    \caption{Real network topologies' simulation time in the multi-protocol scenario.}
    \label{fig:Multi-protocol-Bar}
    % \vspace{-1em}
\end{figure} 

\subsection{Experiment Results}\label{subsec: results}

We conduct an extensive set of experiments using 8 topologies from Topology Zoo (4 with the scale of O(10) and another 4 with O(100)), as well as fat-tree topologies ($k$ values ranging from 4 to 32). Initially, we provide some predefined requirements for each network. Then, we randomly inject one or more types of errors into the correct configurations of each network. To ensure that the introduced errors could violate the requirements, each type of error could also be injected at multiple locations. We perform experiments in the single-protocol scenario, the multi-protocol scenario, and the k-failure scenario. We also conduct the stress tests. 
%, as described earlier
%and give the result in the end.
%, evaluating the results of each experiment

\subsubsection{Single-protocol scenario results.}

%The scenario with only the BGP protocol is first considered. 
We only consider the BGP protocol.
For topologies in the Topology Zoo, we predefine some requirements for both reachability and way-point. 
Since redundancy (\ie, multiple paths) is a major advantage of the fat-tree network, the way-point requirements are meaningless. Therefore, for fat-tree topologies, we have only predefined the reachability requirements.

%\system{} is employed to provide the final repair solution to operators. 
Figure \ref{fig: repair result} illustrates an example of the \system{}'s output. In this context, the \textit{LineNumber} denotes the specific location of the command in the configuration file, and the \textit{Command} is the precise content of the configurations. The $+$ or $-$ indicates the addition or deletion of the command, respectively.
% Figure \ref{} illustrates the final repair results.
% 缺：修复结果表述!!!


\begin{table*}[t]
  \centering
  \begin{tabular}{c}
    \includegraphics[width=\linewidth]{figures/result_table.pdf}
  \end{tabular}
  \caption{Detailed statistics of experiment results.}
  \label{tab: result statistics table}
\end{table*}

% correctness
\para{Correctness.} For all erroneous configurations, \system{} can always provide correct guidance for repairing. Meanwhile, the number of modified lines is small (less than 1.5\%), indicating that \system{} could repair networks on a small scale. However, we also observe that, for errors caused by route policies, not all diagnosis results match exactly the errors we injected. This is because route policies are also presented in the original correct configurations. Given that, there may be multiple viable paths in the network for the same source and destination node pair, leading to various repair solutions. However, \system{} only provides one repair solution, leading to inconsistencies with the injected errors.

%efficiency
\para{Efficiency.} We record the diagnosis and repair time for each network to evaluate the efficiency of \system{}. Figure \ref{fig:BGP-Topology_zoo-Bar} and \ref{fig:BGP-fattree-Bar} show the results in Topology Zoo and fat-tree topologies, respectively. 
% In the 8 topologies of Topology Zoo, the scale of the first four topologies is O(10), while the scale of the last four topologies is O(100). 
In the figures, the first column for each network represents the time required to run Batfish to verify the configuration (\ie, only performing a single round simulation). The next columns represent the time required for \system{} to diagnose and repair a typical kind of requirement. Each column consists of two parts because \system{} needs to simulate the network twice. The first round is to compute the initial data plane, and the second round is to perform the selective symbolic simulation for diagnosing and repairing. 
% Since way-point requirements involve path comparison and selection, which are not involved in reachability requirements, for topologies from the Topology Zoo, we separately recorded the time required for reachability and way-point requirements. 
%bar
The figures show that with the increase of network scale, the end-to-end time increases accordingly, but the increase is not significant. 

Furthermore, for all topologies in the experiment, the first simulation time is almost the same as the time required for running Batfish directly. Minor differences mainly arise from the difficulty of maintaining identical running environments at different times. The second simulation time is generally much less than the first simulation time, because it can reuse the data plane information generated in the first simulation. For 75\% of cases, the second simulation time constitutes less than 40\% of the total time. In the large-scale fat-tree topologies, the second simulation time significantly increases. This is due to errors in the configurations causing many flows to be unreachable. Consequently, compared to the first simulation, the second simulation involves more source-to-destination pairs. Additionally, the fat-tree topologies are dense. So there is a substantial difference in the simulation time between the two runs.
%CDF
Figure \ref{fig:Fattree-Topology-zoo-CDF} shows that for 80\% of cases, the overhead of diagnosing and repairing is within 1500 ms. For 87\% of cases, the overhead is within 10 s. In the worst case, it finishes no more than 5 min.
%, and for all networks (including reachability and waypoint requirements), the whole process could end up in $\leq$ 4400 ms. 
% The CDF of execution time for the fat-tree topologies is shown in Figure \ref{fig:BGP-Fattree-CDF}. In 80\% of cases, the completion time is within 18 seconds. 


%summary
%To summarize, in the single-protocol scenario, \system{} demonstrates correctness and great efficiency.

\subsubsection{Multi-protocol scenario results.}

After collecting real erroneous networks from a well-known network provider, we translate their configurations into Cisco's language and conduct experiments in the multi-protocol scenario. We inject both BGP and OSPF errors into each topology and run \system{} to diagnose and repair errors.

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=220pt]{figures/Fattree-Topology-CDF.png}
%     \caption{Diagnosis and repair overhead (single protocol).}
%     \label{fig:Fattree-Topology-zoo-CDF}
%     % \vspace{-1em}
% \end{figure} 

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=220pt]{figures/Fattree-Topology-CDF(K).png}
%     \caption{Diagnosis and repair time overhead (k-failure).}
%     \label{fig:Fattree-Topology-zoo-CDF(K)}
%     % \vspace{-1em}
% \end{figure} 


\para{Correctness.}
The result in Table \ref{tab: result statistics table} shows that \system{} can successfully diagnose and repair errors for all cases. Meanwhile, the repaired configurations satisfy the requirements. %The details are presented in Table \ref{tab: result statistics table}.

\para{Efficiency.}
Because of the decoupling of various protocols, we need to run the simulation three times for both BGP and IGP. The extra simulation overhead is due to diagnosing and repairing IGP requirements. Simulation time is shown in Figure \ref{fig:Multi-protocol-Bar}. Despite the extra simulation time, system overhead remains below 57\% of the entire process. The overhead of the best case (36 nodes) is 2177 ms. Even in a network scale of O(100), \system{} can finish the diagnosis and repair process in $\leq$ 10 s.

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=220pt]{figures/BGP-Topology_zoo-Bar.pdf}
%     \caption{The real topologies' simulation time with and without diagnosing and repairing in the single protocol scenario.}
%     \label{fig:BGP-Topology_zoo-Bar}
%     % \vspace{-1em}
% \end{figure} 

% \begin{figure}[th]
%     \centering
%     \includegraphics[width =200pt]{figures/BGP-Topology_zoo-CDF.pdf}
%     \caption{Diagnosis and repair time of real topologies.}
%     \label{fig:BGP-Topology_zoo-CDF}
%     % \vspace{-1em}
% \end{figure} 

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=220pt]{figures/BGP-Fattree-Bar.png}
%     \caption{The fat-tree topologies' simulation time with and without diagnosing and repairing in the single protocol scenario.}
%     \label{fig:BGP-fattree-Bar}
%     % \vspace{-1em}
% \end{figure} 

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=200pt]{figures/BGP-Fattree-CDF.pdf}
%     \caption{Diagnosis and repair time of fat-tree topologies.}
%     \label{fig:BGP-Fattree-CDF}
%     % \vspace{-1em}
% \end{figure} 



\subsubsection{K-link failure scenario results.} 

Building upon the foundation of error configurations and reachability requirements in the single-protocol scenario, we further add $k$-link failure requirements ($k$ = 1) to validate \system{}'s capability to handle the fault-tolerant scenario. %Subsequently, we evaluate \system{}'s performance in the k-link failure scenario (k = 1).

\para{Correctness.} 
The repair results for each topology are summarized in Table \ref{tab: result statistics table}. Similarly, for all topologies, \system{}'s repair solutions ensure the networks meet the requirements while inducing a few changes to the configurations.

\para{Efficiency.}
Figure \ref{fig:K-failure-Topology_zoo-Bar} and Figure \ref{fig:K-failure-fattree-Bar} show the time required for diagnosing and repairing in the $k$-link failure scenario. The overall trend is similar to the non-link failure scenario in the single-protocol case. Although multiple route propagation paths need to be computed in this scenario, it does not incur much additional overhead. In some cases, the second simulation time is even less than the non-link failure scenario. For 75\% of the cases, the second simulation time is less than 45\% of the total time. In the worst case, it does not exceed 87\%.
%要不要把topology zoo和fattree的数据合起来画一张CDF
The overhead of \system{} is shown in Figure \ref{fig:Fattree-Topology-zoo-CDF(K)}. For 66.7\% of the cases, \system{} finishes the tasks within 1000 ms. For 73.3\% of the cases, the time is within 2500 ms. In the worst case, the time takes about 5 min.

%That means, in the k-failure scenario, \system{} can also guarantee the correctness of results and has high efficiency.

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=220pt]{figures/BGP-Topology_zoo-Bar(k-failure).pdf}
%     \caption{The real topologies' simulation time with and without diagnosing and repairing in the k-failure scenario.}
%     \label{fig:K-failure-Topology_zoo-Bar}
%     % \vspace{-1em}
% \end{figure} 

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=200pt]{figures/BGP-Topology_zoo-CDF(k-failure).pdf}
%     \caption{Diagnosis and repair time of real topologies.}
%     \label{fig:K-failure-Topology_zoo-CDF}
%     % \vspace{-1em}
% \end{figure} 

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=220pt]{figures/BGP-Fattree-Bar(k-failure).png}
%     \caption{The fat-tree topologies' simulation time with and without diagnosing and repairing in the k-failure scenario.}
%     \label{fig:K-failure-fattree-Bar}
%     % \vspace{-1em}
% \end{figure} 

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=200pt]{figures/BGP-Fattree-CDF(k-failure).pdf}
%     \caption{Diagnosis and repair time of fat-tree topologies.}
%     \label{fig:K-failure-Fattree-CDF}
%     % \vspace{-1em}
% \end{figure} 





\subsubsection{Stress tests.}

To validate the scalability of \system{}, we conducted stress tests using two real network topologies of the O(1000) scale. 
The results are also shown in Table \ref{tab: result statistics table}. As for efficiency, \system{} can finish diagnosing and repairing tasks in minutes. 
The 1006 nodes' topology needs 13 min to diagnose and repair while 12 min for the first simulation. The 1306 nodes' overhead is 19.8 min while 18.6 min for the first simulation.
The findings suggest that even when dealing with a network of such a large scale, \system{} still maintains high efficiency while ensuring correctness.

%In summary, \system{} can guarantee correctness and has high efficiency in diagnosing and repairing across various scenarios, regardless of the network scale.
% performs well





==> introduction.tex <==
% \vspace{-0.6em}

\section{Introduction}

Network configuration verification tools~\cite{feamster2005detecting, fayaz2016efficient, fogel2015general, beckett2017general,gember2016fast,beckett2018control,beckett2019abstract,giannarakis2019efficient,ye2020accuracy,abhashkumar2020tiramisu,zhang2022dna,liu2017crystalnet,lopes2019fast,zhang2022symbolic, brown2023batfish, fang2024network, xu2024relational, wang2024expresso, li2024general} analyze the configuration of network devices to verify whether they would compute invariant conforming (\eg, reachability, blackhole freeness, and loop freeness) forwarding rules. Once they find that the configurations are incorrect, it is up to the operators to manually find which parts are erroneous and fix them, which is time-consuming and error-prone. For example, given a set of incorrect configurations, Minesweeper~\cite{beckett2017general} returns
one counterexample, but fixing these configurations, in the worst case, requires finding all possible counterexamples, which is NP-complete.



Existing studies treat the diagnosis and repair of network configurations as separate issues and propose point solutions with different limitations.
NetCov~\cite{xu2023test} can automatically find all related configurations for a set of given routes using the information flow graph, but it cannot address unobservable events.
Data provenance-based tools~\cite{zhou2010efficient, chen2018data, loo2009declarative, wu2014diagnosing, wu2017automated} diagnoses both observable and unobservable events by analyzing the relationship among events in the network to find the root causes (\eg, link failures) of network behaviors (\eg, updates of forwarding rules). However, they are built on declarative networking languages (e.g., NDLog [27]), which introduces additional slow learning curves for users to re-implement routing protocols in these tools.

CPR \cite{gember2017automatically} repairs the configuration based on an abstract representation of the control plane, but it cannot handle BGP announcements due to the use of the graph-based abstraction. CEL~\cite{gember2022localizing} extends Minesweeper's SMT-based configuration verification formulation and localizes the formula's minimal correction set (\ie, a subset of constraints whose removal would allow the remaining constraints to be satisfied) as the errors. However, it is a black box with rare hints about the relationship between routes and configuration to users, which is important for operating real networks. Moreover, it cannot support AS-path filter configurations due to the path encoding explosion issue of the SMT-based formulation. 
Campion \cite{tang2021campion} focuses on finding the differences between two given configurations of one router, 
SelfStarter~\cite{kakarla2020finding} and Diffy~\cite{kakarla2024diffy} find potential configuration errors by detecting the outlier among a set of configurations. They do not work for single network configurations.
Configuration synthesis tools (\eg, \cite{ abhashkumar2020aed, el2018netcomplete}) automatically generate new configurations to patch erroneous configurations without a diagnosis, making it difficult for operators to understand and reason about the patches. 




\para{Proposal: selectively and symbolically simulating variants of the given configuration can help us find an intent-compliant variant, which enables configuration error diagnosis and repair.}
% Logic Bug Detection and Localization Using Symbolic Quick Error Detection
% SemFix: Program repair via semantic analysis
% SOSRepair: Expressive Semantic Search for Real-World Program Repair
% On test repair using symbolic execution
Symbolic execution~\cite{king1976symbolic} provides a systematic way to analyze multiple execution paths at a time to localize and repair program errors~\cite{singh2018logic,nguyen2013semfix,afzal2019sosrepair,daniel2010testrepair} by exploring program behaviors under varying inputs and conditions. 
We believe it is feasible to diagnose and repair network configuration errors, as the simulation is also a program that takes the configuration as input.
Symbolically simulating all configuration variants to find an intent-compliant variant is equivalent to general configuration synthesis, which is NP-hard~\cite{schneider2022complexity}.
So we turn to selective symbolic simulation~\cite{chipounov2009selective} to narrow down the search space, \ie, simulate only the configuration variants of interest, to quickly find an intent-compliant variant, and differences between the founded intent-compliant configuration and the given configuration can point to configuration errors and potential patches.
Hoyan~\cite{ye2020accuracy} and Expresso~\cite{wang2024expresso} can be seen as special cases of \system{} that perform selective symbolic simulation on the link up/down configuration and external route configuration, respectively.  


While a previous position paper by Yang et al. \cite{yang2023diagnosing} also suggests the promise of diagnosing and repairing distributed routing configuration using symbolic simulation, it fell short in several important aspects, including 1) diagnosing and repairing non-vector-based routing protocols, 2) handling the network where multiple routing protocols co-exist, and 3) diagnosing and repairing the fault-tolerance errors of the network. To this end, we design \system{}, a companion of simulation-based configuration verification tools (\eg, \cite{fogel2015general, brown2023batfish, lopes2019fast, quoitin2005modeling, liu2017crystalnet}) that automatically diagnose and repair distributed routing configurations with four key designs (D1-D3):




\para{D1. Simulating network configuration variants selectively and symbolically (\S\ref{sec: sss}).}  
To explore configuration variations efficiently, 
we introduce the \textit{route propagation graph} (RPG) to help select the appropriate portion of the configuration for symbolic simulation.
The PRG, generated from forwarding requirements and the concrete simulation, is an abstract representation that indicates how route propagation processes form an intent-compliant forwarding graph.
We then simulate the route propagation process to achieve the RPG symbolically.
The simulation will ultimately form the forwarding graph as the RPG guides. 
Thus, we can derive a set of conditions that an intended configuration variant must hold, which helps us diagnose and repair the configuration error.


\para{D2. Supporting for multiple routing protocol networks (\S\ref{multi-protocol section}).} Modern networks are often layered (\ie, underlay and overlay) and use multiple routing protocols (\eg, OSPF and BGP).  
These protocols could interact or depend on each other. To address this, we take a layered approach: First, we generate the route propagation graph for the overlay network and perform selective symbolic simulation on it to diagnose overlay network configuration errors and get sub-requirements for the underlay network. Then, we diagnose the underlay network for the sub-requirements. 


\para{D3. Tolerating k-link failure requirements (\S\ref{k-failure section}).} %Fault tolerance is an important feature of operating networks. 
To diagnose and repair configuration errors for $k$-link failure tolerance requirements, we generate a fault-tolerant route propagation graph by computing k+1 edge-disjoint paths for each requirement. We then selectively and symbolically simulate both configurations and failure scenarios to find a variant that is always intent-compliant under arbitrary k-link failures. 

\para{Evaluation results (\S\ref{sec:eval}).} 
We implement a close-source version of \system{} for a major vendor as a plug-in of its in-house simulator. We also implement an open-source version as a plugin of Batfish~\cite{fogel2015general} and will make it available upon the publication of the paper. We evaluate its performance extensively and provide a set of demos~\cite{demo-2024}. 
%, a widely-used simulation-based configuration verification tool. to study its capability, performance, and overhead %using synthetic network configurations 
We evaluate \system{} on both X(num.) production network configurations from XX(provider) and $O(10)$ to $O(1000)$ synthetic real-network configurations.
Results show that \system{} finishes accurate configuration diagnosis and repair in 1) all WAN configurations within 10 s and 2) all DCN configurations within 20 minutes. \rulan{need to update}











==> k-failure_diagnosis.tex <==



\section{Tolerating K-link Failure}
\label{sec:k-failure}
The K-link failure tolerance refers to the ability to work correctly even after arbitrary \(k\) links fail.
A naive approach would be to compute a reference data plane for each potential failure scenario to diagnose the error. 
However, as \(k\) increases, the number of failure scenarios grows exponentially, making this approach significantly time-consuming.


% We achieve the k-link failure tolerance diagnosis by generating a fault-tolerant forwarding graph to execute the symbolic data plane computation.

\subsection{Key Ideas}
\label{subsec: 7.1}

Our key idea is to construct a fault-tolerant forwarding graph where multiple potential paths exist for forwarding traffic under link failure(s). 
Specifically, we compute $(k+1)$ edge-disjoint paths for each k-link failure tolerance intent. Any two paths are edge-disjoint means that the edges of them do not intersect.
We also proved that:


\begin{proposition}
    Given a fault-tolerant intent $req=(src, dst, n, P, fail \le k), k>0$. If the packet from $src$ to $dst$ with prefix $n$ can be forwarded through the $(k+1)$ edge-disjoint paths $p_1, ..., p_{k+1}$, there must exist at least one path to forward the packet under an arbitrary k-link failure.
\end{proposition} 

\begin{proof}
    Since these paths are edge-disjoint, each link failure results in, at most, one path failing to forward the packet. According to the Pigeonhole Principle, at least one path must exist to forward the packet when $k$ links fail.
\end{proof}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/k-fail.png}
    % \includegraphics[width=\linewidth]{figures/scalpel-sigcomm24-example-multiproc-new.pdf}
    \caption{An example network to diagnose and repair errors for $k$-link failure tolerance ($k$=1).}
    \label{fig: k-fail example}
    \vspace{-1em}
\end{figure} 

\subsection{Detailed Steps}
We use the same topology in Figure~\ref{fig:multiproc-DP} to demonstrate the K-link failure tolerance diagnosis. 
In this network, 
The intent is that all the routers can reach the prefix $p$ under arbitrary one-link failure.
When there is no link failure, or a link such as $l_{AB}, l_{FE}$ fails, the intent is still satisfied. 
However, if link $l_{BE}$ fails, 



\para{The fault-tolerant forwarding graph.}
We now support the automatic construction of a fault-tolerant forwarding graph for: (1) multiple failure tolerance intents, using only full-match path regular expressions that start from their sources and end at the destination (\ie, reachable via any simple paths), or (2) a single failure tolerance intent with an arbitrary path regular expression. 

To construct the type (1) graph, we compute \(k+1\) edge-disjoint paths for each \(k\)-link failure intent individually and then combine them into a single forwarding graph. Path conflicts are not a concern, as each intent can be satisfied by any simple path. Edge-disjoint paths are computed by iteratively traversing the topology using DFS: each time a feasible path is found, we remove its edges and proceed with the next traversal. 
To construct the type (2) graph, we first compute all compliant paths by constructing the product graph for the given intent. Suppose there are \(n\) paths, and the intent requires \(k\)-link failure tolerance. We then select \(k+1\) edge-disjoint paths from these \(n\) paths (\(C_n^{k+1}\)) to build the fault-tolerant forwarding graph.

In this example, we compute the edge-disjoint paths \(SAD\) and \(SBCD\) for \(S\)'s intent, and \(BAD\) and \(BCD\) for \(B\)'s intent. These paths are then aggregated to form the forwarding graph, as illustrated by the green lines in Figure~\ref{fig: k-fail example}.


\para{The fault-tolerance constraints.}
Similar to multi-path routing, the intended best routes of each node are the union of the routes propagated along all reversed forwarding paths (but they do not need to have equal costs).
In the fault-tolerant forwarding graph, each node can have multiple best hops, but only one best hop is allowed for forwarding traffic in a given failure scenario.
However, we do not need to specify which path (or which next hop) is most preferred for each scenario, as all paths are intended, and the routing protocol's path selection algorithm will ultimately choose one of them under a specific scenario.
Therefore, we still add \(BgpPrefer\) constraints to the route selection process to ensure the intended best routes received from the best next hops are selected. However, we do not apply such constraints between routes received from different best next hops. 

The top of Figure~\ref{fig: k-fail example} shows all constraints of node \(B\). Its \(BgpPrefer\) constraints \(c_7\) and \(c_8\) indicate that the route \(r_4\) (\(r_5\)) from the best next hop \(A\) (\(C\)) should be preferred to the route \(r_{11}\) from the non-best next hop \(S\). However, there are no constraints specifying whether \(r_4\) should be preferred to \(r_5\) or \(r_5\) should be preferred to \(r_4\).


\para{Simulating the fault-tolerant network.}
To simulate all potential router behaviors under any failure scenario, we propagate all selected routes rather than just one. 
For example, \(B\) received \(r_4\) and \(r_5\) from \(A, C\), and will select both of them as best routes and send them to \(A\) (getting \(r_6\)) and \(S\) (getting \(r_8\) and \(r_9\)). 
Then, \(S\) selects its best routes as \(r_7\) (from \(A\)) and \(r_9\) (from \(B\)). 
\(S\) selects \(r_9\) rather than \(r_8\) because only \(r_9\) is propagated along the intended path \(SBCD\) reversely.
Next, \(S\) sends \(r_7\) and \(r_9\) to \(A\) (getting \(r_{10}\)) and \(B\) (\(r_{11}\)), respectively. 
Before that, when simulating to the point where \(B\) needs to determine whether to import \(r_4\) from \(C\), the actual behavior is dropping \(r_4\) (going to the "false" branch), which breaks constraint \(c_3\). Therefore, we force the simulation to go to the "true" branch as guided by \(c_3\), revealing that it is a configuration error.



==> motivation-v2.tex <==
%\section{Overview}\label{sec:back}
%In this section, we first demonstrate the limitations of related tools through an
%experiment in a simple network~(\S\ref{sec:limitations}).  We then illustrate
%the key insight and basic workflow of how \system{} diagnoses and repairs
%an erroneous configuration using the same network as an
%example~(\S\ref{sec:workflow}).


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/revise-example.pdf}
    \caption{The example network.}
    \label{fig:example}
    % \vspace{-1em}
\end{figure*}

% To better understand the gap in approaches for network configuration diagnosis and repair, we first demonstrate the limitations of existing tools with an example and then outline the key challenges.

\section{Why Existing Tools Do Not Work}\label{sec:limitations}
In this section, we demonstrate the limitations of related tools through an
experiment in a simple network. The screenshots of outputs of all our experiments
are in Appendix~\ref{appendix}.
% (a) is the actual forwarding paths computed by the simulation tool (\eg,
% Batfish~\cite{fogel2015general}). (b) shows the configuration snippets of B
% and C, including the peer session establishment and the peer policy applied to
% specific neighbor(s) towards a specific direction.

\para{An example network.} 
Consider a small network of six routers running BGP in Figure~\ref{fig:example}.
For simplicity, we use the ID of routers as their AS numbers. The destination IP
prefix $p$ is at router $D$.  The intents of the operator are: (1) all the
routers can reach prefix $p$; (2) the path of router $A$ must waypoint router
$W$; and (3) the path of router $F$ must avoid router $W$. All the routers use
the default BGP configuration except for the snippets of router $A$ and $F$
in the figure, where $A$ discards all route announcements with an AS-path
containing $W$, and $F$ sets a higher local preference for announcements it
receives from $A$ over the ones from $E$. Because it is such a small network, we
can simulate its execution on paper and observe that while all the routers can reach
prefix $p$, the path of $A$ does not satisfy intent 2.

\para{Errors in the configuration: the ground truth.}
There are two errors in the configuration. 
One may quickly observe that one is the import policy at $A$ that discards
all AS paths consisting of $W$. However, removing it only partially fix the
configuration. For example, if $A$ removes this policy, it will prefer $[A, B,
W, D]$ over $[A, F, E, D]$ as its path to reach $p$ because $B$ has a lower ID
than $F$. But $F$ will also switch to path $[F, A, B, W, D]$ because it has
another policy to prefer $A$ over $E$ as the next hop. Therefore, router $F$'s
policy to prefer $A$ over $E$ is also an error, and needs to be removed.


\iffalse{
This is because \(A\) is mistakenly configured to deny the route of path
$[A,B,W,D]$.  However, fixing it does not fully resolve the issue. Though \(A\)
will select \([A, B, W, D]\) as the best path (it is preferred due to the lower
router ID) after correcting this error, \(F\) will then receive and select it as
its best path, causing a violation of intent 2, which reveals that \(F\) setting
a higher preference for $A$ over $E$ is also a configuration error (\ie, the
latent error).
}\fi

\para{Outputs of representative configuration verification/diagnosis/repair tools.}
We select five recent tools to examine the configuration of this small network
against the three intents. To make sure the experiment is fair, we use the
open-source prototypes from the authors. We find that although some of them can
determine the configuration is incorrect, none of them can tell which part of
the configuration is wrong or repair it.

\para{Batfish~\cite{fogel2015general, brown2023batfish} correctly determines the
configuration is erroneous.} As a simulation-based verification tool, Batfish
can correctly compute the paths of each router based on their configurations,
and alert us that these paths violate intent 2 (Figure~\ref{fig:Batfish-output} in Appendix~\ref{appendix}).  However, it does not tell
us where the configuration is wrong, nor suggest any repair.

\para{Minesweeper~\cite{beckett2017general} determines the configuration is
erroneous for the wrong reason.} As an SMT-based verification tool, Minesweeper
also alerts us that the configuration is erroneous and provides a counter
example (Figure~\ref{fig:MS-output} in Appendix~\ref{appendix}).  However, this
counter suggests there is no route at router $A$, which is wrong. It is because
router $A$ has a route policy based on AS path, but it Minesweeper does not
encode AS path or any AS path based route policy in the SMT formula 
to avoid path explosion, resulting an incorrect formula.

\para{CEL~\cite{gember2022localizing} cannot find any error.} CEL analyzes the
configuration SMT formula constructed by Minesweeper and computes its minimal
correction set (MCS) as the errors. However, to our surprise, it reports an
empty MCS (Figure~\ref{fig:CEL-output} in Appendix~\ref{appendix}). This is also due to the lack of AS path encoding in the SMT formula.

\para{CPR~\cite{gember2017automatically} thinks there is no error in the
configuration.} CPR uses an abstract representation to model the network
configuration and finds the repair using constraint programming. Unfortunately,
in this experiment, it reports that there is no error in the configuration (Figure~\ref{fig:CPR-output} in Appendix~\ref{appendix}). This is because the
model of CPR does not support the modeling of local preference related
configurations like the ones used in router $F$. 

\para{ACR~\cite{acr-hotnets24} cannot locate or repair any error in the configuration due
to missing candidates lines.} ACR adopts a trial-and-error approach. In each
iteration, it applies a spectrum-based method to rank potential
erroneous lines, tries to repair them using an experience-based method, and
validate the repair using simulation-based tools (\eg, Batfish). Although it
does not have an open-source prototype, it suggests that it uses a configuration
test coverage tool (\ie, NetCov~\cite{xu2023test}) to first identify some
configuration lines related to the errors as candidates. Therefore, we
implement ACR by ourselves with NetCov as a key component. In this example,
however, when we sends NetCov a test case of path from $A$ to $D$, the candidate
lines NetCov returns does not include any route policies at $A$ or $F$ (Figure~\ref{fig:netcov-output} in Appendix~\ref{appendix}), the
actual errors in the network. As a result, ACR
declares that it cannot locate or repair the configuration after repeating the
trial-and-errors multiples times. 

\para{Takeaway: an accurate tool for configuration diagnosis and repair is still
missing.} Representative existing tools have different limitations,
making it difficult for them to locate or repair the configuration errors in a
simple network with simple configurations.



\iffalse{
We tested various existing tools and found that none of them can accurately
diagnose and repair configuration errors, even in this simple network.  Appendix
\ref{appendix} shows the outputs of all these tools.  Configuration verification
tools (\eg, Batfish~\cite{fogel2015general, brown2023batfish} and
Minesweeper~\cite{beckett2017general}) will alert that configurations cannot
satisfy the intent with some limited auxiliary information (\eg, the resulting
data plane in Figure~\ref{fig:Batfish-output} or a counterexample in
Figure~\ref{fig:MS-output}).  However, we still do not know how to fix the
configuration errors. If there are latent errors, fixing all of them is even
more difficult and time-consuming.

Configuration diagnosis and repair tools either failed to pinpoint the errors or
produced false positives.  CEL~\cite{gember2022localizing} did not compute the
minimal correction set (MCS) that can help localize the erroneous configuration
snippets (Figure~\ref{fig:CEL-output}).  This is because CEL did not correctly
model the configuration semantics (AS path filter).
CPR~\cite{gember2017automatically} found no errors in this network
(Figure~\ref{fig:CPR-output}), and will not continue repairing the errors.
ACR~\cite{acr-hotnets24} missed the real errors despite numerous attempts due to
the coverage testing tools it relies on failing to identify the erroneous
configuration lines as the repair candidates. Figure~\ref{fig:netcov-output}
shows NetCov's output, which did not hit both $A$'s neighboring configuration
with $F$ and also its import policy.
}\fi



\iffalse{ 
$A$ is configured to deny routes (lines 3-4) whose AS\_PATH contains $W$\footnote{we use the router ID to refer to the AS number throughout this paper.} (line 1).
$F$ is configured to set a local preference of $200$ for routes whose next hop is $A$ (lines 1-3) and $60$ for routes whose next hop is $E$ (lines 5-7). The other routers in this network are configured with the default BGP settings (\ie, without any customized route policies).
If two routes are equally preferred, the router will choose the one with the lower router ID.
}\fi

% , and $D$ will announce prefix $n$ to this network.

\iffalse{
\para{The configuration error.} The operator has three intents: (1) \(A\) must transit \(W\) to reach \(D\), (2) \(F\) must not transit \(W\) to reaches \(D\), and (3) other routers can reach $D$. 
The simulated forwarding path shows intent 1 being violated. In the actual data plane, $A$ reaches $D$ via path $[A,F,E,D]$.
This is because \(A\) is mistakenly configured to deny the route of path $[A,B,W,D]$.  
However, fixing it does not fully resolve the issue. Though \(A\) will select \([A, B, W, D]\) as the best path (it is preferred due to the lower router ID) after correcting this error, \(F\) will then receive and select it as its best path, causing a violation of intent 2, which reveals that \(F\) setting a higher preference for $A$ over $E$ is also a configuration error (\ie, the latent error).



\para{Limitations of existing tools.} 
We tested various existing tools and found that none of them can accurately diagnose and repair configuration errors, even in this simple network. 
Appendix \ref{appendix} shows the outputs of all these tools.
Configuration verification tools (\eg, Batfish~\cite{fogel2015general, brown2023batfish} and Minesweeper~\cite{beckett2017general}) will alert that configurations cannot satisfy the intent with some limited auxiliary information (\eg, the resulting data plane in Figure~\ref{fig:Batfish-output} or a counterexample in Figure~\ref{fig:MS-output}). 
However, we still do not know how to fix the configuration errors. If there are latent errors, fixing all of them is even more difficult and time-consuming.

Configuration diagnosis and repair tools either failed to pinpoint the errors or produced false positives.  
CEL~\cite{gember2022localizing} did not compute the minimal correction set (MCS) that can help localize the erroneous configuration snippets (Figure~\ref{fig:CEL-output}). 
This is because CEL did not correctly model the configuration semantics (AS path filter). 
CPR~\cite{gember2017automatically} found no errors in this network (Figure~\ref{fig:CPR-output}), and will not continue repairing the errors.
ACR~\cite{acr-hotnets24} missed the real errors despite numerous attempts due to the coverage testing tools it relies on failing to identify the erroneous configuration lines as the repair candidates. Figure~\ref{fig:netcov-output} shows NetCov's output, which did not hit both $A$'s neighboring configuration with $F$ and also its import policy.
}\fi

% Configuration verification tools also struggle to cope with latent errors (the error that a new error is triggered when the previous error is fixed), \eg, Err3 in this example. Since verification tools focus on the current network state, they need more than one time to deal with latent errors in the network.

% help identify and address configuration errors, their solutions can sometimes fall short. 























==> motivation.tex <==

\section{Background}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/revise-example.pdf}
    \caption{The example network.}
    \label{fig:example}
    \vspace{-1em}
\end{figure}


\label{motivation}


% To better understand the gap in approaches for network configuration diagnosis and repair, we first demonstrate the limitations of existing tools with an example and then outline the key challenges.

\subsection{Why Existing Tools Do not work} \label{limitations}


% (a) is the actual forwarding paths computed by the simulation tool (\eg, Batfish~\cite{fogel2015general}). (b) shows the configuration snippets of B and C, including the peer session establishment and the peer policy applied to specific neighbor(s) towards a specific direction.

\para{The example network.} Consider an example network in Figure~\ref{fig:example}, where six routers use BGP to connect to each other.
% , and $D$ will announce prefix $n$ to this network. 
$A$ is configured to deny routes (lines 3-4) whose AS\_PATH contains $W$\footnote{we use the router ID to refer to the AS number throughout this paper} (line 1).
$F$ is configured to set a local preference of $200$ for routes whose next hop is $A$ (lines 1-3) and $60$ for routes whose next hop is $E$ (lines 5-7). The other routers in this network are configured with the default BGP settings (\ie, without any customized route policies).
If two routes are equally preferred, the router will choose the one with the lower router ID.
% imports routes from \(A\) or \(C\), it will deny all routes whose AS\_PATH contains the number 3 using the as-path ACL 1 (deny\_AS3 policy), and $C$ always sets the local preference 200 to routes from $B$ (prefer\_AS6 policy). The other routers in the network are configured with the default BGP settings (\ie, without any customized route policies). The final tie-break in BGP path selection is preferring the path that comes from the lowest neighbor address.


 % this network:  \((B.*W.*D)\),  \((B.*!W.*D)\).

\para{The configuration error.} The operator wants: (1) \(A\) must transit \(W\) to reach \(D\), (2) \(F\) must not transit \(W\) to reaches \(D\), and (3) other routers can reach $D$. 
The simulation shows intent 1 being violated. In the actual data plane, $A$ reaches $D$ via path $[A,F,E,D]$.
This is because \(A\) is mistakenly configured to deny the route of path $[A,B,W,D]$.  
However, fixing it does not fully resolve the issue. Though \(A\) will select \([A, B, W, D]\) as the best path (it is preferred due to the lower router ID) after correcting this error, \(F\) will then receive and select it as its best path, causing a violation of intent 2, which reveals that \(F\) setting a higher preference for $A$ over $E$ is also a configuration error (\ie, the latent error).
% For example, requirement 1 ($AS6 \rightarrow* \rightarrow AS3 \rightarrow* \rightarrow AS1$) means that the traffic from $AS6$ to $AS1$ must traverse $AS3$, the actual forwarding path $AS6 \rightarrow AS5 \rightarrow AS2 \rightarrow AS1$ violates requirement 1. 
% Additionally, the configuration error that violates requirement 4 is that $AS4$ prefers routes from $AS5$ over those from $AS3$ (Err2) due to the shorter as-path. As a result, traffic from $AS4$ to $AS2$ will not pass through $AS3$. 



We tested various existing tools and found that none of them could accurately diagnose and repair configuration errors, even in this simple network. 
Appendix \ref{appendix} shows the outputs of all these tools.
Configuration verification tools (\eg, Batfish~\cite{fogel2015general, brown2023batfish} and Minesweeper~\cite{beckett2017general}) will alert that configurations cannot satisfy the intent with some limited auxiliary information (\eg, the resulting data plane in Figure~\ref{fig:Batfish-output} or a counterexample in Figure~\ref{fig:MS-output}). 
However, we still do not know how to fix the configuration errors. If there are latent errors, fixing all of them is even more difficult and time-consuming.

Configuration diagnosis and repair tools either failed to pinpoint the errors or produced false positives.  
CEL~\cite{gember2022localizing} localizes the Err1 successfully, and the other error it localized is the peer relationship between A and B or B and D, which means deleting the peer relationship configuration could lead to a correct network. 
Appendix \ref{appendix} also shows the CEL output. However, deleting the peer relationship could have a more disruptive impact on the network than adjusting preferences towards the peer. Similarly, configuration synthesis tools like NetComplete~\cite{el2018netcomplete} always produce entirely new configurations that differ significantly from the existing setup, complicating the ongoing network management.
% Configuration verification tools also struggle to cope with latent errors (the error that a new error is triggered when the previous error is fixed), \eg, Err3 in this example. Since verification tools focus on the current network state, they need more than one time to deal with latent errors in the network.

% help identify and address configuration errors, their solutions can sometimes fall short. 




\subsection{Technical Challenges}

Diagnosing the network configuration error and repairing it with minor disturbance on the current configuration face several challenges:

\para{Reasoning about the huge searching space.} Diagnosing the root cause configuration requires reasoning about default settings (\eg, static routes are not redistributed to the BGP process is a default setting) and non-default settings (\eg, set local-preference 200 for specific routes by configuring the import policy in Figure \ref{fig:example}(b)) in configurations. The searching space of configuration variants is enormous. 
As Schneider ~\cite{schneider2022complexity} et al. demonstrated, even synthesizing configurations for arbitrary waypoint requirements for BGP exclusively network is NP-hard. Hence, existing synthesis tools are based on specific templates. For diagnosis, it is essentially to find such commands whose removal, modification, or addition can lead to an intent-compliant configuration in numerous configuration commands. Searching for the first two types of configuration is relatively easier since it focuses on the configured command space. However, sometimes the root cause is some configurations missing, which means we need to reason in the huge space of default settings. 





\para{Computing the side-effect-free repairs.} There are inter-dependencies between distributed routing configurations. Changing one part of the configuration could have unintended consequences on other parts. Ensuring the repair does not introduce side effects requires understanding and managing these dependencies. For example, consider a network with three requirements where only one requirement is violated. When repairing it, it is crucial to ensure that the fix does not affect the compliance of the other two requirements.


\para{Supporting complex requirements and scenarios.} As the network scales, the configuration complexity grows exponentially (\eg, multiple protocols), and requirements get more complicated (\eg, k-failure tolerance). This exponential growth increases the number of configuration parameters, interactions between different network components, and dependencies among various protocols. As a result, diagnosing these configurations becomes significantly more challenging.


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/sse-example.png}
%     \caption{The example of the selective symbolic execution process. (a) shows the program with a block that is selected to symbolic execute (lines 5-8), and corresponding concrete/symbolic program states and path constraints (pc) at certain points. (b) is the control flow graph of the program, and we use different colors to indicate the path coverage of different explorations.}
%     \label{sse-program-example}
%     \vspace{-1em}
% \end{figure*} 



% %(as Figure \ref{fig:trace} shows)
% At the beginning of data plane computation, $D$ redistributes the route $r_0$ into its BGP process, and the program encounters the first "if" branch where the condition $Cond_1$  determines whether the redistribution is allowed. If it goes to the "false" branch as the actual configurations are, the execution terminates since there is no more route exchange between routers. So, we set a condition $Cond_1=true$ and let the program go to the "true" branch. Then D will transform $r0$ into $r1$ and send $r_1$ to its neighbors with the condition $Cond_1=true$. Then, B will receive $r_1$ from D, transform it to $r_2$, and add $r_2$ to its BGP RIB-in. The process continues to generate routes $r_2, r_3, r_4$. These routes all have the condition $Cond_1$, indicating that they exist only when $Cond_1$ is true. 

% % (as Figure \ref{fig:trace} shows) 
% Then, the program encounters the next "if" branch where the condition $Cond_2$ determines whether $r_3$ would be preferred over $r_4$ in router A. 
% The preferred route will be selected as the best route and be sent to A's neighbors. 
% If the program goes to the "false" branch, A will choose $r_4$ and send it to S. S will drop it since $r_4$ carries community tag $d1$. So we have a condition $Cond_2=true$ and let the program go to the "true" branch. Then A will choose $r_3$, and S will receive it and choose it as the best route. 

% As shown in Figure \ref{fig:trace}, the symbolic execution process generates three traces with different conditions at the end, where trace 3 is the intent-compliant trace with condition $Cond_1 \wedge Cond_2$.
% %The trace condition is the sufficient condition of each route in the trace's data plane. 
% %For example, the trace condition of trace 2 implies the route condition of $r_2$ ($S_1\wedge \neg S_2 \implies S_1$). 
% In this example, $Cond_1=false$ is an error, since the redistribution configuration is missing.  $Cond_2=false$ is another error, since means $r_3$ should be preferred over $r_4$. We can add a command to redistribute the network to fix the first error and set a higher local-preference value for $r_3$ or a lower value for $r_4$ to fix the second error. By the symbolic execution approach, we successfully diagnose and repair all errors.

%because it does not comply with the reference condition. We find the redistribution configuration is missing and add a command to redistribute the network. Another error is $S_2=false$, which means $r_3$ should be preferred over $r_4$, we can set a higher local-preference value for $r_3$ or a lower value for $r_4$ as a repair patch.






% \subsection{Limitations of Existing Tools.} \label{existing tools}
% Using configuration verification tools (\eg, Batfish~\cite{fogel2015general, brown2023batfish} and Minesweeper~\cite{beckett2017general}), an operator will receive an alert indicating that configurations cannot satisfy the requirement and some limited auxiliary information (\eg, the resulting data plane or a counterexample). 
% Appendix \ref{appendix} shows the output provided by Batfish and Minesweeper.

% With such information and her/his experience, the operator may realize that the error is caused by $D$ not redistributing routes and then fix it. However, this fix is incomplete as the requirement will still be violated. This is because there is a latent error (the error that a new error is triggered when the previous error is fixed) that $A$ sets a higher local-preference for routes from $B$ than those from $D$. As a result, $A$ selects $A$-$B$-$D$ and sends it to $S$, which then drops the route due to its community tag. Existing configuration diagnosis and repair tools~\cite{zhou2010efficient, wu2014diagnosing, wu2017automated, gember2017automatically} either have capability limitation (\eg, 
% Y!~\cite{wu2014diagnosing, wu2017automated} only apply in SDN and CPR~\cite{gember2017automatically} cannot handle BGP local-preference), or
% cannot handle latent errors such as the one in this simple example. 



% \rulan{Diagnosing the incorrect configurations is essentially to address two questions: "Why does there exist a path?" or "Why does there not exist a path?". An ideal way to answer the two questions is to find all forwarding rules (\ie, the data plane) that result in the path (or non-path) and then infer all configurations (\ie, the control plane) that contribute to the forwarding rules. Answering the first question is relatively easier since there is an observable event (\ie, the existing path) as a starting point that helps infer the related configurations that could contribute to it. However, the second question is hard to address because the event is unobservable (\ie, there is no route), so there is not even a starting point for diagnosis. %Note 
% It requires reasoning about all possibilities that could lead to the unobservable event. It is called negative provenance in~\cite{wu2014diagnosing}, which is NP-hard.} 





==> multiproc-v2.tex <==




\section{Supporting Multiple Protocols}
\label{sec:multi-protocol}
% This section presents a detailed solution for diagnosing configuration errors in a multi-protocol network. We also modify the basic design to support link-state routing protocol diagnosis.

% \subsection{Key Problems}\label{subsection: challenges of multi-protocol}
In modern networks, the coexistence of multiple routing protocols is common. A typical example is the layered architecture where a link-state routing protocol (e.g., OSPF, ISIS) is used for the underlay network and a path-vector routing protocol (e.g., BGP) is used for the overlay network based on the underlay network -- an architecture frequently seen in real networks.
In this work, we focus on such underlay–overlay architectures. We present a decoupling solution for multi-protocol scenarios in \S\ref{subsec:hybrid}, and describe how to extend the selective symbolic execution approach to support link-state routing protocols in \S\ref{subsec:ospf}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/multiproc-a.pdf}
    \caption{The multiple protocols network.}
    \label{fig:multiproc-network}
\end{figure}


\vspace{-1em}
\subsection{Our Solution}
\label{subsec:hybrid}

%One architecture involves interconnecting networks managed by different protocols, making configuration errors relatively straightforward to diagnose as the protocols can be examined independently. Another architecture is the layered network, where the underlay is typically managed by IGP protocols (such as OSPF and ISIS) to ensure the intra-domain reachability, while the overlay uses BGP to exchange routing information between inter-domain neighbors. Error diagnosis for such networks is more challenging due to the mutual interdependence of the protocols. \xing{need to be simplified}

Inspired by modular verification approaches such as Kirigami~\cite{thijm2024kirigami} and Lightyear~\cite{tang2023lightyear}, we decompose the multi-protocol network into distinct layers for modular analysis.To decouple the underlay from the overlay, we first derive an intent-compliant data plane based on the physical topology, following the methodology in \S\ref{sec:derive-contracts}. We then leverage domain knowledge to partition this data plane into overlay and underlay layers, and extract additional overlay-required intents for the underlay layer. This layering and intent decomposition approach enable independent diagnosis and repair of each layer, effectively supporting multi-protocol networks.

%-v1
%To decouple the underlay from the overlay, we leverage domain knowledge to first extract verification intents for the overlay layer. These derived intents are then used to generate additional intents for the underlay. With this layering and intent propagation, we diagnose and repair each layer independently, enabling structured analysis of the multi-protocol network.

%Inspired by modular verification approaches such as Kirigami~\cite{thijm2024kirigami} and Lightyear~\cite{tang2023lightyear}, we modularize the multi-protocol network by slicing it into different layers. To break the dependency between overlay and underlay, we leverage domain knowledge to first derive intents for overlay, and then derive intents for underlay by considering the new intents derived from overlay. Based on these intents, we diagnose and repair each layer independently.

% To decouple protocol dependencies, we first assume that the underlay networks derive contracts for the overlay network, from which the additional underlay network intents can be derived as preconditions. Then, the underlay network can be diagnosed with these additional intents (\(\S\ref{subsec:ospf}\)). This approach allows constraints for each protocol layer to be generated separately, enabling the independent diagnosis of each routing protocol.



\para{An erroneous example network.} We use the network in Figure \ref{fig:multiproc-network} to illustrate our solution. 
In this network, node $S$ connects to node $B$ via eBGP, while nodes $A$, $B$, $C$, and $D$ form a full-mesh iBGP network. Additionally, some interfaces of $A$, $B$, $C$, and $D$ are OSPF-enabled, with edge labels indicating OSPF link costs. The destination IP prefix $p$ is located at node $D$ and is advertised via BGP.
The intended network behavior is: (1) all nodes should be able to reach prefix $p$, and (2) traffic from $S$ must avoid $B$. However, the actual forwarding path [S, B, D] violates Intent 2. This is due to two configuration errors: first, $S$ lacks a BGP peer with $A$; second, misconfigured OSPF costs in AS 2 cause $A$ to prefer reaching $D$ via $B$ instead of $C$.

%The intents are: (1) all nodes reach $p$, and (2) the path of $S$ must avoid $B$. 
%However, the actual data plane [S,B,D] shows that Intent 2 is violated. 
%There are two errors in the configuration: one is that $S$ did not neighbor with $A$, and the other is AS 2's improper OSPF costs that makes $A$ prefer reaching $D$ via $B$ rather than $C$. 
% When two BGP paths are equally preferred, the path with the smallest neighbor address is selected.


% Although \(A-D\) are connected and can exchange routes with each other, the actual forwarding path of \(10/8\) and \(20/8\) are \(SAC\) and \(SBAD\) respectively, which do not compliant with the intents.

\para{Assumptions and guarantees of this network.} 
We first derive intent-compliant data plane following the design in \S\ref{sec:derive-contracts} by considering the physical topology.
In this example, to satisfy these intents, $S$ must reach $D$ via path $[S,A,C,D]$. Given the domain knowledge that an iBGP node does not re-advertise routes learned from its iBGP neighbors (i.e., path $[A,C,D]$ is forbidden) and $A$, $C$, $D$ belong to the IGP domain, we generate BGP Intent 1: $[S,A,\cdots,D]$ and OSPF Intent 1: $[A,C,D]$. 
Furthermore, BGP has an dependency on OSPF networks: BGP uses IPs learned from OSPF to establish neighbor sessions, which enables iBGP neighbors to be non-physically connected. Thus, we have OSPF Intent 2: $D$ and its neighbors $A,B,C$ in the forwarding paths are reachable.

%We decouple BGP's dependency on OSPF by assuming that OSPF satisfies the specific requirements on which BGP relies. This assumption serves as OSPF's intent to guide the corresponding diagnosis and repair. There are two dependencies of BGP on OSPF networks: (1) BGP uses IPs learned from OSPF to establish neighbor sessions, which enables iBGP neighbors to be non-physically connected, and (2) BGP uses the OSPF-determined path to reach the next hop. 

%To yield the intent-compliant data plane in Figure~\ref{fig:multiproc-network}, we should guarantee that two OSPF intents are satisfied: (1) $D$ and its neighbors $A,B,C$ in the forwarding paths are reachable. (2) the OSPF path from $A$ to its next hop $D$ is $[A,C,D]$. And use them as assumptions for BGP diagnosis and repair.

\para{Processing each network layer independently.} 
We derive intent-compliant contracts for the BGP network as \S\ref{finding contracts} demonstrated\xing{how to handle path difference between iBGP and OSPF?}. By selectively simulating the BGP network as the contracts guide, we found that $isPeered$ contract for $S$ and $A$ is violated. 
Meanwhile, the OSPF network also performs selective symbolic simulation based on contracts derived from the assumption intents, and we continue introducing the details in \(\S\ref{subsec:ospf}\).

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multiproc-b.pdf}
        \caption{Intent-compliant contracts of the OSPF network.}
        \label{fig:ospf-contracts}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multiproc-c.pdf}
        \caption{The symbolic simulation of the OSPF network.}
        \label{fig:ospf-sim}
    \end{subfigure}
    \caption{The diagnosis of the OSPF network.}
    \label{fig:ospf-diagnosis}
\end{figure}


\vspace{-1em}
\subsection{Supporting Link-State Routing Protocol}\label{subsec:ospf}

We use OSPF, the most representative link-state routing protocol, to illustrate our approach. Unlike path-vector protocols, which select the best path for each prefix independently, link-state protocols compute the best path for different prefixes from a global perspective (\ie, link cost). To address this, we introduce two design adjustments for link-state protocols: (1) deriving consistent conflict contracts for different prefixes in the same node, and (2) repairing the error by solving it as a MaxSMT problem.



% \para{Modeling the routing configuration.}
% The link-state routing process does not have a flexible routing control mechanism like path-vector-based protocols. That is, it can not process different routes from different neighbors with different policies, which allows us to model such protocols with fewer router behavior variables. We only need three types of variables, similar to BGP, to represent the router behaviors of OSPF, they are: (1) \(RedisToOspf_u^{pfx}\), denoting whether a node \(u\) redistribute its route with prefix \(pfx\) to its OSPF successfully; (2) \(OspfPeer_{u,v}\), denoting whether two nodes are OSPF neighbors; (3) \(OspfPrefer_u^{r_1,r_2}\), denoting whether \(u\) prefers route \(r_1\) to \(r_2\) (based on link cost).


\para{Diagnosing the OSPF network with conflict-free contracts.} 
Deriving conflict-free contracts involves computing conflict-free data planes for different prefixes. 
To achieve this, we compute the intent-compliant data plane for each node, rather than for each prefix individually. \xing{Why each node can be processed independently? How to deal with the path dependency between nodes?}
We continue following algorithm~\ref{algorithm: DP} to compute intent-compliant paths. However, for intents from the same source node, we perform topology multiplication using the intersection of the regular expressions for these intents, rather than treating them separately.
Figure~\ref{fig:ospf-diagnosis} gives the intent-compliant contracts and simulation of the OSPF network. Since the OSPF protocol does not support customizing route policies for neighbors, we derive only $isPeered$ and $isPreferred$ contracts for the OSPF network. 
We simulate the OSPF protocol as a path-vector-based protocol, where the route selections are based on the weighted shortest path, to diagnose the error. In this example, we find one contract violation, indicating $A$ should not prefer route $[A,C,D]$ over $[A,B,D]$. 



\para{Repairing the error.} 
In OSPF networks, contract violations fall into two categories: peering and preference errors. 
Peering errors ($isPeered$ contract) can be fixed simply by enabling routing on the affected interfaces. 
Preference errors ($isPreferred$ contract) require adjusting link costs, which could influence the global path selection. 
We repair preference errors by encoding the whole network with the contracts of all prefixes as a constraint-solving problem to compute the patches collectively.
To preserve as much of the existing configuration as possible, we model it as a MaxSMT problem. 
Hard constraints are the violated contracts that must be fixed and the non‑violated contracts that must remain satisfied, and soft constraints are the link costs of the original configuration.
In this example, we encode the repair problem as: 
\vspace{-0.5em}
\begin{flalign*}
  &\ (hard) \quad l_{AB} + l_{BD} > l_{AC}+ l_{CD} \land l_{AB} + l_{AC}+ l_{CD}  > l_{BD} \\ 
  &\ (soft) \quad l_{AB}==1\land l_{BD}==2 \land l_{AC}==3 \land l_{CD}==4
\end{flalign*}
where $l_{a,b}$ is the link cost of the edge $(a,b)$. A satisfied assignment is to change $l_{AB}$ to $7$ while other link costs remain unchanged, indicating that modifying the link cost of $A,B$ to 7 only can repair the error.


% %\emph{Dealing with conflicts among constraints.} 
% %As far as we're concerned, 
% However, a conflict may exist among SMT constraints for the $Prefer$ condition since edge cost is a positive integer and the number of variables on the left side of the inequality may be greater than the concrete value on the right side. 
% %For example, there are edge cost symbols $a$ and $b$, while we require $a+b<1$. 
% To solve this issue, we assign a larger cost to the concrete value. Since the concrete value must appear on the right side of the inequality, a larger cost won’t influence the result of other SMT constraints. In this way, we resolve the conflict and generate the final patch.

% Consider a new example after we fix the errors in the previous example: the new requirement is an underlay way-point requirement $(C_{1}, C_{3}, C_{3}, C_{1}C_{4}C_{3}, 0)$. We need to generate the $Peer$ condition for $(C_{3}, C_{4})$ and $(C_{1}, C_{4})$, along with $Prefer$ condition for $C_{1}$ and $C_{4}$. Then, during the selective symbolic simulation on the route propagation graph, we construct a constraint that $C_{1}$ prefers the route from $C_{4}$ to $C_{2}$ with symbols $a$ and $b$ to denote the edge costs of $(C_{3}, C_{4})$ and $(C_{4}, C_{1})$. The corresponding inequality is generated as $a+b<edge(C_{1}, C_{2}).cost+edge(C_{2}, C_{3}).cost$. Since the original cost values 10 and 10 do not satisfy the requirement, we turn to the SMT solver for solving $a$ and $b$.
% We notice that $edge(C_{1}, C_{2}).cost$ and $edge(C_{2}, C_{3}).cost$ are both 1. 
% In this situation, $a$ and $b$ cannot be assigned smaller than 1 anymore. 
% As a consequence, we increase $edge(C_{1}, C_{2}).cost$ or $edge(C_{2}, C_{3}).cost$, then call the SMT solver again to generate the solution until the inequality is satisfied. %In this way, we resolve the conflict in error diagnosis and repair.

%

%After that, when we add an additional requirement that C1 reaches C3 and specifies C4 as a waypoint(\ie, the way-point requirement mentioned above), in addition to generating conditions 1) $Peer(C_{1}, C_{2}, OSPF) = true$, 2) $Peer(C_{2}, C_{3}, OSPF) = true$, we also generate $Prefer$ condition for $C_{1}$ and $C_{4}$ and allocate variables $x$ and $y$ to edge $(C_{3}, C_{4})$ and $(C_{4}, C_{1})$. Then, through symbolic execution on the route propagation graph, we will construct a constraint that $C_{1}$ prefers the route from $C_{4}$ to $C_{2}$. The corresponding inequality is generated as $x+y<edge(C_{1}, C_{2}).cost+edge(C_{2}, C_{3}).cost$. \xing{replace x with another symbol, x denotes node before. And explain x and y}

% Computing route propagation paths for way-point requirements is more complex. It is insufficient to compute a $p_{packet}$ which matches the regular expression $P$. There could exist conflict between the calculated path and the existing ones. To avoid this, we calculate a set of route propagation paths $\{p_{i_1}, p_{i_2}, ..., p_{i_n}\}$ for each way-point requirement $i$. We then select a path for each way-point requirement (\eg, $\{p_{1_m}, p_{2_n}, ..., p_{k_q}\}$ if there are k way-point requirements for the network $n$) to check if the path won't conflict with paths that exist in the graph. 

% \para{Reachability violation diagnosis.} We diagnose reachability violations by calculating the shortest path between the source node and the destination node and guaranteeing that the OSPF peer adjacency between every two nodes on the path has been established. We first diagnose reachability violations since waypoint violations are more complicated and some waypoint violations may be satisfied after fixing the connection between peer nodes.

% In link-state protocol, every source node usually chooses the shortest path (the lowest cost) in its RIB as the best path to reach the destination. Once we verify and find that a requirement cannot be satisfied on the current data plane, we compute the shortest path for the source and the destination pair as the desired forwarding path on a graph. The graph is constructed based on the connection of L2 topology. The edge cost is assigned according to the interface configuration. In Figure \ref{fig: multi-protocol example}, we calculate the shortest path for each OSPF reachability requirement. As the shortest path of requirement 2 is a sub-path of requirement 1, we could merge 3 paths into 2 paths. We then generate the peer symbol of each two adjacent nodes on the path. The symbol indicates whether the OSPF adjacency between two nodes has been established. In the example, we will check symbol \textit{Peer}(C1, C2, OSPF), \textit{Peer}(C2, C3, OSPF) and \textit{Peer}(C4, C3, OSPF) accordingly. Since Batfish models the process of OSPF link state announcement like the path-vector one, the process of symbolic execution on OSPF is then similar to that of BGP symbol execution. We won't go into details.

% \para{Waypoint violation diagnosis.} Here's an additional constraint to the original requirement that packets have to traverse a waypoint C4 to reach p. The key to solving the waypoint violation is to first guarantee the reachability of the desired forwarding path and second, assign appropriate costs to the edges and ensure the route of the desired path is selected. Consequently, we introduce \textit{Peer} and \textit{Prefer} symbols to the symbolic execution process.

% We first compute a desired intent-compliant data plane for each destination prefix. A intent-compliant data plane consists of forwarding paths for all requirements with the same destination node. We aim to compute a desired forwarding path for each unsatisfied waypoint requirement. Meanwhile, ensure the original forwarding paths of satisfied waypoint requirements remain unchanged as much as possible. In concrete terms, we first compute a desired forwarding path set for each unsatisfied requirement according to the topology and the requirement. Then, we select one path from the set for each requirement and try to find a combination of these paths such that this combination does not conflict with the forwarding paths of the satisfied requirements. Otherwise, we may have to compute new paths for the satisfied requirements. As long as we could compute a desired intent-compliant data plane for the destination IP prefix, we argue that it would be able to modify the configuration to ensure that the waypoint requirements are satisfied. Conversely, we assume that the current requirements cannot be satisfied simultaneously. In the example network, we calculate a desired path (C1, C4, C3).

% Then we solve waypoint violations via symbolic execution. To make sure packets are sent through the correct forwarding path we compute for a specific requirement, we propagate two symbols (\textit{Peer} and \textit{Prefer}) along the opposite direction of the forwarding path (route propagation direction). The \textit{Peer} symbol ensures the destination node is reachable from the source node. The \textit{Prefer} symbol guarantees that the desired forwarding path is the shortest. We take the edge cost to edges in the desired forwarding path as variables. When a router A receives a route from its peer B, it adds \textit{cost}(B, \textit{p}) with \textit{cost}(A, B) where \textit{cost}(B, \textit{p}) is the cost from peer to the destination, and \textit{cost}(A, B) is the edge cost between peer and itself. For all nodes in the desired forwarding path, we construct a set of SMT constraints to ensure the \textit{Prefer} symbols are satisfied. We use \textit{Prefer} symbol to make sure that the route from the node downstream of the desired forwarding path has a lower cost compared to other routes in the RIB table. Thus the desired route will be selected and installed in the RIB. We then use the SMT solver({\eg}, z3) to solve for the concrete values of the edge cost variables. In the example network, we first allocate variables x and y to edge (C3, C4) and (C4, C1). We then construct a constraint that C1 prefers the route from C4 to C2. The corresponding inequality is x+y<1+1.




==> multiproc-v3.tex <==
\begin{figure*}[!htbp]
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/multiproc-a.pdf}
    \caption{The intent-compliant data plane.}
    \label{fig:multiproc-DP}
  \end{subfigure}
   \hspace{1em}
  \begin{subfigure}[b]{0.6\textwidth}
    \includegraphics[width=\linewidth]{figures/multiproc-b.pdf}
    \caption{Intent-compliant contracts and selective symbolic simulation of the OSPF network.}
    \label{fig:multiproc-OSPF}
  \end{subfigure}
  \caption{The multiple protocol network example.}
  \label{fig:multiproc}
\end{figure*}

\section{Multi-Protocol Networks}\label{sec:multi-protocol}
After describing \system{}'s basic design using BGP as an example, we introduce
how it diagnoses and repairs networks where multiple protocols (\eg, OSPF and
BGP) co-exist. Because \system{} can handle a network running different routing
protocols in different regions by examining these regions separately, we focus
on networks running different routing protocols in a layered setting (\eg, OSPF
as underlay and BGP as overlay). To this end, we use the following example to
first illustrate how \system{}
diagnoses and repairs link-state routing protocols (\S\ref{}), and then
introduce how it works for layered networks (\S\ref{}).

\para{Example.}
Figure~\ref{fig:multiproc-DP} shows an example of two ASes peered with eBGP and routers $A$, $B$, $C$, and $D$ are connected using OSPF in underlay and peered with iBGP in a full mesh in overlay. In the configuration, $S$ is only peered with $B$ via eBGP and the OSPF cost of each link in $AS$ 2 is shown in the edges. The destination IP prefix $p$ is located at node $D$ and is advertised via BGP.
The network intents are: (1) all routers can reach prefix $p$, and (2) the path of $S$ to reach $p$ should not pass $B$. The data plane of the original configuration is marked in red, which is erroneous.

\subsection{Link-State Routing Protocols}\label{subsec:ospf}
The fundamental difference between path vector and link-state protocols is that
the former selects the best paths for different prefixes independently (\ie,
per-prefix policy routing) while the latter does so with a unified metric (\ie,
prefix-oblivious link costs).


========

%Unlike path-vector protocols, which select the best path for each prefix independently, link-state protocols compute the best path for different prefixes from a global perspective (\ie, link cost). 

To address this, we introduce two designs for link-state protocols: (1) deriving conflict-free contracts for different prefixes in the same node, and (2) repairing the error by solving it as a MaxSMT problem. We use OSPF, the most representative link-state routing protocol, to illustrate our approach.

% \para{Modeling the routing configuration.}
% The link-state routing process does not have a flexible routing control mechanism like path-vector-based protocols. That is, it can not process different routes from different neighbors with different policies, which allows us to model such protocols with fewer router behavior variables. We only need three types of variables, similar to BGP, to represent the router behaviors of OSPF, they are: (1) \(RedisToOspf_u^{pfx}\), denoting whether a node \(u\) redistribute its route with prefix \(pfx\) to its OSPF successfully; (2) \(OspfPeer_{u,v}\), denoting whether two nodes are OSPF neighbors; (3) \(OspfPrefer_u^{r_1,r_2}\), denoting whether \(u\) prefers route \(r_1\) to \(r_2\) (based on link cost).


\para{Diagnosing the OSPF network with conflict-free contracts.} 
Deriving conflict-free contracts involves computing conflict-free data planes for different prefixes. 
To achieve this, we compute the intent-compliant data plane for each node, rather than for each prefix individually. \xing{Why each node can be processed independently? How to deal with the path dependency between nodes?}
We continue following algorithm~\ref{algorithm: DP} to compute intent-compliant paths. However, for intents from the same source node, we perform topology multiplication using the intersection of the regular expressions for these intents, rather than treating them separately.
Figure~\ref{fig:multiproc-OSPF} gives the intent-compliant contracts and simulation of the OSPF network. Since the OSPF protocol does not support customizing route policies for neighbors, we derive only $isPeered$ and $isPreferred$ contracts for the OSPF network. 
We simulate the OSPF protocol as the path-vector-based protocols, where the route selections are based on the weighted shortest path, to diagnose the error. In this example, we find one contract violation, indicating $A$ should not prefer route $[A,C,D]$ over $[A,B,D]$. 



\para{Repairing the error.} 
In OSPF networks, contract violations fall into two categories: peering and preference errors. 
Peering errors ($isPeered$ contract) can be fixed simply by enabling routing on the affected interfaces. 
Preference errors ($isPreferred$ contract) require adjusting link costs, which could influence the global path selection. 
We repair preference errors by encoding the whole network with the contracts of all prefixes as a constraint-solving problem to compute the patches collectively.
To preserve as much of the existing configuration as possible, we model it as a MaxSMT problem. 
Hard constraints are the violated contracts that must be fixed and the non‑violated contracts that must remain satisfied, and soft constraints are the link costs of the original configuration.
In this example, we encode the repair problem as: 
\vspace{-0.5em}
\begin{flalign*}
  &\ (hard) \quad l_{AB} + l_{BD} > l_{AC}+ l_{CD} \land l_{AB} + l_{AC}+ l_{CD}  > l_{BD} \\ 
  &\ (soft) \quad l_{AB}==1\land l_{BD}==2 \land l_{AC}==3 \land l_{CD}==4
\end{flalign*}


where $l$ is the link cost of the edge, a satisfied assignment is changing $l_{AB}$ to $7$ while other link costs remain unchanged, indicating that modifying only the link cost of $A,B$ to 7 can repair the error.


% %\emph{Dealing with conflicts among constraints.} 
% %As far as we're concerned, 
% However, a conflict may exist among SMT constraints for the $Prefer$ condition since edge cost is a positive integer and the number of variables on the left side of the inequality may be greater than the concrete value on the right side. 
% %For example, there are edge cost symbols $a$ and $b$, while we require $a+b<1$. 
% To solve this issue, we assign a larger cost to the concrete value. Since the concrete value must appear on the right side of the inequality, a larger cost won’t influence the result of other SMT constraints. In this way, we resolve the conflict and generate the final patch.

% Consider a new example after we fix the errors in the previous example: the new requirement is an underlay way-point requirement $(C_{1}, C_{3}, C_{3}, C_{1}C_{4}C_{3}, 0)$. We need to generate the $Peer$ condition for $(C_{3}, C_{4})$ and $(C_{1}, C_{4})$, along with $Prefer$ condition for $C_{1}$ and $C_{4}$. Then, during the selective symbolic simulation on the route propagation graph, we construct a constraint that $C_{1}$ prefers the route from $C_{4}$ to $C_{2}$ with symbols $a$ and $b$ to denote the edge costs of $(C_{3}, C_{4})$ and $(C_{4}, C_{1})$. The corresponding inequality is generated as $a+b<edge(C_{1}, C_{2}).cost+edge(C_{2}, C_{3}).cost$. Since the original cost values 10 and 10 do not satisfy the requirement, we turn to the SMT solver for solving $a$ and $b$.
% We notice that $edge(C_{1}, C_{2}).cost$ and $edge(C_{2}, C_{3}).cost$ are both 1. 
% In this situation, $a$ and $b$ cannot be assigned smaller than 1 anymore. 
% As a consequence, we increase $edge(C_{1}, C_{2}).cost$ or $edge(C_{2}, C_{3}).cost$, then call the SMT solver again to generate the solution until the inequality is satisfied. %In this way, we resolve the conflict in error diagnosis and repair.

%

%After that, when we add an additional requirement that C1 reaches C3 and specifies C4 as a waypoint(\ie, the way-point requirement mentioned above), in addition to generating conditions 1) $Peer(C_{1}, C_{2}, OSPF) = true$, 2) $Peer(C_{2}, C_{3}, OSPF) = true$, we also generate $Prefer$ condition for $C_{1}$ and $C_{4}$ and allocate variables $x$ and $y$ to edge $(C_{3}, C_{4})$ and $(C_{4}, C_{1})$. Then, through symbolic execution on the route propagation graph, we will construct a constraint that $C_{1}$ prefers the route from $C_{4}$ to $C_{2}$. The corresponding inequality is generated as $x+y<edge(C_{1}, C_{2}).cost+edge(C_{2}, C_{3}).cost$. \xing{replace x with another symbol, x denotes node before. And explain x and y}

% Computing route propagation paths for way-point requirements is more complex. It is insufficient to compute a $p_{packet}$ which matches the regular expression $P$. There could exist conflict between the calculated path and the existing ones. To avoid this, we calculate a set of route propagation paths $\{p_{i_1}, p_{i_2}, ..., p_{i_n}\}$ for each way-point requirement $i$. We then select a path for each way-point requirement (\eg, $\{p_{1_m}, p_{2_n}, ..., p_{k_q}\}$ if there are k way-point requirements for the network $n$) to check if the path won't conflict with paths that exist in the graph. 

% \para{Reachability violation diagnosis.} We diagnose reachability violations by calculating the shortest path between the source node and the destination node and guaranteeing that the OSPF peer adjacency between every two nodes on the path has been established. We first diagnose reachability violations since waypoint violations are more complicated and some waypoint violations may be satisfied after fixing the connection between peer nodes.

% In link-state protocol, every source node usually chooses the shortest path (the lowest cost) in its RIB as the best path to reach the destination. Once we verify and find that a requirement cannot be satisfied on the current data plane, we compute the shortest path for the source and the destination pair as the desired forwarding path on a graph. The graph is constructed based on the connection of L2 topology. The edge cost is assigned according to the interface configuration. In Figure \ref{fig: multi-protocol example}, we calculate the shortest path for each OSPF reachability requirement. As the shortest path of requirement 2 is a sub-path of requirement 1, we could merge 3 paths into 2 paths. We then generate the peer symbol of each two adjacent nodes on the path. The symbol indicates whether the OSPF adjacency between two nodes has been established. In the example, we will check symbol \textit{Peer}(C1, C2, OSPF), \textit{Peer}(C2, C3, OSPF) and \textit{Peer}(C4, C3, OSPF) accordingly. Since Batfish models the process of OSPF link state announcement like the path-vector one, the process of symbolic execution on OSPF is then similar to that of BGP symbol execution. We won't go into details.

% \para{Waypoint violation diagnosis.} Here's an additional constraint to the original requirement that packets have to traverse a waypoint C4 to reach p. The key to solving the waypoint violation is to first guarantee the reachability of the desired forwarding path and second, assign appropriate costs to the edges and ensure the route of the desired path is selected. Consequently, we introduce \textit{Peer} and \textit{Prefer} symbols to the symbolic execution process.

% We first compute a desired intent-compliant data plane for each destination prefix. A intent-compliant data plane consists of forwarding paths for all requirements with the same destination node. We aim to compute a desired forwarding path for each unsatisfied waypoint requirement. Meanwhile, ensure the original forwarding paths of satisfied waypoint requirements remain unchanged as much as possible. In concrete terms, we first compute a desired forwarding path set for each unsatisfied requirement according to the topology and the requirement. Then, we select one path from the set for each requirement and try to find a combination of these paths such that this combination does not conflict with the forwarding paths of the satisfied requirements. Otherwise, we may have to compute new paths for the satisfied requirements. As long as we could compute a desired intent-compliant data plane for the destination IP prefix, we argue that it would be able to modify the configuration to ensure that the waypoint requirements are satisfied. Conversely, we assume that the current requirements cannot be satisfied simultaneously. In the example network, we calculate a desired path (C1, C4, C3).

% Then we solve waypoint violations via symbolic execution. To make sure packets are sent through the correct forwarding path we compute for a specific requirement, we propagate two symbols (\textit{Peer} and \textit{Prefer}) along the opposite direction of the forwarding path (route propagation direction). The \textit{Peer} symbol ensures the destination node is reachable from the source node. The \textit{Prefer} symbol guarantees that the desired forwarding path is the shortest. We take the edge cost to edges in the desired forwarding path as variables. When a router A receives a route from its peer B, it adds \textit{cost}(B, \textit{p}) with \textit{cost}(A, B) where \textit{cost}(B, \textit{p}) is the cost from peer to the destination, and \textit{cost}(A, B) is the edge cost between peer and itself. For all nodes in the desired forwarding path, we construct a set of SMT constraints to ensure the \textit{Prefer} symbols are satisfied. We use \textit{Prefer} symbol to make sure that the route from the node downstream of the desired forwarding path has a lower cost compared to other routes in the RIB table. Thus the desired route will be selected and installed in the RIB. We then use the SMT solver({\eg}, z3) to solve for the concrete values of the edge cost variables. In the example network, we first allocate variables x and y to edge (C3, C4) and (C4, C1). We then construct a constraint that C1 prefers the route from C4 to C2. The corresponding inequality is x+y<1+1.










=================
% This section presents a detailed solution for diagnosing configuration errors in a multi-protocol network. We also modify the basic design to support link-state routing protocol diagnosis.

% \subsection{Key Problems}\label{subsection: challenges of multi-protocol}
In modern networks, multiple routing protocols coexist in two common architectures. One architecture involves interconnecting networks managed by different protocols, making configuration errors relatively straightforward to diagnose as the protocols can be examined independently. Another architecture is the layered network, where the underlay is typically managed by IGP protocols (such as OSPF and ISIS) to ensure the intra-domain reachability, while the overlay uses BGP to exchange routing information between inter-domain neighbors. Error diagnosis for such networks is more challenging due to the mutual interdependence of the protocols. \xing{need to be simplified}





\vspace{-1em}
\subsection{Our Solution}
\label{subsection: BGP in multi-protocol}
Inspired by modular verification approaches such as Kirigami~\cite{thijm2024kirigami} and Lightyear~\cite{tang2023lightyear}, we modularize the multiple protocol network by slicing it into different network layers, and leverage domain knowledge to define the assumption and guarantee for each layer, to diagnose and repair these network layers independently.
% To decouple protocol dependencies, we first assume that the underlay networks derive contracts for the overlay network, from which the additional underlay network intents can be derived as preconditions. Then, the underlay network can be diagnosed with these additional intents (\(\S\ref{subsec:ospf}\)). This approach allows constraints for each protocol layer to be generated separately, enabling the independent diagnosis of each routing protocol.






\para{An erroneous example network.} We use the network in Figure \ref{fig:multiproc-DP} as an example to demonstrate our solution. 
In this network, $S$ uses eBGP to connect $B$, while $A,B,C,D$ are fully meshed using iBGP\xing{not full-meshed in the graph?}. The edge number\xing{number on the edge?} is the OSPF link cost. 
The destination IP prefix $p$ is at $D$. 
The intents are: (1) all nodes reach $p$, and (2) the path of $S$ must avoid $B$. 
To satisfy these intents, $S$ must reach $D$ via path $[S,A,C,D]$.
However, the actual data plane shows that Intent 2 is violated. 
There are two errors in the configuration: one is that $S$ did not neighbor with $A$, and the other is AS 2's bad OSPF cost that leads $A$ to prefer reaching $D$ via $B$ rather than $C$. 
% When two BGP paths are equally preferred, the path with the smallest neighbor address is selected.


% Although \(A-D\) are connected and can exchange routes with each other, the actual forwarding path of \(10/8\) and \(20/8\) are \(SAC\) and \(SBAD\) respectively, which do not compliant with the intents.

\para{Assumptions and guarantees of this network.} 
We decouple BGP's dependency on OSPF by assuming that OSPF satisfies the specific requirements on which BGP relies. This assumption serves as OSPF's intent to guide the corresponding diagnosis and repair. 
There are two dependencies of BGP on OSPF networks: (1) BGP uses IPs learned from OSPF to establish neighbor sessions, which enables iBGP neighbors to be non-physically connected, and (2) BGP uses the OSPF-determined path to reach the next hop. 
The domain knowledge of the full meshed network is that 
An iBGP node will send its originated (or external) route to all iBGP neighbors and use itself as the next hop for those neighbors. However, it will not re-advertise routes learned from other iBGP neighbors. \xing{delete? the domain knowledge seems not used?}
To yield the intent-compliant data plane in Figure~\ref{fig:multiproc-DP}, we should guarantee that two OSPF intents are satisfied: (1) $D$ and its neighbors $A,B,C$ in the forwarding paths are reachable. (2) the OSPF path from $A$ to its next hop $D$ is $[A,C,D]$. And use them as assumptions for BGP diagnosis and repair.




\para{Processing each network layer independently.} 
We derive intent-compliant contracts for the BGP network as \S\ref{finding contracts} demonstrated\xing{how to handle path difference between iBGP and OSPF?}. By selectively simulating the BGP network as the contracts guide, we found that $isPeered$ contract for $S$ and $A$ is violated. 
Meanwhile, the OSPF network also performs selective symbolic simulation based on contracts derived from the assumption intents, and we continue introducing the details in \(\S\ref{subsec:ospf}\).



%\vspace{-1em}




==> multiprotocol_diagnosis.tex <==
%\section{Diagnosing the Multi-Protocol Network}
\section{Supporting Multiple Protocols}
\label{sec:multi-protocol}
This section presents a detailed solution for diagnosing configuration errors in a multi-protocol network. We also modify the basic design to support link-state routing protocol diagnosis.
%decouple the requirements and achieve hierarchical diagnosis to 

%  This section proposes a detailed solution to the multiple protocol problem extended from the basic design. We generate underlay reachability and way-point requirements from overlay BGP requirements. 
% We diagnose and repair all the requirements of each protocol using Batfish. Besides, we modify Batfish to apply symbolic execution on link-state protocols. 
% Today’s distributed network control planes are highly sophisticated, with multiple interacting protocols operating at layers 2 and 3. 


\subsection{Key Problems}\label{subsection: challenges of multi-protocol}
In modern networks, multiple routing protocols coexist in two common architectures. The first involves interconnecting networks managed by different protocols, making configuration errors relatively straightforward to diagnose as the protocols can be examined independently. In the second, layered architecture, the underlay is typically managed by IGP protocols (such as OSPF and ISIS), while the overlay uses BGP to exchange routing information between autonomous systems. Diagnosing errors here is more challenging due to the mutual interdependence of the protocols.

% In modern networks, multiple routing protocols commonly coexist. One common architecture involves interconnecting networks managed by different routing protocols. Another common design is the layered network, where the underlay employs one routing protocol while the overlay utilizes another.

% Configuration errors in the first architecture are relatively straightforward to diagnose, as the two routing protocols can be examined independently. While errors in layered networks are more challenging to diagnose because the protocols can be interdependent, generally, IGP protocols (such as OSPF and ISIS) typically manage the underlay network, while BGP is used in the overlay network. Specifically, BGP exchanges routing information between different autonomous systems (ASes), whereas IGP handles reachability within an AS. 



% Configuration errors for the first kind of network are easy to diagnose: We simply diagnose these two routing protocols separately. Diagnosing the second kind of network is challenging because protocols could be dependent on each other. In modern networks, IGP protocols (\eg, OSPF and ISIS) are used for the underlay network and BGP protocols for the overlay network. 
% Specifically, BGP exchanges routing information between different autonomous systems (ASes), while IGP handles the reachability within an autonomous system (AS). Thus, the IGP does not need to be aware of external AS connections, and traffic traversing the AS via BGP behaves as if the entire AS were a single node.


% As a result, IGP need not be aware of external AS connections, and traffic routed through BGP behaves as if the entire AS were a single node.


%the network using one protocol in one part and another protocol in another part.


%Challenges of multi-protocol network diagnosis arise from the coupling between protocols.  We simply diagnose the network for each part and ensure the connectivity between networks.  


% to exchange routing information hop-by-hop to reach the destination
% Routers in different AS use BGP to exchange routing information, and routers in the same AS use OSPF to connect each other and synchronize routes.

% design strategies exist for such networks to reach different IP prefixes using different routing protocols. 
\begin{figure*}[t]
    \centering
    % \includegraphics[width=\linewidth]{figures/scalpel-sigcomm24-example-multiproc.pdf}
    \includegraphics[width=\linewidth]{figures/multi-proc.png}
    \caption{An example network with multiple routing protocols for error diagnosis and repair.}
    \label{fig: multi-protocol example}
    \vspace{-1em}
\end{figure*} 


\subsection{Our Solution}\label{subsection: BGP in multi-protocol}
The key insight in diagnosing the multi-protocol layered network is decoupling the protocol dependencies (\eg, BGP relies on IGP) by computing additional intents for the underlay network. 
First, we construct an intended intent-compliant data plane using the method from \(\S\ref{subsec:intent-compliant data plane}\). Next, we generate the overlay network constraints, from which the additional underlay network intents can be derived as preconditions. Then, the underlay network can be diagnosed with these additional intents (\(\S\ref{subsec:ospf}\)). This approach allows constraints for each protocol layer to be generated separately, enabling the independent diagnosis of each routing protocol.






\para{An example network.} We will use the network in Figure \ref{fig: multi-protocol example} as an example to demonstrate our solution. 
In this network, \(S\) (in AS1) uses eBGP to connect \(A, B\). \(A-D\) (in AS 2) use iBPG in a full mesh manner to connect each other with their loopback0 IPs, which are learned from OSPF. The number on the edges represents the OSPF link cost (Figure~\ref{fig: multi-protocol example}(b)). When two BGP paths are equally preferred, the path with the smallest neighbor address is selected.

\(D\) connects a subnet $10/8$, and we want $S$ to reach $D$ ($10/8$) through $C$ (denoted as $(S, D, 10/8, S.*C.*D, any\_path)$). 
However, the actual path that S takes is \(SAD\). Both of OSPF and BGP configuration errors contribute to this unintended path:
(1) $B$ and \(C\) do not enable their OSPF routing on the connected interfaces; (2) \(B\) forwards packets to \(10/8\) via path \(BAD\) since this path has lower cost than \(BCD\); (3) S will select \(A\) rather than \(B\) as the next-hop due to the smaller neighbor address.
% Although \(A-D\) are connected and can exchange routes with each other, the actual forwarding path of \(10/8\) and \(20/8\) are \(SAC\) and \(SBAD\) respectively, which do not compliant with the intents.

\para{Constraints for the overlay network.} 
The route propagation and selection constraints in multi-protocol networks differ from those in single-protocol networks, as the reversed forwarding paths sometimes (\ie, iBGP peers are not physically connected) do not always align with the route propagation paths. 
Given a sub-path \(p = [u_1, ..., u_x]\) within the same AS, where \(u_x\) is the farthest node and \(u_1\) is the nearest node from the source.
We add route propagation constraints for each \(u_i\) (\(1 \leq i < x\)) to peer with \(u_x\) and import the routes from it, and for \(u_x\) to export its routes to each \(u_i\). 
In this example, we have constructed the intended forwarding path \([S,B,C,D]\) for \(10/8\), and the sub-path within the same AS is \([B,C,D]\).
As such, we have \(bc1-bc6\) constraints (Figure~\ref{fig: multi-protocol example}(a)) for the route propagation of the sub-path, we omit the route propagation constraints \(bc7-bc9\) for edge \(S\rightarrow B\) here.
Then, we add route selection constraints to ensure each \(u_i\) (\(1 \leq i < x\)) prefers the route from \(u_x\) over the route from other neighbors. We choose the route from \(u_x\) rather than \(u_{i+1}\) as iBGP routers generally do not advertise routes learned from one iBGP neighbor to another iBGP neighbor within the same AS, as \(bc10\) shows.


\para{Additional intents for the underlay network.} 
The dependency between overlay and underlay networks includes: (1) BGP relies on IPs learned from IGP to establish neighbor sessions, enabling iBGP neighbors to be non-physically connected, (2) BGP relies on IPs learned from IGP as the next-hop, ensuring the accurate recursive lookups. 
Similarly, given a sub-path \(p = [u_1, ..., u_x]\) within the same AS.
We first add intents for neighboring IP reachability. Specifically, for each node \(u_i\) where \(1 \leq i < x\), we add intents of neighboring IPs of \(u_x\) and \(u_i\) are reachable from each other, serving as preconditions for establishing their BGP neighbor session. 
Next, we add next-hop reachability intents, ensuring that \(u_1\) reaches \(u_x\) along the intended path \(p\).
In this example, additional intents are (1) \(D\) and \(B\), \(D\) and \(C\) should be reachable, (2) \(B\) should reach \(D\) via \(BCD\) (as Figure~\ref{fig: multi-protocol example}(b) shows). 

\para{Diagnosing each protocol independently.} 
The overlay (BGP) and underlay (IGP) networks can be diagnosed independently since we have decoupled dependent intents for the underlay networks. 
The overlay network can perform selectively symbolic simulation assuming the preconditions are satisfied, \eg, \(B\) will forward traffics to \(10/8\) with next-hop D along the path \(BCD\). 
The BGP constraints will guide the simulation to achieve to the intended routes, as Figure~\ref{fig: multi-protocol example}(a) shows, each route is represented as \((prefix, as\_path,next\_hop,broken\_condistions)\), with the best route underline. We find \(bc10\) is a broken constraint, which indicates the BGP configuration error. 
The underlay network can also perform selective symbolic simulation based on constraints derived from the additional intents, and we continue introducing the details in \(\S\ref{subsec:ospf}\).




% In a multi-protocol network, two neighboring routers in the packet forwarding path may not be physically connected, and they may belong to the same AS. For the former case, we need to generate new requirements for the underlay network. For the latter case, we need to shrink the packet forwarding path to exclude redundant routers belonging to the same AS, since the reachability of nodes in an AS is managed by the underlay routing protocol.

% Thus, we modify the transformation of a packet forwarding path to a route propagation path as follows: 1) replacing $x_i$ with $x_i.proc$ where $proc$ is the overlay routing protocol; 
% 2) starting from $x_n.proc$ to add the edge from the current node to its farthest routing neighbor (here, the farthest routing neighbor of $x_i.proc$ is defined as its farthest upstream node $x_j.proc$ where $x_j$ and $x_i$ are in the same AS, and $x_{j-1}$ and $x_j$ are not in the same AS); 
% 3) repeating this process until $x_1$ is reached;
% %Then repeat this process for the farthest routing neighbor. 
% % (or $x_j=x_1$ if they are in the same AS)
% and 4) adding a redistribution edge for $x_n$. 
% add an edge from $x_i.proc$ to $x_j.proc$ where $x_j$ is the farthest router in  the same AS with $x_i$, 3) 


% \parablue{mainly talks about how to convert an overlay requirement to a detailed underlay requirement. and give an example of two kinds of underlay requirements (reachability and waypoint).}

% In a network only configured with BGP, the requirement that two nodes can access each other depends on the establishment of their BGP peer. Specifically, BGP peer establishment requires basic IP layer connectivity, a unique AS number, and other correct BGP configurations.

% In a network with underlay and overlay design. A BGP requirement implicitly implies some IGP requirements. According to \S\ref{sec: basic design}, a BGP requirement is first converted to a forwarding path. Then we draw nodes belonging to the same AS from the path as IGP reachable/waypoint requirements.









%\subsection{Break down the Requirement for Each Protocol.}\label{subsec: multiple protocol example}





\subsection{Supporting Link-State Routing Protocol}\label{subsec:ospf}

We use OSPF, which is the most representative link-state routing protocol, to illustrate our approach.
The general steps for OSPF diagnosis are the same as BGP, as \cite{fogel2015general} demonstrates, we can simulate the route propagation process of a link-state protocol by modeling it as a simplified path-vector protocol, where the path selection is purely based on link costs. 
However, unlike the path-vector protocol, which handles each prefix independently, the link-state protocol handles all prefixes jointly (the OSPF path selection is based on global link costs). 
Therefore, we introduce two design adaptations for link-state protocols: (1) computing the intent-compliant data plane for all prefixes in the same destination collectively and (2) repairing the OSPF configuration as a MaxSMT problem.

\para{Modeling the routing configuration.}
The link-state routing process does not have a flexible routing control mechanism like path-vector-based protocols. That is, it can not process different routes from different neighbors with different policies, which allows us to model such protocols with fewer router behavior variables. We only need three types of variables, similar to BGP, to represent the router behaviors of OSPF, they are: (1) \(RedisToOspf_u^{pfx}\), denoting whether a node \(u\) redistribute its route with prefix \(pfx\) to its OSPF successfully; (2) \(OspfPeer_{u,v}\), denoting whether two nodes are OSPF neighbors; (3) \(OspfPrefer_u^{r_1,r_2}\), denoting whether \(u\) prefers route \(r_1\) to \(r_2\) (based on link cost).


\para{Computing the intent-compliant data plane.} 
We compute a single intent-compliant data plane for a destination, rather than for individual prefixes, to avoid conflicts between prefixes within the same destination.
We gather the path regular expressions of intents with the same destination to build the intent-compliant data plane. 
Starting with the existing shortest intent-compliant data plane, we preserve paths as much as possible by replacing the path regex of satisfied intents with existing paths.
The conflict-free traversal (\(\S\ref{subsec:intent-compliant DP}\)) computes an intended intent-compliant data plane, even if multiple path regexes exist for the same source, by searching for the intersection of all path regexes. If no solution is found due to path preservation, we use greedy algorithm 1 to iteratively find the intent-compliant data plane.
In Figure~\ref{fig: multi-protocol example}(b) example, we compute the intended intent-compliant data plane as the green dash lines indicate.


%\para{Generating router behavior conditions.} 
\para{Simulating configuration variants as the intent-compliant data plane indicates.} 
We also represent each route as a 4-tuple \((dst,path,next\_hop, broken\_conditions)\) where \(path\) is the forwarding path of this route.
The default path-vector implementation of link-state protocols does not carry path information. So, we modify this implementation to identify the best route during selective symbolic simulation.
The best route of each node is the one whose \(path\) is the intended forwarding path.
We then generate route propagation and selection constraints for OSPF as the intent-compliant data plane indicates, just as how we generate BGP constraints. In this example, they are \(oc_1\sim oc_5\) shown in \ref{fig: multi-protocol example}(b). At first, \(D\) send the originated route \(or_1\) to \(A,C\), and \(A,C\) select it as their best routes \(or_1,or_2\). \(A\) continue sending \(or_2\) to \(B\) to get \(or_3\). \(C\), as the given configuration suggests, is not peer with \(B\), thus will not send \(or_2\) to \(B\), which violates constraint \(oc_2\), so we still simulate as the constraint guides and add it as a broken constraint to \(oc_4\). Similarly, when \(B\) determines which route is preferred, also prefers \(or_4\) to \(or_3\) and add the broken constraint to \(or_4\). 


% We use the $Prefer$ and $Peer$ symbols to generate symbolic route behavior conditions based on the reference route propagation graph. For the reachability route propagation graph $G_{R}(V, E)$, we generate $Peer(u, v, OSPF) = true$ for each edge $(u,v)$. For the way-point route propagation graph $G_{WR}(V, E)$, besides $Peer(u, v, OSPF) = true$ for each edge $(u,v)$, we also generate $Prefer(r_{x}, r_{y}, OSPF) = true$ for each $v \in V$ where $r_{x}$ is the route comes from  $v$'s upstream node in $G_{WR}(V, E)$ and $r_{y}$ denotes the routes from the other nodes. Here, to make the $Prefer$ condition true, we need to assign appropriate costs to the $e \in E$ to make the route cost of $r_{x}$ smaller than $r_{y}$. We allocate edge cost symbols to represent edge costs on $G_{WR}(V, E)$. In the end, we can get a constraint-solving problem. By solving the problem, we can ensure the requirement-compliant routes are selected and installed in the RIB. 

% In the example, to meet the reachability requirement, we use $G_{R}(V, E)$ to generate two $Peer$ conditions $Peer(C_{1}, C_{2}, OSPF) = true$ and $Peer(C_{2}, C_{3}, OSPF) = true$. %

\para{Repairing the error.} 
Repairing the link-state routing configuration essentially fixes the peer-enabled and link-cost errors. Fixing the first error is straightforward: Enable routing on the corresponding interfaces.
We repair the link-cost error by encoding it as a MaxSMT problem. The hard constraints of the problem are the route selection constraints generated from the intent-compliant data plane. The soft constraints are the link costs of the given configuration. Then, we use the SMT solver (\eg, Z3) to solve a satisfied assignment, as such, we find a repair while maximumly preserving the given configuration.
In this example, we encode the repair problem as: 

\[(hard)\ cost_{AD} + cost_{AB} > cost_{CD}+ cost_{CB} \]
\[\hspace{0.8cm} \land\ cost_{AD} < cost_{CD}+ cost_{CB} + cost_{AB}\]
\[(soft)\ cost_{AD}==1\land cost_{AB}==2 \land cost_{CB}==3 \land cost_{CD}==4\ \]

A satisfied assignment is \(cost_{AB}==7\), while other link costs remain unchanged, then we modify the link cost of AB to 7 as the repair patch.


% %\emph{Dealing with conflicts among constraints.} 
% %As far as we're concerned, 
% However, a conflict may exist among SMT constraints for the $Prefer$ condition since edge cost is a positive integer and the number of variables on the left side of the inequality may be greater than the concrete value on the right side. 
% %For example, there are edge cost symbols $a$ and $b$, while we require $a+b<1$. 
% To solve this issue, we assign a larger cost to the concrete value. Since the concrete value must appear on the right side of the inequality, a larger cost won’t influence the result of other SMT constraints. In this way, we resolve the conflict and generate the final patch.

% Consider a new example after we fix the errors in the previous example: the new requirement is an underlay way-point requirement $(C_{1}, C_{3}, C_{3}, C_{1}C_{4}C_{3}, 0)$. We need to generate the $Peer$ condition for $(C_{3}, C_{4})$ and $(C_{1}, C_{4})$, along with $Prefer$ condition for $C_{1}$ and $C_{4}$. Then, during the selective symbolic simulation on the route propagation graph, we construct a constraint that $C_{1}$ prefers the route from $C_{4}$ to $C_{2}$ with symbols $a$ and $b$ to denote the edge costs of $(C_{3}, C_{4})$ and $(C_{4}, C_{1})$. The corresponding inequality is generated as $a+b<edge(C_{1}, C_{2}).cost+edge(C_{2}, C_{3}).cost$. Since the original cost values 10 and 10 do not satisfy the requirement, we turn to the SMT solver for solving $a$ and $b$.
% We notice that $edge(C_{1}, C_{2}).cost$ and $edge(C_{2}, C_{3}).cost$ are both 1. 
% In this situation, $a$ and $b$ cannot be assigned smaller than 1 anymore. 
% As a consequence, we increase $edge(C_{1}, C_{2}).cost$ or $edge(C_{2}, C_{3}).cost$, then call the SMT solver again to generate the solution until the inequality is satisfied. %In this way, we resolve the conflict in error diagnosis and repair.

%

%After that, when we add an additional requirement that C1 reaches C3 and specifies C4 as a waypoint(\ie, the way-point requirement mentioned above), in addition to generating conditions 1) $Peer(C_{1}, C_{2}, OSPF) = true$, 2) $Peer(C_{2}, C_{3}, OSPF) = true$, we also generate $Prefer$ condition for $C_{1}$ and $C_{4}$ and allocate variables $x$ and $y$ to edge $(C_{3}, C_{4})$ and $(C_{4}, C_{1})$. Then, through symbolic execution on the route propagation graph, we will construct a constraint that $C_{1}$ prefers the route from $C_{4}$ to $C_{2}$. The corresponding inequality is generated as $x+y<edge(C_{1}, C_{2}).cost+edge(C_{2}, C_{3}).cost$. \xing{replace x with another symbol, x denotes node before. And explain x and y}

% Computing route propagation paths for way-point requirements is more complex. It is insufficient to compute a $p_{packet}$ which matches the regular expression $P$. There could exist conflict between the calculated path and the existing ones. To avoid this, we calculate a set of route propagation paths $\{p_{i_1}, p_{i_2}, ..., p_{i_n}\}$ for each way-point requirement $i$. We then select a path for each way-point requirement (\eg, $\{p_{1_m}, p_{2_n}, ..., p_{k_q}\}$ if there are k way-point requirements for the network $n$) to check if the path won't conflict with paths that exist in the graph. 

% \para{Reachability violation diagnosis.} We diagnose reachability violations by calculating the shortest path between the source node and the destination node and guaranteeing that the OSPF peer adjacency between every two nodes on the path has been established. We first diagnose reachability violations since waypoint violations are more complicated and some waypoint violations may be satisfied after fixing the connection between peer nodes.

% In link-state protocol, every source node usually chooses the shortest path (the lowest cost) in its RIB as the best path to reach the destination. Once we verify and find that a requirement cannot be satisfied on the current data plane, we compute the shortest path for the source and the destination pair as the desired forwarding path on a graph. The graph is constructed based on the connection of L2 topology. The edge cost is assigned according to the interface configuration. In Figure \ref{fig: multi-protocol example}, we calculate the shortest path for each OSPF reachability requirement. As the shortest path of requirement 2 is a sub-path of requirement 1, we could merge 3 paths into 2 paths. We then generate the peer symbol of each two adjacent nodes on the path. The symbol indicates whether the OSPF adjacency between two nodes has been established. In the example, we will check symbol \textit{Peer}(C1, C2, OSPF), \textit{Peer}(C2, C3, OSPF) and \textit{Peer}(C4, C3, OSPF) accordingly. Since Batfish models the process of OSPF link state announcement like the path-vector one, the process of symbolic execution on OSPF is then similar to that of BGP symbol execution. We won't go into details.

% \para{Waypoint violation diagnosis.} Here's an additional constraint to the original requirement that packets have to traverse a waypoint C4 to reach p. The key to solving the waypoint violation is to first guarantee the reachability of the desired forwarding path and second, assign appropriate costs to the edges and ensure the route of the desired path is selected. Consequently, we introduce \textit{Peer} and \textit{Prefer} symbols to the symbolic execution process.

% We first compute a desired intent-compliant data plane for each destination prefix. A intent-compliant data plane consists of forwarding paths for all requirements with the same destination node. We aim to compute a desired forwarding path for each unsatisfied waypoint requirement. Meanwhile, ensure the original forwarding paths of satisfied waypoint requirements remain unchanged as much as possible. In concrete terms, we first compute a desired forwarding path set for each unsatisfied requirement according to the topology and the requirement. Then, we select one path from the set for each requirement and try to find a combination of these paths such that this combination does not conflict with the forwarding paths of the satisfied requirements. Otherwise, we may have to compute new paths for the satisfied requirements. As long as we could compute a desired intent-compliant data plane for the destination IP prefix, we argue that it would be able to modify the configuration to ensure that the waypoint requirements are satisfied. Conversely, we assume that the current requirements cannot be satisfied simultaneously. In the example network, we calculate a desired path (C1, C4, C3).

% Then we solve waypoint violations via symbolic execution. To make sure packets are sent through the correct forwarding path we compute for a specific requirement, we propagate two symbols (\textit{Peer} and \textit{Prefer}) along the opposite direction of the forwarding path (route propagation direction). The \textit{Peer} symbol ensures the destination node is reachable from the source node. The \textit{Prefer} symbol guarantees that the desired forwarding path is the shortest. We take the edge cost to edges in the desired forwarding path as variables. When a router A receives a route from its peer B, it adds \textit{cost}(B, \textit{p}) with \textit{cost}(A, B) where \textit{cost}(B, \textit{p}) is the cost from peer to the destination, and \textit{cost}(A, B) is the edge cost between peer and itself. For all nodes in the desired forwarding path, we construct a set of SMT constraints to ensure the \textit{Prefer} symbols are satisfied. We use \textit{Prefer} symbol to make sure that the route from the node downstream of the desired forwarding path has a lower cost compared to other routes in the RIB table. Thus the desired route will be selected and installed in the RIB. We then use the SMT solver({\eg}, z3) to solve for the concrete values of the edge cost variables. In the example network, we first allocate variables x and y to edge (C3, C4) and (C4, C1). We then construct a constraint that C1 prefers the route from C4 to C2. The corresponding inequality is x+y<1+1.




==> overview-v2.tex <==


% \begin{table}[t]
%   \centering
%   \begin{tabular}{c}
%     \includegraphics[width=\linewidth]{figures/boolean-condition-table.pdf}
%   \end{tabular}
%   \caption{The routing Boolean conditions.}
%   \label{tab: routing boolean conditions}
% \end{table}


\section{\system{} in a Nutshell}\label{sec:overview}
% \qiao{I am locking this section, please do not touch it.}

Figure \ref{fig:workflow} describe the architecture of \system{}. We use the same
example Figure~\ref{fig:example} to illustrate the key insight and basic
workflow of how \system{} accurately diagnoses and repairs network
configuration.

\iffalse{
given an erroneous data plane, the original configurations, and a set of
high-level routing intents, how \system{} diagnoses and repairs configuration
errors if the original configuration does not produce an intent-compliant data
plane.
}\fi

%\subsubsection{Basic Workflow}
%\label{basic_workflow}

\subsection{Contracts}\label{sec:contract}
A contract is a predicate that specifies the behavior of a router. 
To be concrete, a routing process, defined as a 2-tuple of device identifier and
routing protocol agent identifier, runs as an event-driven program. It receives
route updates (\eg, BGP route announcement and link-state announcement) and
processes them through a series of conditional statements. Each Boolean
condition in this program is a \textit{contract}. For example,
Figure~\ref{fig:BGP-program} gives the basic program of a BGP process, which consists of four
types of contracts: $isPeered$, $isImported$, $isPreferred$, and $isExported$.  

\para{Key observation: network configuration decides the values of contracts.}
Given a network configuration script, it does not change the structure of the
event-driven program, but only the value of its contracts. Take the route policy
of router $A$ in Figure~\ref{fig:example} as an example, it sets $isImported$ to be $false$
for all route announcements $A$ receives that have $W$ on the AS path. 

\iffalse{
To be concrete, a forwarding path $
[\ldots, R_{i-1},
R_{i}, R_{i+1}, \ldots]$ will exist in the data plane if and only if for each
router $R_i$, it peers with $R_{i+1}$, imports the route $[R_{i+1}, \ldots]$,
prefers it over other routes, and exports it to $R_{i-1}$. In other words, all
the routing Boolean conditions for $R_i$ to process the route $[R_{i+1}, \ldots]$
(\ie, $isPeered$, $isImported$, $isPreferred$, and $isExported$) must be $true$.
}\fi

\subsection{Workflow}\label{sec:workflow}
The basic workflow of \system{} consists of four steps: (1) find a set of
contracts that ensure an intent-compliant configuration; (2) 
simulate the original configuration symbolically and selectively to find all
possible violations of these contracts; (3) locate which part of the
configuration causes the violations as the errors; and (4) compute a conflict-free 
repair using constraint programming. We illustrate this procedure using the same
example in Figure~\ref{fig:example}.


\iffalse{
\para{From routing configurations to high-level routing Boolean conditions.}
%\para{Modeling routing configuration behaviors as Boolean conditions in a program.}
%\para{Modeling a routing process as a program with conditional statements.}
A routing process, defined as a 2-tuple of device identifier and routing
protocol agent identifier, runs as an event-driven program. 
It receives route updates (\eg, BGP route announcement and link-state announcement) and processes them through a series of conditional statements.


%\para{Routing configurations change the program's Boolean conditions.}
Our key observation is that routing configurations do not change the
structure of the program, but only change the value of its Boolean conditions. We call these
conditions \textit{the routing Boolean conditions}. 
We abstract the key phases of the routing process into four high-level routing Boolean conditions, as shown in Table~\ref{tab: routing boolean conditions}, to represent all routing behaviors.
For example, when router $A$
receives route\footnote{We refer to a BGP route by its AS path throughout this paper.} $[F, E, D]$, its configuration will set the
Boolean condition $isImported$ to be $true$. If it receives route $[B, W, D]$,
its configuration will set $isImported$ to be $false$.
}\fi

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/BGP-program.pdf}
    \caption{The BGP process.}
    \label{fig:BGP-program}
\end{figure}

\para{Step 1: Derive intent-compliant contracts from the intents and erroneous data plane.} 
%\para{Computing an intent-compliant data plane as reference from the erroneous
%data plane and the intent.} 
Motivated by recent network synthesis (\eg, Propane~\cite{beckett2016don} and
Contra~\cite{}) and verification tools (\eg, RCDC~\cite{} and Tulkun~\cite{xiang2023beyond}),
we derive intent-compliant contracts from an intent-compliant
data plane. A strawman to find such a data plane is to express intents in a regular expression
and multiply it with the topology. Although it works, the resulting data plane
could be very different from the one yielded by the original erroneous
configuration. If we derive contracts from this data plane and use them to
guide the diagnose and repair, it could result in a large number of changes of
lines in the configuration.

\iffalse{
Instead of computing an intent-compliant data plane
purely from the intent and the topology, \eg, Propane\cite{beckett2016don}, 
}\fi

With this in mind, we reuse the intent-compliant part of the erroneous data
plane from the original configuration as a starting point, compute an
intent-compliant data plane with a small difference from the erroneous one, and
use it to derive intent-compliant contracts. Our intuition is the smaller the
change in the data plane, the less contract violations in the configuration, and
the less lines in the configuration need to be updated. Specifically, we use a
regular expression to encode only \textit{unsatisfied intents} and multiply it
with the topology. We use all intent-compliant paths in the erroneous data plane
to guide the multiplication such that the valid paths found for unsatisfied
intents use these existing ones as segments as much as possible. 

In the example in Figure~\ref{fig:example}, router $B$, $E$, $F$ and $W$ each has an
intent-compliant path, but $A$ does not. We multiply the waypoint intent of $A$
(\ie, $A .^* W .^* D$ and loop-free) with the topology, and uses the paths of
other routers as guidance constraints. In the end, we get an intent-compliant data plane
in Figure~\ref{fig:workflow-a} \qiao{we don't know how to use subfigure???} 
with only one link different from the erroneous data plane.

\para{From an intent-compliant data plane to intent-compliant contracts.}
The reverse of the data plane computed above (\ie, changing the direction of all
links) provides a set of \textit{sufficient and necessary} conditions for the
routers to yield it. We call them the \textit{intent-compliant contracts}.  To
be concrete, a forwarding path $ [\ldots, R_{i-1}, R_{i}, R_{i+1}, \ldots]$ will
exist in the data plane if and only if for each router $R_i$, it peers with
$R_{i+1}$, imports the route $[R_{i+1}, \ldots]$, prefers it over other routes,
and exports it to $R_{i-1}$. In other words, when $R_i$ processes the route
$[R_{i+1}, \ldots]$, all its contracts (\ie, $isPeered$, $isImported$,
$isPreferred$, and $isExported$) must be $true$. Figure~\ref{fig:workflow-b} lists the
intent-compliant contracts of this example. \qiao{add a figure for this.}



\iffalse{
We then use a dedicated algorithm to multiply the regular expressions of the
rest of the unsatisfied intents with the topology, to find an intent-complaint
data plane, while maximally preserving the existing intent-complaint paths.


In the erroneous data plane in Figure~\ref{fig:example}, router $B$, $E$, and $W$ each has an
intent-compliant path. Although $A$ appears to have a valid path, it uses 
the non-compliant path of $F$ as a subpath. As such, $A$ does not have an
intent-compliant path in the erroneous data plane.
We multiply the regular expression of the unsatisfied intent of $A$ with the topology, with the paths of $F$, $E$, $B$, $W$ as prune constraints, to find the intent-complaint path of $A$. In the end, we get an intent-compliant data plane in
Figure~\ref{fig:workflow}(a) with only one link different from the erroneous data plane.

\para{From the reference data plane to reference intent-compliant routing contracts.}
The reverse of the reference data plane (\ie, changing the direction of all
links) provides a set of sufficient and necessary contracts for the routing
process to yield it. We call them the \textit{the reference routing contracts}.
To be concrete, a forwarding path $ [\ldots, R_{i-1}, R_{i}, R_{i+1}, \ldots]$
will exist in the data plane if and only if for each router $R_i$, it peers with
$R_{i+1}$, imports the route $[R_{i+1}, \ldots]$, prefers it over other routes,
and exports it to $R_{i-1}$. In other words, all the routing Boolean conditions
for $R_i$ to process the route $[R_{i+1}, \ldots]$ (\ie, $isPeered$,
$isImported$, $isPreferred$, and $isExported$) must be $true$.
}\fi

\para{Step 2: Simulate the configuration to identify all possible violations of
the intent-compliant contracts.}
We start an iterative simulation of the original configuration. At each step,
for each router, we examine the values of its contracts. If they are different
from the values of the intent-compliant contracts, we record this violation,
force the router's behavior to obey the intent-compliant contracts, and continue
the simulation. As such, the simulation switches to a symbolic variant of the
original configuration.  In the end, the simulation yields the intent-compliant
data plane in Step 1 as the output because (1) the whole simulation follows the
intent-compliant contracts as invariants, and (2) the latter are the sufficient
and necessary conditions for generating the intent-compliant data plane. 

Figure~\ref{fig:workflow} \qiao{FIX IT, PLEASE!} shows the simulation of our
example. At one step, when $A$ receives $[B, W, D]$, the original configuration
decides that $A$ will set the corresponding $isImported$ to be $false$, while in
the intent-compliant contracts, this contract should be $true$. Therefore, we
force the simulation to obey the intent-compliant contracts and as a result, $A$
selects $[A, B, W, D]$ as its path. In the next step, when $F$ receives route
$[A, B, W, D]$, $F$'s configuration would set $isPreferred$ of this route to be
$true$.  However, the intent-compliant contracts require $F$ sets $isPreferred$
of $[E, D]$ to be $true$, contradicting the original configuration. We again
force the simulation to follow the intent-compliant contracts and as a result,
$F$ keeps $[F, E, D]$ as its path, instead of $[A, B, W, D]$. In the end, each
router selects the path underlined in the Figure.

\begin{figure*}[!htbp]
  \centering
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/workflow-a.pdf}
    \caption{Computing an intent-compliant data plane for the erroneous data plane.}
    \label{fig:workflow-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/workflow-b.pdf}
    \caption{Generating the intent-compliant contracts from the intent-compliant data plane.}
    \label{fig:workflow-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/workflow-c.pdf}
    \caption{Identifying all contracts violation via selective symbolic simulation.}
    \label{fig:workflow-c}
  \end{subfigure}
  \caption{The workflow of \system{}.}
  \label{fig:workflow}
\end{figure*}


% \para{Comparing the differences between actual and reference routing Boolean
% conditions to localize the errors.}
\para{Step 3: Examine violated contracts to localize configuration errors.}
For each violated contract, we analyze the configuration to determine which
snippets causes the violation. In our example, two contracts are violated. In
the first one, $A$ sets $isImported$ of $[B, W, D]$ to be $false$. We find that
it is because of the policy of $A$ that discards all routes containing $W$. In
the second one, $F$ sets $isPreferred$ of $[A, B, W, D]$ to be $true$. We find
that it is because of the policy of $F$ that sets a higher local preference of
routes with $A$ as the next hop \qiao{add line XX back}. Both snippets are consistent with the ground
truth presented at the beginning of our experiment (\S\ref{sec:limitations}). 

\para{Computing conflict-free repair patches using constraint programming.}
\qiao{not done.}
Repairing the error requires computing a patch that sets the different routing Boolean conditions to the reference ones 
% without affecting the other actual conditions set by the erroneous configurations.
without affecting other actual conditions, which satisfy the reference.
We model this as a constraint-solving problem to compute a satisfiable assignment for the erroneous configurations. 
% Except for the peering condition, which can be fixed directly (just enable the peer routing).
% except for peering errors, which 
% We repair the error by computing a patch that correctly sets the routing Boolean conditions, which differ from the reference ones, without affecting the other actual conditions for the erroneous configuration.

In this example, erroneous configuration $policyA$ controls two routing Boolean conditions, \ie, $isImported$ for the route $[B,W,D]$ and the route $[F,E,D]$. We let the first condition be set $true$ as the reference one suggests and keep the second condition to $true$. Thus we change the $deny$ at line 3 to $permit$ as a repair.
% $policyF$ sets routing Boolean condition $isPreferred$, denote as $(60>200)$, where $60\ (200)$ is the local-preference of route from $E\ (A)$, to be $false$. 
$policyF$ sets routing Boolean condition $isPreferred$, denote as $(60>200)$, to be $false$ (where $60\ (200)$ is the local-preference of route from $E\ (A)$).
A satisfiable assignment that lets $isPreferred$ be $true$ is $(60>50)$, where $50$ is the local-preference assigned to the route from $A$. The repaired configurations are shown in Figure \ref{fig: repaired-cfgs}.




% Because the routing Boolean condition
% $isImported$ for route announcement of AS path $[B, W, D]$ is set $false$ in the original
% configuration while the reference condition sets it $true$, 
% the configuration lines X-X in the configuration of router $A$ that filter all AS paths containing $w$ are identified as errors. 
% Similarly, lines X-X in the configuration of router $F$ that set a higher local preference on routes from next-hop $A$ are also errors because the reference routing Boolean condition requires $F$ to prefer the route formed along path $[E, D]$ (from next-hop $E$) over all other routes.  



%Use the intent-compliant contracts to selectively simulate variants of the original configurations.}

\iffalse{
Starting from a simulation of the original configurations, 
every time we encounter a conditional statement whose value is specified by the reference contract, 
if the actual condition value is different from the reference one, 
we deem this contract violated and force it to obey the reference condition and continue simulating.
Thus, we can simulate variants of the original configurations, without truly modifying low-level configuration languages during the simulation, to form the intent-complaint data plane. 
% which can track subsequent routing conditions could be triggered by this one.


Figure~\ref{fig:workflow}(b) shows the simulation process with the best routes
underlined. In the original configurations, router $A$ will receive route $[B,
W, D]$ and set its $isImpored$ to $false$.  However, the reference contract
specifies that this routing condition should be $true$.  Therefore, we continue
simulating a variant of the original configurations, as the reference contract
indicates.  Thus $A$ can choose $[A, B, W,D]$ as the best route and send it to
its neighbors (getting $r_6$).  Similarly, when $F$ determines whether to prefer
$r_4$ over $r_6$, the actual routing condition violates the reference one, so we
follow the reference one to simulate (getting $r_7$).  



% \para{Comparing the differences between actual and reference routing Boolean conditions to localize the errors.}
\para{Using violated contracts to localize configuration errors.}
By simulating variants of the original configurations following the intent-complaint contracts, we can eventually find a symbolic variant representation (Figure~\ref{fig:workflow}(c)), where the violated contracts indicate erroneous routing conditions.
Leveraging the observation that routing configurations decide the value of
routing Boolean conditions, 
we localize the configuration errors as lines in the original configurations that set the
violated routing Boolean condition values.  


In this example, we identify $A$'s configuration lines 3-4 that filter all AS paths containing $W$ as errors. 
Similarly, lines 1-3 in the configuration of router $F$ that set a higher local preference on routes from next-hop $A$ are also errors because the reference routing contract requires $F$ to prefer the route $[F, E, D]$ over all other routes.
% Because the routing Boolean condition
% $isImported$ for route announcement of AS path $[B, W, D]$ is set $false$ in the original
% configuration while the reference condition sets it $true$, 
% the configuration lines X-X in the configuration of router $A$ that filter all AS paths containing $w$ are identified as errors. 
% Similarly, lines X-X in the configuration of router $F$ that set a higher local preference on routes from next-hop $A$ are also errors because the reference routing Boolean condition requires $F$ to prefer the route formed along path $[E, D]$ (from next-hop $E$) over all other routes.  


\para{Computing conflict-free repair patches using constraint programming.}

Repairing the error requires computing a patch that sets the different routing Boolean conditions to the reference ones 
% without affecting the other actual conditions set by the erroneous configurations.
without affecting other actual conditions, which satisfy the reference.
We model this as a constraint-solving problem to compute a satisfiable assignment for the erroneous configurations. 
% Except for the peering condition, which can be fixed directly (just enable the peer routing).
% except for peering errors, which 
% We repair the error by computing a patch that correctly sets the routing Boolean conditions, which differ from the reference ones, without affecting the other actual conditions for the erroneous configuration.

In this example, erroneous configuration $policyA$ controls two routing Boolean conditions, \ie, $isImported$ for the route $[B,W,D]$ and the route $[F,E,D]$. We let the first condition be set $true$ as the reference one suggests and keep the second condition to $true$. Thus we change the $deny$ at line 3 to $permit$ as a repair.
% $policyF$ sets routing Boolean condition $isPreferred$, denote as $(60>200)$, where $60\ (200)$ is the local-preference of route from $E\ (A)$, to be $false$. 
$policyF$ sets routing Boolean condition $isPreferred$, denote as $(60>200)$, to be $false$ (where $60\ (200)$ is the local-preference of route from $E\ (A)$).
A satisfiable assignment that lets $isPreferred$ be $true$ is $(60>50)$, where $50$ is the local-preference assigned to the route from $A$. The repaired configurations are shown in Figure \ref{fig: repaired-cfgs}.
}\fi




\iffalse{
 (\eg,
import filter, route ordering and selection, and export filter). \qiao{needs a
figure as Minesweeper encoding to show that.}
}\fi



\iffalse{

The routing process's configuration essentially determines the specific values
of these branching conditions. \qiao{prefer?}

\qiao{use table to list all Boolean configuration variables, including 4
routings and 1 ACL} 

to update its internal state (\eg, RIB and link state database), and
then sends messages to neighboring processes (\qiao{?}). 

A routing process, defined as a 2-tuple of device identifier and routing
protocol agent identifier, runs as an event-driven program with branching
conditions. Its configuration determines the specific values of these branching
conditions. To be concrete, we abstract the key (4) phases 



\para{From non-compliant data plane to intent-compliant route propagation graph
(RPG).} 
Given an intent and a non-compliant data plane, \system{} first designs a
heuristic algorithm to compute an intent-compliant data plane, and then reverse
it to get an intent-compliant route propagation graph. Specifically, the
algorithm works in four steps: (1) constructing the set of all intent-compliant paths from the
non-compliant data plane; (2) computing a product graph to represent all
intent-compliant paths in the topology; and (3) for each non-compliant path in
the non-compliant data plane, find an intent-compliant alternative that does not
conflict with existing intent-compliant paths, \ie, each node has at most one
next-hop node; \qiao{Is step (2) even necessary? at most one next-hop or one
incoming node?} and (4) aggregating all intent-compliant paths from (1) and (3)
into a graph and reverse it to get the intent-compliant route propagation graph. 



\para{Using RPG as constraints to simulate configuration variants selectively.}


\para{Comparing the differences between the original configuration and
intent-compliant variant to localize errors.}


\para{Computing conflict-free repair patches using constraint programming.}







Given an intent, \system{} first leverages the automata theory~\ref{} to compute
a product graph to represent all intent-compliant paths in the topology.
It then adopts a greedy algorithm to construct a in-tree consisting of all
intent-compliant paths in the data plane and 
}
\fi

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/BGP-program.pdf}
%     \caption{The BGP process.}
%     \label{fig:BGP-program}
% \end{figure}



























==> overview.tex <==

\section{Overview}
\label{sec:overview}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/sse-simple-example.png}
    \caption{The comparison of the full symbolic execution (SE) and selective symbolic execution (SSE).}
    \label{sse-simple-example}
    \vspace{-1em}
\end{figure} 
% In this section, we first introduce and then introduce \system{}'s architecture.

\subsection{A Primer on Selective Symbolic Execution}

\para{Full symbolic execution does not scale.} As a means to improve the coverage of program testing, symbolic execution assumes symbolic values for inputs, so that each symbolic execution path of a program can represent many concrete executions with the same execution path. However, symbolic execution suffers from the \textit{path explosion} problem, where the number of symbolic execution paths increases exponentially with an increase of the number of branching conditions in the program. For example, in the program snippet in Figure~\ref{sse-simple-example}, there are $2^{n}+2^{m}$ symbolic execution paths. 

\para{Selective symbolic execution (SSE): only exploring symbolic execution paths of interest.} SSE allows users to specify a set of constraints \qiao{I use 'constraint' here.} on inputs and branching conditions of the program, so that only symbolic execution paths satisfying such constraints will be explored. In other words, it provides a full coverage on symbolic execution paths of interest rather than the exponential number of all paths, substantially improving the scalability of symbolic execution. Consider the same example in Figure~\ref{sse-simple-example}. If the user specifies a constraint $x\ge 0 \land x<9$, SSE only explores $2^{m-1}$ symbolic execution paths instead of $2^{n}+2^{m}$ ones. 

\para{Challenge of SSE: how to specify the right constraints to explore?} \qiao{stop here.}  



\iffalse{
Symbolic execution~\cite{king1976symbolic} is a powerful technique that helps analyze program behavior, find bugs, and generate tests. The key idea is to use symbolic variables to track the private conditions that form each path to explore all program paths exhaustively. The symbolic execution forks a new path every time the execution reaches a branch whose condition satisfies both the "true" and "false" branches, forming an execution tree, as the SE execution tree in Figure~\ref{sse-simple-example} shows. However, it suffers from the \textit{path explosion problem, \ie, the size of the tree grows exponentially with the number of condition statements}, which is a primary obstacle in scaling it to large systems.

Selective symbolic execution~\cite{chipounov2009selective, stephens2016driller} is a powerful optimization designed to scale up symbolic execution by symbolically executing only the selected portion of the program. Specifically, it allows users to \textit{specify a set of conditions} to determine which branches must be searched and which can be pruned.
Each condition is a logical constraint that the paths must satisfy, thus guiding the exploration to focus only on the space of interest.
Figure~\ref{sse-simple-example} illustrates how much selective symbolic execution can improve efficiency. The example program consists of $(n+m)$ if-else statements, with only line 2 modifying the value of $y$.  
Given an input range for $x$ (\eg, $x = 10$) that could lead the program to always go to the "else" branch, it will eventually reach the assertion $y < 10$, triggering the bug (\eg, with $y=12$ for $x=10$).
The full symbolic execution, in the worst case, needs to explore $2^n+2^m$ paths to find the error. However, if we choose to execute only the paths following the "false" branch of $x<0$ and the "false" branch of $x<9$, \ie, specify the condition as $x\ge 0 \land x<9$, we can reduce the path search space to $2^{n-1}$. In the best case, the error can be found in $O(1)$ complexity by specifying a condition that allows the execution to always go to the "false" branch. 
}\fi




% It is a hybrid technique that improves efficiency by combining the strengths of symbolic and concrete execution. The central idea enabling symbolic and concrete execution to coexist is to keep both the concrete and symbolic store (\ie, program states) and path constraints.
% When switching to symbolic execution, concrete execution can guide symbolic execution, allowing the system to run with actual inputs while maintaining symbolic information.


% \begin{lstlisting}[language=C, numbers=left, stepnumber=1, numberstyle=\tiny\color{gray}]
% void func(int x, int y)
%   int z = 2 * y
%   if (z == x) {     
%     if (x > y + 10) 
%       assert ERROR
%   }
% }
% \end{lstlisting}





           

% We use a simple example in Figure~\ref{sse-program-example}(a) to illustrate how selective symbolic execution works. The $func(x, y)$ takes two int numbers as input, and a bug will be triggered when the program executes to line 7. To quickly explore the path that reaches the bug, we select lines 5-8 to perform symbolic execution while the rest do concrete execution. The program starts with a concrete input, suppose we read x=9 and y=2. At point \textcircled{1}, we have z=4, and its symbolic value is 2*y0, so now we will take the "else" branch of z<0, and also add 2*y0 to the path constraint. When executed to point \textcircled{2}, the concrete execution will follow the "else" branch of z==x to reach point \textcircled{3},


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/revise-arc.png}
%     \caption{The architecture of \system{}. The black lines indicate the original verification process, and the yellow lines indicate the diagnosis and repair process beyond verification.}
%     \label{scalpel-arc}
%     \vspace{-1em}
% \end{figure} 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/receive-pseudocode.pdf}
    \caption{A simplified BGP routing process program.}
    \label{fig:BGP-program}
\end{figure}  

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/canimport-program.png}
%     \caption{The pseudocode of router B imports a route with the deny\_AS3 policy shown in Figure~\ref{fig:example}.}
%     \label{fig:enter-label}
% \end{figure}                                                                 


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/revise-sss.pdf}
    \caption{The intent-complaint configuration variant exploration.}
    \label{sss process}
    \vspace{-1em}
\end{figure*}



\iffalse{

\subsection{Workflow of \system{}}

% \system{} builds upon the core idea of selective symbolic execution while adapting it for the network simulation program to diagnose and repair the configuration error. 



\system{} works as a companion of simulation-based configuration verification tools (\eg, \cite{fogel2015general, brown2023batfish, lopes2019fast, quoitin2005modeling, liu2017crystalnet}). Given a set of forwarding requirements (\ie, the path regular expression), when verification ends with detecting unsatisfied requirements, \system{} will automatically conduct the after-verification diagnosis and repair. 

At a high level, \system{} consists of three steps: (1) generating the constraints that guide the exploration during the simulation; (2) simulating the network to find the intent-compliant configuration representation; (3) computing the patches to repair the error. We first use the BGP network in Figure~\ref{fig:example} to demonstrate these three steps. We then introduce how \system{} extends to support multiple protocol networks in \S\ref{multi-protocol section} and handles k-link failure tolerance in \S\ref{k-failure section}.
% select configuration variants (S1-S2) to symbolically re-simulate (S3) to diagnose (S4) and repair (S5) the configuration error in five steps: 
% Figure \ref{sss process} gives the overall architecture of \system{}. 
% Router configuration defines . It receives events (\eg, routing messages and topology change), updates its internal states (\eg, RIB), and sends routing messages to neighboring routing processes. 

% \begin{table}[t!]
%   \small
%   \centering
%   \begin{tabular}{p{2.7cm}|p{5cm}} %p{5.3cm}|p{11.5cm}
%     \hline
%     Boolean variable & Description \\
    
%     % \hline
%     % $\{attr_1, attr_2, ...\}$ & Represent a set of routes that match corresponding $attr_1$ and $attr_2$ attributes as the set specified.\\
    
%     \hline
%     $peer(n, m)$ & Do protocol instances $n$ and $m$ successfully establish peer session. \\

%     \hline
%     $canExport(u \rightarrow v, r)$ &  Can routing process $u$ export route $r$ to routing process $v$ successfully. \\

%     \hline
%     $canImport(u \leftarrow v, r)$ & Can routing process $u$ import route $r$ from routing process $v$ successfully.\\

%     \hline
%     $prefer(r_1, r_2)$ & Is route $r_1$ preferred to $r_2$. \\
     
%     \hline
%   \end{tabular}
%   \caption{Router behavior variables.}
%   \vspace{-1em}
%   \label{tab:router behavior}
% \end{table}




\para{S1. Constraint generation.}
We first abstract the router configuration, which controls how each routing process exchanges advertisements with neighbors and computes paths, into four Boolean \textit{router behavior variables}. As Table~\ref{tab:router behavior} shows, it includes peering, importing/exporting a route, and selecting a route. We represent the constraint with the four variables and only explore the branches where the constraint is satisfied.

% % To automatically generate the constraints that could lead the simulation to execute to a point where the network state meets all intents. 
% We compute an intended forwarding graph for the intents that are destined for the same prefix. Then transform it into the routing graph to generate the constraints that form this routing graph. The edges of the forwarding graph indicate each node's intended next hop to reach a specific destination prefix, while the reverse edges in the routing graph indicate the propagation of corresponding best routes. 





Then we reverse the forwarding graph to get the routing graph\footnote{Generall, reversing edges hop-by-hop is feasible, but there could be a little difference in multiple-protocol networks, this will be discussed in \S\ref{multi-protocol section}.}, which indicates the necessary route propagation and selection of each routing process, as Figure~\ref{sss process}(c) shows. 
We use two well-known mandatory BGP attributes\footnote{The two attributes may be modified during the route propagation, we discuss the solution in Appendix~\ref{appendix}.} that can be computed from the routing graph to indicate a set of best routes we intend to select at each node, \eg, BEST$_A$=\{10/8, [3,1], W\} represents the routes whose AS\_PATH matches $[3,1]$ and NEXT\_HOP matches $W$ should be the best route of \(A\). 
We define constraints on the four router behaviors to represent how the routing graph forms. 
The edge indicates the $peer, canImport$, and $canExport$ conditions that should be specified to propagate the intended route, and we use the $perfer$ condition to specify the route we intend to select at each node. 
Figure~\ref{sss process}(d) shows parts of the conditions.
For example, $A\rightarrow B$ indicates: (1) A and B must peer with each other, \ie, $peer(A, B)$ holds, (2) for each route $r$ sent to B, if it matches BEST\_A, it should be successfully exported, as condition (1) shows, (3) for each route $r$ received from A, if it matches BEST\_B, it should be successfully imported, as condition (2) shows. Also, C should prefer the route from neighbor E, which also matches BEST\_C, to routes from all other neighbors W and B, as conditions (3)-(4) show.



% To achieve this, we introduce the \textit{route propagation graph} (RPG) to help select the appropriate portion of the configuration for symbolic simulation.
% An abstract representation indicates how route propagation processes form an intent-compliant forwarding graph.



% We then derive a set of rules from the RPG to guide the selective symbolic simulation.
% We represent configurable router behaviors using four types of boolean variables (\ref{subsec: 4.1}). Such that we can generate a set of quantified formulas over these variables, indicating the rules (\eg, Figure\ref{sss process}(d)) that intended configuration variants should follow. 


% prune unnecessary searching space. 




\para{S2. Selective symbolic simulation.}
We then simulate the route propagation process to achieve the routing graph symbolically. The distributed routing process updates its RIB when it receives new messages and sends them to its neighbors. In well-behaved networks, the routing process will converge to a stable state~\cite{griffin2002stable} in which all routing processes do not change their route selections upon receiving routing information.  
We associate each route with a condition to track its execution path. 
The key to symbolically exploring the intended configuration is that we always \textit{select to explore the path that satisfies the routing graph condition at each conditional branch} during the simulation. That is, if the actual branch that the simulation would take (\ie, the decision controlled by the given configuration) breaks the condition, we will force the simulation to take the branch that meets the condition. For simplicity, we only show the broken conditions in the following example.

Figure~\ref{sss process}(e)-(f) shows part of the selective symbolic simulation process and the simulated RIBs. Each route is represented as a 4-tuple $(n, as\_path, next\_hop, condition)$, with the best route underlined. At the start, D sends its route $r_0$ to E and W. E and W receive the route and select it as their best routes, $r_1$ and $r_2$. Then, E sends $r_1$ to C, and C selects it as the best route $r_3$, while W sends $r_2$ to A and C, getting $r_4$ (best route) and $r_5$ (since $r_3$ is preferred to $r_5$ due to the lower neighbor address), respectively. Until now, there has been no actual condition decision that breaks the routing graph condition. 
Next, A sends $r_4$ to B, as Figure~\ref{sss process}(e) condition branch 1 ($canExport(r_4, A\rightarrow B)$) shows. The given configuration would go to the "true" branch and still comply with condition (1) in Figure~\ref{sss process}(d). 


However, when the simulation comes to condition branch 2 ($canImport(r_6, A \rightarrow B)$), \ie, B receives $r_4$ as $r_6$ (appends its AS number). The actual decision is to drop $r_6$, since AS6 will deny all routes whose AS\_PATH contains the number 3 due to the deny\_AS3 policy (Figure~\ref{fig:example}(b)), which violates condition (2). So we force the simulation to go to the "true" branch of condition branch 2, \ie, let B import $r_6$, and also attach the symbolic variable $c_2$ to $r_6$, indicating that $r_6$ could exist in B's RIB only if $c_2$ is true.


Then, C imports $r_6$ from B and sets a local preference of 200 for the route, obtaining $r_7$ (the prefer\_AS6 policy). When C updates its best route, \ie, comes to condition branch 3 that determines if $r_3$ is preferred to $r_7$, the actual decision is false since $r_7$ has the higher local preference. 
However, as the routing condition (3) specified, $r_3$ ($r_7$) is in RIB-in.E (RIB-in.B), \ie, imported from the routing process E (B), and $r_3$ matches BEST$_3$, which implies that $prefer(r_3, r_7)$ needs to hold. Therefore, we select to explore the "true" branch as the routing condition indicates. As such, C still selects $r_3$ as the best route with the condition $c_2\land c_3$, and sends it to all its neighbors, thus getting $r_8, r_9, r_{10}$. So far, all routing processes have converged, and we reach a stable state, as Figure~\ref{sss process}(f) shows, where each node computes the intended best route as the routing graph indicates (Figure~\ref{sss process}(c)).


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/repaired-config.png}
    \caption{The repaired configuration of the example network. Red lines represent the error configuration, and blue lines represent the patch.}
    \label{fig: repair result}
    \vspace{-1em}
\end{figure} 


\para{S3. Configuration error diagnosis and repair.} 
The selective symbolic simulation will eventually result in at least one execution path where all routing conditions encountered in this path hold as specified by the routing graph. As the (origin) and (intended) paths in Figure~\ref{sss process}(f) show. 
These conditions of the intended path also indicate the routing behaviors an intended configuration must hold. Such that the broken conditions, \ie, those where the given configuration does not hold, are the root cause of the intent violation. We then map them to the original configuration files to pinpoint the specific error lines. In the above example, we find Err1 and Err2, and Figure~\ref{fig: repair result} shows the corresponding error lines.

Fixing the configuration error requires computing side-effect-free patches that satisfy the broken conditions while preserving the unbroken conditions.
We handle path-vector-based routing protocols, such as BGP, with a customized patch generation method. Figure~\ref{fig: repair result} shows one of the feasible patches, \ie, adding a rule at the top of the route policy for the specific route. The correctness of our repair approach has been demonstrated (\ref{sec:diag-repair}). For link-state-based protocols, such as OSPF, we compute the patch through a constraint-solving method (\ref{subsec:ospf}).

}


==> sse.tex <==
% \vspace{-1em}
\section{Control-Flow Diagnoser} \label{sec:control-flow}

\begin{figure}[t]
    \centering
    \includegraphics[width=240pt]{figures/sse.pdf}
    \small 
    \vspace{-1em}
    \caption{Symbolic execution of the example network.}
    \label{fig:sse}
    % \vspace{-0.12in}
\end{figure}

We leverage control flow analysis to diagnose unobservable errors. This is because the route computation data flow of such errors is usually \textit{unobservable} (\eg, the route propagation will terminate prematurely once the target route is filtered by the origin redistribution process). We view the data plane computation as a program that consists of route propagation and computation and is controlled by network configurations. Symbols of the program are router decisions such as the delivery of routes and the transformation of routes. Configuration errors that contribute to the deviations of router decisions will not surprisingly result in incorrect route computation outputs (\ie, incorrect forwarding behaviors of routers). So our goal is to find \textit{a minimal decision deviation set} by symbolically executing the data plane computation to localize configuration errors. 

We use the same network topology in Figure \ref{fig:crg}(a) to present details. Assume there are multiple errors: (1) D has not configured the network command to redistribute the target route to its BGP process, (2) S filters route to $T1$ from both peers A and B. The requirement is: $T0$ and B should reach $T1$. % 

% Different combinations of router decisions will lead to different computation results. 

% \vspace{-1.4em}
\subsection{Selective Execution Conditions}
 
We efficiently execute the symbolic data plane computation using selective execution conditions to avoid exploring huge execution path space. 
We first introduce how to generate such conditions using the forwarding tree representation. 
Each forwarding tree is a directed graph toward a prefix that specifies the forwarding paths of all nodes.
% with the following properties: (1) there is only one root node without out-neighbors where the prefix originates from; (2) all nodes except the root node have one and only one out-neighbor. 
The reversal of it indicates the route propagation and selection conditions that nodes need to comply with. We construct such a tree based on previous causal relationships to avoid incurring unnecessary interference.
Specifically, we first keep existing policy-compliant paths in the tree. Second, we complete paths for remaining source nodes that do not satisfy requirements.
Figure \ref{fig:sse}(a) shows the forwarding tree of the network: node S and node B forward traffic to $T1$ along with path S-A-D and path B-D respectively.

% Specifically, first, we keep existing paths that satisfy requirements unchanged: if a router already has a policy-compliant path $p$ to reach the destination prefix, add it to the tree. Second, we complete source nodes that do not satisfy requirements: if a router did not have a policy-compliant path to the destination, we assign one of the policy-compliant paths for it without conflicts with other nodes. Figure \ref{fig:sse}(a) shows the forwarding tree of the network: node S forwards traffic from $T0$ to $T1$ along with S-A-D, and node B reaches $T1$ through B-D.

%We define four types of conditions to compute the deviation of router decisions to localize errors: 


\para{Priority condition for route selection.} 
To ensure that each node $i$ eventually follows the path in the forwarding tree to propagate traffic, we use prefix, next-hop, and as-path attributes to identify the target route for node $i$.
The priority condition is that $i$ always chooses the target route as the best route (\ie, has the highest priority) for the destination prefix.
% an abstract condition for each node in the forwarding tree except for the root node, it does not explicitly specify the priority of concrete routes and will be triggered on demand during symbolic execution.  

% We use several attributes to identify the target route: (1) the next-hop of the target route is the out-neighbor of $i$ (we consider the entry iBGP node that is in the same AS with $i$ along the path as the next-hop of $i$ if $i$'s out-neighbor is its iBGP peer), (2) the network of the route is the destination prefix, (3) the as-path of the route is consistent with the actual as-path along the forwarding path (for the BGP route). The priority condition is an abstract condition for each node in the forwarding tree except for the root node, it does not explicitly specify the priority of concrete routes and will be triggered on demand during symbolic execution.  

\para{Export condition for route delivery.} 
Each node $i$ is obligated to propagate the route to its in-neighbors so that its in-neighbors can receive the target route. 
% The export condition guides the propagation of the target route. Once a node $i$ received a target route $r$ from its out-neighbor, based on the priority condition, $i$ will choose $r$ as the best route. 
Additionally, if node $i$ adjacent to its out-neighbor $n_{out}$ and in-neighbor $n_{in}$ uses different protocols, node $i$ needs to redistribute the target route to the routing processes of nodes $i$ and $n_{in}$.

\para{Import condition for route delivery.} The import condition follows the same intuition as the export condition: ensuring the target route is delivered to the corresponding node in the forwarding tree. Specifically, node $i$ has to receive the target route from its out-neighbor rather than filter it. If a node has no out-neighbor, the condition for it is to filter all routes from adjacent peers.

\para{Adjacency condition between routers.} The adjacency condition is a pre-condition for route deliveries between routers. We define the adjacency condition for nodes that have out-neighbors in the forwarding tree as the node needs to establish the peer session with its out-neighbor.

\begin{figure}[t]
	\centering
		\centering
		\includegraphics[width=0.48\textwidth]{figures/CRG-MUC-inline.png}
\caption{\small{Running time on diagnosing observable errors.}}
	\label{fig:observable-latency}
% \vspace{-1cm}
\end{figure}


% \vspace{-1em}
\subsection{Symbolic Data Plane Computation}
We define four types of conditions (\ie, router decisions) as symbols when executing them. These conditions are the abstraction of router decisions that are sufficient to result in one of the error-free data planes towards the prefix.
To improve efficiency, we do not keep all execution paths triggered by the above conditions. We tend to always guard the newest execution path that satisfies all conditions in this way: once a condition is triggered and the actual router decision deviates from it, we enforce the condition satisfiable and record it as the deviation condition of this path, and then continue to execute the computation. 
% For efficiency, we do not preserve all deviation paths (it means there already has a deterministic deviation of conditions) triggered by the above conditions since they are most likely to lead to errors too. We tend to always guard the newest execution path that satisfies all conditions in this way: Once a condition is triggered and the actual router decision is deviating from it, we make the condition satisfies forcibly and record it as the deviation condition of this path then continues to execute the computation.   
Figure \ref{fig:sse}(b) shows the correct execution path that results in the same data plane as the forwarding tree. We only symbolically execute two symbols during the computation: export and import decisions on nodes D and B, respectively (the purple and pink branches). We forcibly assign them the true values so that the divergences are the deviations of router decisions.  
% The non-deterministic decisions could lead to  
% \rulan{the correct path trace how a desired computation executes}
% to conduct selective symbolic execution during data plane computation. 
% When executing these conditions, we view them as a symbol to 

% \para{Carrying conditions in routes.}


% \vspace{-1em}
\subsection{Configuration Error Localization}
After symbolic data plane computation converges, each route carries these symbols to represent its existing conditions (concrete conditions), as shown in Figure \ref{fig:sse}(a).
The symbolic conditions are the minimal deviation set of router decisions that indicates the causes of the error. We map their keywords to defined types and localize configuration errors.
% such that we can know how to ensure the desirable route being computed during data plane computation: make the symbolic conditions satisfied. 
% Then we can get a 
 



% \para{Computing the minimal decision deviation set.}


==> sss.tex <==


\section{Basic Design}
\label{sec: sss}

We now present details on how \system{} diagnoses and repairs configuration errors. We use the path vector-based protocol (e.g., Border Gateway Protocol) network in Figure \ref{fig:example} as the illustration for presentation simplicity. We then introduce how \system{} extends to support multiple protocol networks in \S\ref{multi-protocol section} and handle k-link failure tolerance in \S\ref{k-failure section}.

\para{Requirement.} We define a requirement as a set of intended paths $P$ to forward the traffic from a source node $src$ to a destination node $dst$ with a network prefix $n$ under $k$ link failure, denoted by $req=(src, dst, n, P, k)$. The operator can express the path set $P$ as a regular expression. In the example network, the requirement is $(S, D, n, S*A*D, 0)$. If we want S to reach D under an arbitrary link failure, we can write it as $(S, D, n, S*D, 1)$. Notably, if a node must be included in the path set, we call it a way-point node of this requirement, and if a node must not be included in the path set, we call it a bypass node. 












\subsection{Routing Behavior Abstraction}\label{subsec: 4.1}

\rulan{ACL, ECMP}

% \begin{itemize}
%     \item $Peer(u, v, proc)$. The peer router behavior variable determines whether router $u$ establishes the peer session of protocol $proc$ with $v$. 
    
%     \item $Prefer(r_1, r_2, proc)$. The preference router behavior variable determines whether protocol $ proc$ prefers route $ r_1$ over route $r_2$.

%     \item $isExport(u.proc_1\rightarrow v.proc_2, r)$. The export router behavior variable determines whether the route $r$ can be exported by routing process $proc_1$ at router $u$ to $proc_2$ at $v$, including sending a route to a neighbor or redistributing a route to another routing process.
    
%     \item $isImport(u.proc_1\leftarrow v.proc_2, r)$. The import variable determines if the route $r$ can imported by routing process $proc_1$ at router $u$ from $proc_2$ at $v$. 
%     % the import symbol is a boolean variable indicating if the routing process $proc_1$ at $u$ will import route $r$ from $proc_2$ at $v$.  
% \end{itemize}

\para{Route Propagation Graph Computation.} 
\rulan{for single prefix}
Each RPG is a directed graph in which each node is a routing process with only one incoming edge. It implies how to propagate routes and what routes should be selected as best.
% The RPG is an abstract representation indicating the sufficient (but not necessary) conditions a set of intent-compliant configuration variants must hold. 
\rulan{
The edges and nodes in the RPG are labeled with a set of conditions that a policy-compliant configuration must hold.
Once encountering a broken condition, we force the simulation to go as the condition indicates rather than the given configuration indicates, when the simulation ends, we can find at least one configuration variant whose differences (i.e., the broken conditions) from the given configuration reveals the error.
}

Given a route propagation graph $G(V, E)$, each edge $e(u.proc_1\rightarrow v.proc_2) \in E$ indicates that: 1) routing process $proc_1$ in $u$ and $proc_2$ in $v$ should be routing neighbor, 2) $u.proc_1$ must send its best route to $v.proc_2$, 3) $v.proc_2$ must receive the route from $u.proc_1$. In Figure \ref{fig:example} example, the RPG is D-A-S (we omit the BGP process notation since this is a single-protocol network). Such that D-A and A-S should be BGP neighbors, D (A) should send its best route to A (S), and A (S) should receive routes from D (A), respectively. 
We define the best route of a node $v$ in RPG as the route propagated along the path from $dst$ to $v$. For example, A's BGP routing process should select the route whose next-hop is D and as-path is $[D]$ as the best route.

We build one RPG for all requirements destined to the same prefix. Given a set of requirements for the same prefix, we build the RPG as follows.
% There is one requirement in the example network, so we choose D-A-S as the route propagation graph since its reverse (\ie, S-A-D) is the shortest intent-compliant traffic forwarding path. It indicates that the route originated from D must be propagated and selected along the path. 

\para{Computing all intent-compliant paths for the given configuration.} 
We first compute all possible paths for reversed regular expressions ($D*A*S$ in the example network) based on the routing-level topology (BGP neighbor relationship in the example network) we extract from the network configuration. Suppose there is no such path for a requirement in the routing-level topology. We will try to add routing neighbors by scanning the configuration to search for potential neighbors that are configured but have not established peer sessions successfully. 
Specifically, we transform each regular expression into a deterministic finite automaton (DFA). Then, traversing the routing topology based on these DFAs using depth-first search. Starting from the initial state of DFA, we explore all possible paths in the topology, ensuring each transition between nodes corresponds to a valid transition in the DFA. As the traversal progresses, we continue exploring that path if the current state and edge comply with the automaton's transitions. The current path is stored as valid whenever the traversal reaches a node corresponding to an accepting state in the DFA. This process repeats until all possible paths are explored. In the example network, we will get D-A-S, D-A-B-S, and D-B-A-S.

% we choose the shortest path if . Otherwise, we choose the first satisfiable path for way-point/bypass requirements using the breadth-first search algorithm.
%for the requirement having no way-point or bypass node. 



% \para{Solving conflicts between packet forwarding paths.} 
% % After computing the packet forwarding path for each requirement, we aggregate them into a graph. 
% Conflicts could exist between paths if a node has different forwarding paths to reach the same prefix. Suppose we compute two packet forwarding paths $p_i$ and $p_j$ for requirements $req_i=(src_i, dst, n, P_i, 0)$ and $req_j=(src_j, dst, n, P_j, 0)$ respectively. 
% We define that $p_i$ and $p_j$ have a conflict if they have an intersection node where the next node of it in path $p_i$ and $p_j$ are different.
% In that case, we find the first intersection node $v$ and check if we can replace the sub-path of one forwarding path with the other one's sub-path. Formally, if $subpath(src_i, v, p_i)\oplus subpath(v, dst, p_j) \in P_i$ (or $subpath(src_j, v, p_j)\oplus subpath(v, dst, p_i) \in P_j$), we replace it with $p_i$ (or $p_j$). Otherwise, we must re-compute an intent-compliant path for $req_i$ where $req_i$ is the violated requirement. 


\para{Generating the RPG for the given requirements.}
We now choose a specific route propagation path for each requirement to generate the RPG.
For satisfied requirements, we still use the reserved existing packet forwarding paths as their route propagation paths. 
For violated requirements, we choose an intent-compliant path that does not conflict with current route propagation paths, \ie, each node has at most one incoming node, indicating it only selects the route from that node as the best route.
Finally, we aggregate all route propagation paths into a graph to generate the RPG.

% \begin{table*}[t!]
%   \centering
%   \begin{tabular}{p{4.7cm}|p{12cm}} %p{5.3cm}|p{11.5cm}
%     \hline
%     Violated condition & Configuration patch \\
    
%     \hline
%     $Peer(u, v, proc)$ & Enable the routing peer of the $proc$ protocol between $u$ and $v$. \\
    
%     $isExport(u.proc_1 \rightarrow v.proc_2, r)$ &  Do not filter the route $r$ to $v.proc_2$ in $u.proc_1$. Change the policy rule to permit or add the redistribution command. \\
    
%     $isImport(u.proc_1 \leftarrow v.proc_2, r)$ & Do not filter the route $r$ from $v.proc_2$ in $u.proc_1$. Change the policy rule to permit.\\
    
%     $Prefer(r_1, r_2, proc)$ & Let route $r_1$ be selected by protocol $proc$ by setting a lower cost to $r_1$. \\
     
%     \hline
%   \end{tabular}
%   \caption{Patch generation for violated conditions.}
%   \vspace{-1em}
%   \label{tab:patch table}
% \end{table*}



\subsection{Patches Generation} \label{subsec:4.2}
Once the simulation reaches the network state that does not comply with the RPG, we fork a new simulation process that complies with the RPG to keep simulating.

The goal of selective symbolic simulation is to find a configuration variant. We achieve this by introducing router behavior variables that violate these conditions as RPG indicates to keep simulating until we obtain at least one intent-compliant configuration. 


Figure \ref{sss process} shows the selective symbolic simulation of the example network. We use a quadruple
(prefix, as-path, community-set, conditions) to denote a BGP
route.  
In part (1), $D$ needs to decide whether to redistribute the route $r_0$ into its BGP process. The given configuration determines not to redistribute. However, it violates the condition $Cond_1: isExport(D.static\rightarrow D.BGP, r0)=True$ that indicates $r_0$ should be redistributed from D's static process to its BGP process. So, we introduce the symbolic router behavior $Cond_1$ and let the simulation continue. Then D will transform $r0$ into $r1$, choose $r_1$ as the best BGP route with $Cond_1$, and send it to neighbors A and B. The simulation continues to compute routes $r_2, r_3$. These routes all have the condition $Cond_1$, indicating that they exist only if $Cond_1$ holds.



In part (2), we simulate B sends its best route to A and S. S will drop the route from B since it has the forbidden community tag $d_1$. In part (3), A received two routes and needs to select one as its best route; the given configuration determines $r_4$ is preferred since it will be set local-preference 200 compared to the 100 for $r_3$. However, as the RPG indicates, this behavior violates the condition $Cond_2: Prefer(r_3, r_4, BGP)=True$ because $r_3$ sent by neighbor D is supposed to be preferred over routes from all other neighbors. So we add the second symbolic router behavior $Cond_2$ to A's egress route $e_4$ and $e_5$ to continue simulating, indicating that $r_3$ will be sent to its neighbors only if $r_3$ is selected as A's best route (\ie, $Cond_2$ holds) and D redistributes $r_0$ to its BGP process (\ie, $Cond_1$ holds).

In part (4), after S sends its best route to B, the network converges, and the selective symbolic simulation ends, outputting a set of symbolic routes computed as the RPG suggests. Hence, their symbolic router behaviors indicate the conditions that the intent-compliant configuration must hold. 


% the program encounters the next "if" branch where the condition $Cond_2$ determines whether $r_3$ would be preferred over $r_4$ in router A. 
% The preferred route  
% If the program goes to the "false" branch, A will choose $r_4$ and send it to S. S will drop it since $r_4$ carries community tag $d1$. So we have a condition $Cond_2=true$ and let the program go to the "true" branch. Then A will choose $r_3$, and S will receive it and choose it as the best route. 




% To improve efficiency, we do not keep all execution paths triggered by the above conditions. We tend always to guard the newest execution path that satisfies all conditions in this way. Once a condition is triggered and the actual router behavior does not comply it, we record it as the deviation condition of this path, and then continue to execute the computation. 










\subsection{Supporting Complex Configuration}
% To ensure that each node $i$ eventually follows the path in the forwarding tree to propagate traffic, we use prefix, next-hop, and as-path attributes to identify the target route for node $i$.
% The priority condition is that $i$ always chooses the target route as the best route (\ie, has the highest priority) for the destination prefix.
% Each node $i$ must propagate the route to its in-neighbors so that its in-neighbors can receive the target route. 
% Additionally, if node $i$ adjacent to its out-neighbor $n_{out}$ and in-neighbor $n_{in}$ uses different protocols, node $i$ needs to redistribute the target route to the routing processes of nodes $i$ and $n_{in}$.
% Import condition for route delivery. The import condition follows the same intuition as the export condition: ensuring the target route is delivered to the corresponding node in the forwarding tree. Specifically, node $i$ has to receive the target route from its out-neighbor rather than filter it. If a node has no out-neighbor, the condition for it is to filter all routes from adjacent peers.
% Adjacent condition between routers. The adjacency condition. In the forwarding tree, we define the adjacency condition for nodes with out-neighbors as the node must establish the peer session with its out-neighbor.
